PViT: Prior-augmented Vision Transformer for Out-of-distribution Detection

Vision Transformers (ViTs) have achieved remarkable success over various vision tasks, yet their robustness against data distribution shifts and inherent inductive biases remain underexplored. To enhance the robustness of ViT models for image Out-of-Distribution (OOD) detection, we introduce a novel and generic framework named Prior-augmented Vision Transformer (PViT). Taking as input the prior class logits from a pretrained model, we train PViT to predict the class logits. During inference, PViT identifies OOD samples by quantifying the divergence between the predicted class logits and the prior logits obtained from pre-trained models. Unlike existing state-of-the-art(SOTA) OOD detection methods, PViT shapes the decision boundary between ID and OOD by utilizing the proposed prior guided confidence, without requiring additional data modeling, generation methods, or structural modifications. Extensive experiments on the large-scale ImageNet benchmark, evaluated against over seven OOD datasets, demonstrate that PViT significantly outperforms existing SOTA OOD detection methods in terms of FPR95 and AUROC. The codebase is publicly available at https://github.com/RanchoGoose/PViT.

==> bib_backup.tex <==
% IEEE Transactions
@String(PAMI   = {IEEE Transactions on Pattern Analysis and Machine Intelligence})
@String(TIP    = {IEEE Transactions on Image Processing})
@String(TVCG   = {IEEE Transactions on Visualization and Computer Graphics})
@String(TMM    = {IEEE Transactions on Multimedia})
@String(TCSVT  = {IEEE Transactions on Circuits and Systems for Video Technology})
@String(SPL    = {IEEE Signal Processing Letters})

% ACM Transactions and Conferences
@String(TOG    = {ACM Transactions on Graphics})
@String(ACMMM  = {ACM International Conference on Multimedia})
@String(CGF    = {Computer Graphics Forum})

% Computer Vision Conferences
@String(CVPR   = {IEEE Conference on Computer Vision and Pattern Recognition})
@String(CVPRW  = {IEEE Conference on Computer Vision and Pattern Recognition Workshops})
@String(ICCV   = {International Conference on Computer Vision})
@String(ECCV   = {European Conference on Computer Vision})
@String(BMVC   = {British Machine Vision Conference})
@String(ICPR   = {International Conference on Pattern Recognition})
@String(ACCV   = {Asian Conference on Computer Vision})

% Machine Learning and AI Conferences
@String(NIPS   = {Advances in Neural Information Processing Systems})
@String(ICLR   = {International Conference on Learning Representations})
@String(ICML   = {International Conference on Machine Learning})
@String(IJCAI  = {International Joint Conference on Artificial Intelligence})
@String(AAAI   = {Association for the Advancement of Artificial Intelligence Conference})

% Multimedia and Vision Journals
@String(ICIP   = {IEEE International Conference on Image Processing})
@String(ICME   = {IEEE International Conference on Multimedia and Expo})
@String(TVC    = {The Visual Computer})
@String(JCST   = {Journal of Computer Science and Technology})
@String(VR     = {Vision Research})
@String(JOV    = {Journal of Vision})

% Miscellaneous
@String(PR     = {Pattern Recognition})
@String(CVM    = {Computational Visual Media})


@article{cosmides1996humans,
	title={Are humans good intuitive statisticians after all? Rethinking some conclusions from the literature on judgment under uncertainty},
	author={Cosmides, Leda and Tooby, John},
	journal={Cognition},
	volume={58},
	number={1},
	pages={1--73},
	year={1996},
	publisher={Elsevier}
}

@article{janai2017computer,
  title={Computer vision for autonomous vehicles: Problems, datasets and state of the art},
  author={Janai, Joel and G{\"u}ney, Fatma and Behl, Aseem and Geiger, Andreas and others},
  journal={Foundations and Trends in Computer Graphics and Vision},
  volume={12},
  number={1--3},
  pages={1--308},
  year={2020},
  publisher={Now Publishers, Inc.}
}

@article{feng2019modal,
	title={Deep multi-modal object detection and semantic segmentation for autonomous driving: Datasets, methods, and challenges},
	author={Feng, Di and Haase-Schuetz, Christian and Rosenbaum, Lars and Hertlein, Heinz and Timm, Fabian and Glaeser, Claudius and Wiesbeck, Werner and Dietmayer, Klaus},
	year={2020},
	pages={1-20},
	journal=IEEE_J_ITS,
	doi={10.1109/TITS.2020.2972974},
	ISSN={1524-9050},}


@inproceedings{wang2020inferring,
	title={Inferring Spatial Uncertainty in Object Detection},
	author={Zining Wang and Feng, Di and Zhou, Yiyang and Zhan, Wei and Rosenbaum, Lars and Timm, Fabian and Dietmayer, Klaus and Tomizuka, Masayoshi},
	booktitle=IEEE_IROS,
	xorganization={IEEE},
	year={2020},
}

@article{mackay1992practical,
	title={A practical {B}ayesian framework for backpropagation networks},
	author={MacKay, David J. C.},
	journal={Neural Computation},
	volume={4},
	number={3},
	pages={448--472},
	year={1992},
	publisher={MIT Press}
}

@book{neal2012bayesian,
  title={Bayesian learning for neural networks},
  author={Neal, Radford M},
  volume={118},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{mandt2017stochastic,
  title={Stochastic gradient descent as approximate bayesian inference},
  author={Mandt, Stephan and Hoffman, Matthew D and Blei, David M},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={4873--4907},
  year={2017},
  publisher={JMLR. org}
}

@article{chen2020statistical,
  title={Statistical inference for model parameters in stochastic gradient descent},
  author={Chen, Xi and Lee, Jason D and Tong, Xin T and Zhang, Yichen and others},
  journal={The Annals of Statistics},
  volume={48},
  number={1},
  pages={251--273},
  year={2020},
  publisher={Institute of Mathematical Statistics}
}

@article{brostow2009semantic,
  title={Semantic object classes in video: A high-definition ground truth database},
  author={Brostow, Gabriel J and Fauqueur, Julien and Cipolla, Roberto},
  journal={Pattern Recognition Letters},
  volume={30},
  number={2},
  pages={88--97},
  year={2009},
  publisher={Elsevier}
}

@article{everingham2010pascal,
	title={The {PASCAL} visual object classes ({VOC}) challenge},
	author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
	journal={Int. J. Computer Vision},
	volume={88},
	number={2},
	pages={303--338},
	year={2010},
	publisher={Springer}
}

@inproceedings{czarnecki2018towards,
	title={Towards a framework to manage perceptual uncertainty for safe automated driving},
	author={Czarnecki, Krzysztof and Salay, Rick},
	booktitle={International Conference on Computer Safety, Reliability, and Security},
	pages={439--445},
	year={2018},
	organization={Springer}
}

@article{costante2020uncertainty,
  title={Uncertainty estimation for data-Driven visual odometry},
  author={Costante, Gabriele and Mancini, Michele},
  journal={IEEE Transactions on Robotics},
  year={2020},
  publisher={IEEE}
}

@article{brocker2007properscoring,
  title={Scoring probabilistic forecasts: The importance of being proper},
  author={Br{\"o}cker, Jochen and Smith, Leonard A},
  journal={Weather and Forecasting},
  volume={22},
  number={2},
  pages={382--388},
  year={2007}
}

@article{segu2019general,
	title={A general framework for uncertainty estimation in deep learning},
	author={Seg{\`u}, Mattia and Loquercio, Antonio and Scaramuzza, Davide},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={2},
  pages={3153--3160},
  year={2020},
  publisher={IEEE}
}

@article{yan2018second,
	title={Second: Sparsely embedded convolutional detection},
	author={Yan, Yan and Mao, Yuxing and Li, Bo},
	journal={Sensors},
	volume={18},
	number={10},
	pages={3337},
	year={2018},
	publisher={Multidisciplinary Digital Publishing Institute}
}
@article{braun2019eurocity,
  title={EuroCity persons: A novel benchmark for person detection in traffic scenes},
  author={Braun, Markus and Krebs, Sebastian and Flohr, Fabian and Gavrila, Dariu M},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={41},
  number={8},
  pages={1844--1861},
  year={2019},
  publisher={IEEE}
}

@article{nicholson2018quadricslam,
  title={Quadricslam: Dual quadrics from object detections as landmarks in object-oriented slam},
  author={Nicholson, Lachlan and Milford, Michael and S{\"u}nderhauf, Niko},
  journal={IEEE Robotics and Automation Letters},
  volume={4},
  number={1},
  pages={1--8},
  year={2018},
  publisher={IEEE}
}

@article{gneiting2007strictly,
  title={Strictly proper scoring rules, prediction, and estimation},
  author={Gneiting, Tilmann and Raftery, Adrian E},
  journal={Journal of the American statistical Association},
  volume={102},
  number={477},
  pages={359--378},
  year={2007},
  publisher={Taylor \& Francis}
}

@inproceedings{hu2018probabilistic,
  title={Probabilistic prediction of vehicle semantic intention and motion},
  author={Hu, Yeping and Zhan, Wei and Tomizuka, Masayoshi},
  booktitle=IEEE_IV,
  year={2018},
  organization={IEEE}
}

@INPROCEEDINGS{sun2019scalability,
  title={Scalability in perception for autonomous driving: Waymo open dataset},
  author={Pei Sun and Henrik Kretzschmar and Xerxes Dotiwalla and Aurelien Chouard and Vijaysai Patnaik and Paul Tsui and James Guo and Yin Zhou and Yuning Chai and Benjamin Caine and Vijay Vasudevan and Wei Han and Jiquan Ngiam and Hang Zhao and Aleksei Timofeev and Scott Ettinger and Maxim Krivokon and Amy Gao and Aditya Joshi and Yu Zhang and Jon Shlens and Zhifeng Chen and Dragomir Anguelov},
	booktitle = CVPR,
	year = {2020},
	pages={2446--2454},
	xorganization = {IEEE},
}

@book{huber2004robust,
  title={Robust statistics},
  author={Huber, Peter J},
  volume={523},
  year={2004},
  publisher={John Wiley \& Sons}
}

@article{huang2019apolloscape,
  title={The apolloscape open dataset for autonomous driving and its application},
  author={Huang, Xinyu and Wang, Peng and Cheng, Xinjing and Zhou, Dingfu and Geng, Qichuan and Yang, Ruigang},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={42},
  number={10},
  pages={2702--2719},
  year={2019},
  publisher={IEEE}
}

@inproceedings{quinonero2005evaluating,
  title={Evaluating predictive uncertainty challenge},
  author={Quinonero-Candela, Joaquin and Rasmussen, Carl Edward and Sinz, Fabian and Bousquet, Olivier and Sch{\"o}lkopf, Bernhard},
  booktitle={Machine Learning Challenges Workshop},
  pages={1--27},
  year={2005},
  organization={Springer}
}

@inproceedings{kohonen2005lessons,
  title={Lessons learned in the challenge: making predictions and scoring them},
  author={Kohonen, Jukka and Suomela, Jukka},
  booktitle={Machine Learning Challenges Workshop},
  pages={95--116},
  year={2005},
  organization={Springer}
}

@article{brocker2007scoring,
  title={Scoring probabilistic forecasts: The importance of being proper},
  author={Br{\"o}cker, Jochen and Smith, Leonard A},
  journal={Weather and Forecasting},
  volume={22},
  number={2},
  pages={382--388},
  year={2007}
}

@article{bernardo_1979,
  title={Expected information as expected utility},
  author={Bernardo, Jos{\'e} M},
  journal={the Annals of Statistics},
  pages={686--690},
  year={1979},
  publisher={JSTOR}
}

@article{brier_1950,
  title={Verification of forecasts expressed in terms of probability},
  author={Brier, Glenn W},
  journal={Monthly weather review},
  volume={78},
  number={1},
  pages={1--3},
  year={1950}
}

@article{brocker2009reliability,
  title={Reliability, sufficiency, and the decomposition of proper scores},
  author={Br{\"o}cker, Jochen},
  journal={Quarterly Journal of the Royal Meteorological Society: A journal of the atmospheric sciences, applied meteorology and physical oceanography},
  volume={135},
  number={643},
  pages={1512--1519},
  year={2009},
  publisher={Wiley Online Library}
}
@article{gneiting2007probabilistic,
  title={Probabilistic forecasts, calibration and sharpness},
  author={Gneiting, Tilmann and Balabdaoui, Fadoua and Raftery, Adrian E},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={69},
  number={2},
  pages={243--268},
  year={2007},
  publisher={Wiley Online Library}
}
%% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %% %%
%% Conferences
@inproceedings{harakeh2021estimating,
title={Estimating and Evaluating Regression Predictive Uncertainty in Deep Object Detectors},
author={Ali Harakeh and Steven L. Waslander},
booktitle={Proceedings of International Conference on Learning Representations},
year={2021}}

@inproceedings{yang2020surfelgan,
  title={SurfelGAN: Synthesizing Realistic Sensor Data for Autonomous Driving},
  author={Yang, Zhenpei and Chai, Yuning and Anguelov, Dragomir and Zhou, Yin and Sun, Pei and Erhan, Dumitru and Rafferty, Sean and Kretzschmar, Henrik},
  booktitle=CVPR,
  year={2020}
}
@article{wang2017detecting,
  title={Detecting semantic parts on partially occluded objects},
  author={Wang, Jianyu and Xie, Cihang and Zhang, Zhishuai and Zhu, Jun and Xie, Lingxi and Yuille, Alan},
  journal=MACHINE_VISION,
  year={2017}
}
@inproceedings{hall2020probability,
  title={Probabilistic object detection: Definition and evaluation},
  author={Hall, David and Dayoub, Feras and Skinner, John and Zhang, Haoyang and Miller, Dimity and Corke, Peter and Carneiro, Gustavo and Angelova, Anelia and S{\"u}nderhauf, Niko},
  booktitle={The IEEE Winter Conference on Applications of Computer Vision},
  pages={1031--1040},
  year={2020}
}
@inproceedings{dong2020probabilistic,
  title={Probabilistic Oriented Object Detection in Automotive Radar},
  author={Dong, Xu and Wang, Pengluo and Zhang, Pengyue and Liu, Langechuan},
  booktitle={CVPR Workshops},
  year={2020}
}
@misc{he2020deep,
    title={Deep Mixture Density Network for Probabilistic Object Detection},
    author={Yihui He and Jianren Wang, Wang, Zhixin and Jia, Kui},
	booktitle=IEEE_IROS,
	year={2020}}
	
@inproceedings{le2018uncertainty,
  title={Uncertainty estimation for deep neural object detectors in safety-critical applications},
  author={Le, Michael Truong and Diehl, Frederik and Brunner, Thomas and Knol, Alois},
  booktitle=IEEE_ITSC,
  year={2018}}

@inproceedings{manivasagam2020lidarsim,
  title={LiDARsim: Realistic LiDAR Simulation by Leveraging the Real World},
  author={Manivasagam, Sivabalan and Wang, Shenlong and Wong, Kelvin and Zeng, Wenyuan and Sazanovich, Mikita and Tan, Shuhan and Yang, Bin and Ma, Wei-Chiu and Urtasun, Raquel},
  booktitle=CVPR,
  year={2020}
}

@inproceedings{kato2018autoware,
  title={Autoware on board: Enabling autonomous vehicles with embedded systems},
  author={Kato, Shinpei and Tokunaga, Shota and Maruyama, Yuya and Maeda, Seiya and Hirabayashi, Manato and Kitsukawa, Yuki and Monrroy, Abraham and Ando, Tomohito and Fujii, Yusuke and Azumi, Takuya},
  booktitle={2018 ACM/IEEE 9th International Conference on Cyber-Physical Systems (ICCPS)},
  pages={287--296},
  year={2018},
  organization={IEEE}
}

@inproceedings{fruhwirth2020towards,
  title={Towards Data-driven Multi-target Tracking for Autonomous Driving},
  author={Fruhwirth-Reisinger, Christian and Krispel, Georg and Possegger, Horst and Bischof, Horst},
  booktitle={Computer Vision Winter Workshop (CVWW)},
  year={2020}
}
@article{ashukha2020pitfalls,
  title={Pitfalls of in-domain uncertainty estimation and ensembling in deep learning},
  author={Ashukha, Arsenii and Lyzhov, Alexander and Molchanov, Dmitry and Vetrov, Dmitry},
  journal={Eighth International Conference on Learning Representations (ICLR)},
  year={2020}
}
@article{chen2020monopair,
  title={MonoPair: Monocular 3D Object Detection Using Pairwise Spatial Relationships},
  author={Chen, Yongjian and Tai, Lei and Sun, Kai and Li, Mingyang},
  journal=CVPR,
  year={2020}
}
@inproceedings{bodla2017soft,
  title={{Soft-NMS}-improving object detection with one line of code},
  author={Bodla, Navaneeth and Singh, Bharat and Chellappa, Rama and Davis, Larry S},
  booktitle=ICCV,
  year={2017}
}
@inproceedings{pan2020towards,
  title={Towards Better Performance and More Explainable Uncertainty for 3D Object Detection of Autonomous Vehicles},
  author={Pan, Hujie and Wang, Zining and Zhan, Wei and Tomizuka, Masayoshi},
  booktitle=IEEE_ITSC,
  year={2020}
}

@inproceedings{choi2019gaussian,
  title={Gaussian yolov3: An accurate and fast object detector using localization uncertainty for autonomous driving},
  author={Choi, Jiwoong and Chun, Dayoung and Kim, Hyun and Lee, Hyuk-Jae},
  booktitle=ICCV,
  year={2019}
}
@inproceedings{lin2014microsoft,
	title={Microsoft {COCO}: Common Objects in Context},
	author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C. Lawrence},
	booktitle=ECCV,
	year={2014}}
	
@inproceedings{sunderhauf2016place,
  title={Place categorization and semantic mapping on a mobile robot},
  author={S{\"u}nderhauf, Niko and Dayoub, Feras and McMahon, Sean and Talbot, Ben and Schulz, Ruth and Corke, Peter and Wyeth, Gordon and Upcroft, Ben and Milford, Michael},
  booktitle=IEEE_ICRA,
  year={2016},
  organization={IEEE}
}

@article{nuscenes2019,
	title={nu{S}cenes: A multimodal dataset for autonomous driving},
	author={Holger Caesar and Varun Bankiti and Alex H. Lang and Sourabh Vora and 
	Venice Erin Liong and Qiang Xu and Anush Krishnan and Yu Pan and 
	Giancarlo Baldan and Oscar Beijbom},
	journal=CVPR,
	year={2020}
}

@inproceedings{mccormac2017scenenet,
  title={SceneNet RGB-D: Can 5M synthetic images beat generic ImageNet pre-training on indoor segmentation?},
  author={McCormac, John and Handa, Ankur and Leutenegger, Stefan and Davison, Andrew J},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{wirges2018object,
  title={Object detection and classification in occupancy grid maps using deep convolutional networks},
  author={Wirges, Sascha and Fischer, Tom and Stiller, Christoph and Frias, Jesus Balado},
  booktitle=IEEE_ITSC,
  year={2018}}

@inproceedings{kraus2019uncertainty,
  title={Uncertainty Estimation in One-Stage Object Detection},
  author={Kraus, Florian and Dietmayer, Klaus},
  booktitle=IEEE_ITSC,
  year={2019}}

@inproceedings{bertoni2019monoloco,
  title={MonoLoco: Monocular 3D Pedestrian Localization and Uncertainty Estimation},
  author={Bertoni, Lorenzo and Kreiss, Sven and Alahi, Alexandre},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{szegedy2015going,
	title={Going deeper with convolutions},
	author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
	booktitle=CVPR,
	year={2015}
}

@inproceedings{he2016deep,
	title={Deep residual learning for image recognition},
	author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	booktitle=CVPR,
	year={2016}
}


@article{liu2020deep,
  title={Deep learning for generic object detection: A survey},
  author={Liu, Li and Ouyang, Wanli and Wang, Xiaogang and Fieguth, Paul and Chen, Jie and Liu, Xinwang and Pietik{\"a}inen, Matti},
  journal={International journal of computer vision},
  volume={128},
  number={2},
  pages={261--318},
  year={2020},
  publisher={Springer}
}


@inproceedings{roddick2019orthographic,
  title={Orthographic feature transform for monocular 3D object detection},
  author={Roddick, T and Kendall, A and Cipolla, R},
  booktitle=MACHINE_VISION,
  year={2019}
}

@article{simonyan2014very,
	title={Very deep convolutional networks for large-scale image recognition},
	author={Simonyan, Karen and Zisserman, Andrew},
	journal={Third International Conference on Learning Representations (ICLR)},
	year={2015}
}

@inproceedings{huang2017speed,
	title={Speed/accuracy trade-offs for modern convolutional object detectors},
	author={Huang, Jonathan and Rathod, Vivek and Sun, Chen and Zhu, Menglong and Korattikara, Anoop and Fathi, Alireza and Fischer, Ian and Wojna, Zbigniew and Song, Yang and Guadarrama, Sergio and others},
	booktitle=CVPR,
	volume={4},
	year={2017}
}

@INPROCEEDINGS{qi2017pointnet, 
	author={Qi, Charles R. and Su, Hao and Mo, Kaichun and Guibas, Leonidas J.},
	booktitle=CVPR, 
	title={{PointNet}: Deep Learning on Point Sets for 3D Classification and Segmentation}, 
	year={2017}}

@inproceedings{lang2018pointpillars,
	title={{PointPillars}: Fast Encoders for Object Detection from Point Clouds},
	author={Lang, Alex H and Vora, Sourabh and Caesar, Holger and Zhou, Lubing and Yang, Jiong and Beijbom, Oscar},
	booktitle=CVPR,
	year={2018}
}

@inproceedings{xu2017pointfusion,
	title={{PointFusion}: Deep Sensor Fusion For {3D} Bounding Box Estimation},
	author={Xu, Danfei and Anguelov, Dragomir and Jain, Ashesh},
	booktitle=CVPR,
	year={2018}}

@inproceedings{fei2020semanticvoxels,
	title={SemanticVoxels: Sequential Fusion for 3D Pedestrian Detection using LiDAR Point Cloud and Semantic Segmentation},
	author={Fei, Juncong and Chen, Wenbo and Heidenreich, Philipp and Wirges, Sascha and Stiller, Christoph},
	booktitle={IEEE Int. Conf. Multisensor Fusion and Integration},
	year={2019}
}

@inproceedings{shi2019pointrcnn,
	title={{Point-RCNN}: 3d object proposal generation and detection from point cloud},
	author={Shi, Shaoshuai and Wang, Xiaogang and Li, Hongsheng},
	booktitle=CVPR,
	year={2019}
}

@inproceedings{yang2018pixor,
	title={{PIXOR}: Real-Time 3D Object Detection From Point Clouds},
	author={Yang, Bin and Luo, Wenjie and Urtasun, Raquel},
	booktitle=CVPR,
	year={2018}
}

@inproceedings{zhou2017voxelnet,
	title={{VoxelNet}: End-to-End Learning for Point Cloud Based 3D Object Detection},
	author={Zhou, Yin and Tuzel, Oncel},
	booktitle=CVPR,
	year={2018}}

@inproceedings{tian2019fcos,
  title={Fcos: Fully convolutional one-stage object detection},
  author={Tian, Zhi and Shen, Chunhua and Chen, Hao and He, Tong},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{shi2020pv,
	title={{PV-RCNN}: Point-Voxel Feature Set Abstraction for 3D Object Detection},
	author={Shi, Shaoshuai and Guo, Chaoxu and Jiang, Li and Wang, Zhe and Shi, Jianping and Wang, Xiaogang and Li, Hongsheng},
	booktitle=CVPR,
	year={2020}
}

@inproceedings{simon2018complex,
	title={Complex-YOLO: An Euler-Region-Proposal for Real-Time 3D Object Detection on Point Clouds},
	author={Simon, Martin and Milz, Stefan and Amende, Karl and Gross, Horst-Michael},
	booktitle=ECCV,
	year={2018}}

@INPROCEEDINGS{ku2017joint, 
	author={Ku, Jason and Mozifian, Melissa and Lee, Jungwook and Harakeh, Ali and Waslander, Steven},
	booktitle=IEEE_IROS, 
	title={Joint 3D Proposal Generation and Object Detection from View Aggregation},
	year={2018}}
	
@inproceedings{chen2017multi,
	title={Multi-view {3D} Object Detection Network for Autonomous Driving},
	author={Chen, Xiaozhi and Ma, Huimin and Wan, Ji and Li, Bo and Xia, Tian},
	booktitle=CVPR,
	year={2017}}

@article{carion2020end,
  title={End-to-End Object Detection with Transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  journal=ECCV,
  year={2020}
}

@inproceedings{girshick2015fast,
	title={{Fast R-CNN}},
	author={Girshick, Ross},
	booktitle=ICCV,
	pages={1440--1448},
	year={2015},
}

@inproceedings{girshick2014rich,
	title={Rich feature hierarchies for accurate object detection and semantic segmentation},
	author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
	booktitle=CVPR,
	pages={580--587},
	year={2014}
}

@article{zhou2019objects,
  title={Objects as Points},
  author={Zhou, Xingyi and Wang, Dequan and Kr{\"a}henb{\"u}hl, Philipp},
  journal={arXiv preprint arXiv:1904.07850},
  year={2019}
}

@inproceedings{ren2015faster,
	title={{Faster R-CNN}: Towards real-time object detection with region proposal networks},
	author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
	booktitle=NIPS,
	year={2015},
}

@inproceedings{engelcke2017vote3deep,
	title={{Vote3Deep}: Fast object detection in 3d point clouds using efficient convolutional neural networks},
	author={Engelcke, Martin and Rao, Dushyant and Wang, Dominic Zeng and Tong, Chi Hay and Posner, Ingmar},
	booktitle=IEEE_ICRA,
	year={2017}}

@inproceedings{asvadi2017depthcn,
	title={{DepthCN}: Vehicle detection using 3D-LIDAR and {ConvNet}},
	author={Asvadi, Alireza and Garrote, Lu{\'\i}s and Premebida, Cristiano and Peixoto, Paulo and Nunes, Urbano J},
	booktitle=IEEE_ITSC,
	year={2017}}

@inproceedings{deng2009imagenet,
  title={{ImageNet}: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle=CVPR,
  year={2009}}
  
@inproceedings{redmon2016you,
	title={You only look once: Unified, real-time object detection},
	author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
	booktitle=CVPR,
	year={2016}
}

@inproceedings{liu2016ssd,
	title={{SSD}: Single shot multibox detector},
	author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C.},
	booktitle=ECCV,
	year={2016}}

@article{kuleshov2018accurate,
  title={Accurate uncertainties for deep learning using calibrated regression},
  author={Kuleshov, Volodymyr and Fenner, Nathan and Ermon, Stefano},
  journal= {Thirty-fifth Interntional Conference on Machine Learning (ICML)},
  year={2018}
}
@inproceedings{kumar2019verified,
  title={Verified uncertainty calibration},
  author={Kumar, Ananya and Liang, Percy S and Ma, Tengyu},
  booktitle=NIPS,
  year={2019}
}
@inproceedings{guo2017calibration,
	title={On calibration of modern neural networks},
	author={Guo, Chuan and Pleiss, Geoff and Sun, Yu and Weinberger, Kilian Q},
	booktitle=ICML,
	year={2017},
}

@inproceedings{snoek2019can,
  title={Can you trust your model's uncertainty? Evaluating predictive uncertainty under dataset shift},
  author={Snoek, Jasper and Ovadia, Yaniv and Fertig, Emily and Lakshminarayanan, Balaji and Nowozin, Sebastian and Sculley, D and Dillon, Joshua and Ren, Jie and Nado, Zachary},
  booktitle=NIPS,
  year={2019}
}

@inproceedings{lakshminarayanan2017simple,
	title={Simple and scalable predictive uncertainty estimation using deep ensembles},
	author={Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
	booktitle=NIPS,
	year={2017}
}
@inproceedings{gal2017concrete,
	title={Concrete dropout},
	author={Gal, Yarin and Hron, Jiri and Kendall, Alex},
	booktitle=NIPS,
	year={2017}
}
@inproceedings{blum2019fishyscapes,
  title={Fishyscapes: A benchmark for safe semantic segmentation in autonomous driving},
  author={Blum, Hermann and Sarlin, Paul-Edouard and Nieto, Juan and Siegwart, Roland and Cadena, Cesar},
  booktitle={CVPR Workshops},
  year={2019}
}
@article{tai2019visual,
  title={Visual-based autonomous driving deployment from a stochastic and uncertainty-aware perspective},
  author={Tai, Lei and Yun, Peng and Chen, Yuying and Liu, Congcong and Ye, Haoyang and Liu, Ming},
  journal=IEEE_IROS,
  year={2019}
}

@inproceedings{makansi2019overcoming,
  title={Overcoming limitations of mixture density networks: A sampling and fitting framework for multimodal future prediction},
  author={Makansi, Osama and Ilg, Eddy and Cicek, Ozgun and Brox, Thomas},
  booktitle=CVPR,
  year={2019}
}

@inproceedings{hudnell2019robust,
  title={Robust Aleatoric Modeling for Future Vehicle Localization},
  author={Hudnell, Max and Price, True and Frahm, Jan-Michael},
  booktitle={CVPR Workshops},
  year={2019}
}
@inproceedings{haussmann2020scalable,
  title={Scalable Active Learning for Object Detection},
  author={Haussmann, Elmar and Fenzi, Michele and Chitta, Kashyap and Ivanecky, Jan and Xu, Hanson and Roy, Donna and Mittel, Akshita and Koumchatzky, Nicolas and Farabet, Clement and Alvarez, Jose M},
  booktitle=IEEE_IV,
  year={2020},
}

@InProceedings{Beluch_2018_CVPR,
	author = {Beluch, William H. and Genewein, Tim and N\"urnberger, Andreas and K\"ohler, Jan M.},
	title = {The Power of Ensembles for Active Learning in Image Classification},
	booktitle = CVPR,
	month = jun,
	year = {2018}
} 
@inproceedings{gast2018lightweight,
	title={Lightweight probabilistic deep networks},
	author={Gast, Jochen and Roth, Stefan},
	booktitle=CVPR,
	year={2018}
}
@inproceedings{yang2020d3vo,
  title={D3VO: Deep Depth, Deep Pose and Deep Uncertainty for Monocular Visual Odometry},
  author={Yang, Nan and Stumberg, Lukas von and Wang, Rui and Cremers, Daniel},
  booktitle=CVPR,
  year={2020}
}
@inproceedings{eldesokey2020uncertainty,
  title={Uncertainty-Aware CNNs for Depth Completion: Uncertainty from Beginning to End},
  author={Eldesokey, Abdelrahman and Felsberg, Michael and Holmquist, Karl and Persson, Michael},
  booktitle=CVPR,
  year={2020}
}
@inproceedings{gustafsson2020evaluating,
  title={Evaluating scalable bayesian deep learning methods for robust computer vision},
  author={Gustafsson, Fredrik K and Danelljan, Martin and Schon, Thomas B},
  booktitle={CVPR Workshops},
  year={2020}
}
@inproceedings{kendall2017uncertainties,
	title={What Uncertainties Do We Need in {Bayesian} Deep Learning for Computer Vision?},
	author={Kendall, Alex and Gal, Yarin},
	booktitle=NIPS,
	year={2017}
}

@inproceedings{postels2019sampling,
	title={Sampling-free Epistemic Uncertainty Estimation Using Approximated Variance Propagation},
	author={Postels, Janis and Ferroni, Francesco and Coskun, Huseyin and Navab, Nassir and Tombari, Federico},
	booktitle=ICCV,
	year={2019}
}

@inproceedings{kiani2017need,
  title={Need for speed: A benchmark for higher frame rate object tracking},
  author={Kiani Galoogahi, Hamed and Fagg, Ashton and Huang, Chen and Ramanan, Deva and Lucey, Simon},
  booktitle=ICCV,
  year={2017}
}

@inproceedings{mueller2016benchmark,
  title={A benchmark and simulator for uav tracking},
  author={Mueller, Matthias and Smith, Neil and Ghanem, Bernard},
  booktitle=ECCV,
  year={2016},
}

@inproceedings{wu2013online,
  title={Online object tracking: A benchmark},
  author={Wu, Yi and Lim, Jongwoo and Yang, Ming-Hsuan},
  booktitle=CVPR,
  pages={2411--2418},
  year={2013}
}

@inproceedings{gruber2019gated2depth,
  title={Gated2depth: Real-time dense lidar from gated images},
  author={Gruber, Tobias and Julca-Aguilar, Frank and Bijelic, Mario and Heide, Felix},
  booktitle=ICCV,
  year={2019}
}

@inproceedings{danelljan2020probabilistic,
  title={Probabilistic regression for visual tracking},
  author={Danelljan, Martin and Gool, Luc Van and Timofte, Radu},
  booktitle=CVPR,
  year={2020}
}

@article{hu2020probabilistic,
  title={Probabilistic Future Prediction for Video Scene Understanding},
  author={Hu, Anthony and Cotter, Fergal and Mohan, Nikhil and Gurau, Corina and Kendall, Alex},
  journal=ECCV,
  year={2020}
}

@inproceedings{dosovitskiy2017carla,
  title={CARLA: An Open Urban Driving Simulator},
  author={Dosovitskiy, Alexey and Ros, German and Codevilla, Felipe and Lopez, Antonio and Koltun, Vladlen},
  booktitle={Conference on Robot Learning},
  year={2017}
}

@inproceedings{michelmore2019uncertainty,
	title={Uncertainty Quantification with Statistical Guarantees in End-to-End Autonomous Driving Control},
	author={Michelmore, Rhiannon and Wicker, Matthew and Laurenti, Luca and Cardelli, Luca and Gal, Yarin and Kwiatkowska, Marta},
	booktitle=IEEE_ICRA,
	year={2020}
}

@article{colyar2007us,
  title={US highway 101 dataset},
  author={Colyar, James and Halkias, John},
  journal={Federal Highway Administration (FHWA), Tech. Rep. FHWA-HRT-07-030},
  year={2007}
}

@inproceedings{song2015sun,
  title={{SUN RGB-D}: A {RGB-D} scene understanding benchmark suite},
  author={Song, Shuran and Lichtenberg, Samuel P and Xiao, Jianxiong},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  year={2015}
}

@inproceedings{choi2018uncertainty,
	title={Uncertainty-aware learning from demonstration using mixture density networks with sampling-free variance modeling},
	author={Choi, Sungjoon and Lee, Kyungjae and Lim, Sungbin and Oh, Songhwai},
	booktitle=IEEE_ICRA,
	year={2018}
	}

@inproceedings{ilg2018uncertainty,
	title={Uncertainty Estimates and Multi-Hypotheses Networks for Optical Flow},
	author={Ilg, Eddy and Ci{\c{c}}ek, Ozg{\"u}n and Galesso, Silvio and Klein, Aaron and Makansi, Osama and Hutter, Frank and Brox, Thomas},
	booktitle=ECCV,
	year={2018}
}

@inproceedings{butler2012naturalistic,
  title={A naturalistic open source movie for optical flow evaluation},
  author={Butler, Daniel J and Wulff, Jonas and Stanley, Garrett B and Black, Michael J},
  booktitle=ECCV,
  year={2012}
}

@inproceedings{cordts2016cityscapes,
	title={The {Cityscapes} dataset for semantic urban scene understanding},
	author={Cordts, Marius and Omran, Mohamed and Ramos, Sebastian and Rehfeld, Timo and Enzweiler, Markus and Benenson, Rodrigo and Franke, Uwe and Roth, Stefan and Schiele, Bernt},
	booktitle=CVPR,
	year={2016}
}

@inproceedings{mackowiak2018cereals,
  title={Cereals-cost-effective region-based active learning for semantic segmentation},
  author={Mackowiak, Radek and Lenz, Philip and Ghori, Omair and Diego, Ferran and Lange, Oliver and Rother, Carsten},
  booktitle = MACHINE_VISION,
  year={2018}
}


@inproceedings{kendall2015bayesian,
	title={Bayesian {SegNet}: Model Uncertainty in Deep Convolutional Encoder-Decoder Architectures for Scene Understanding},
	author={Kendall, Alex and Badrinarayanan, Vijay and Cipolla, Roberto},
	booktitle=MACHINE_VISION,
	year={2017}
}

@inproceedings{kendall2015posenet,
  title={Posenet: A convolutional network for real-time 6-dof camera relocalization},
  author={Kendall, Alex and Grimes, Matthew and Cipolla, Roberto},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  year={2015}
}

@inproceedings{kendall2016modelling,
	title={Modelling uncertainty in deep learning for camera relocalization},
	author={Kendall, Alex and Cipolla, Roberto},
	booktitle=IEEE_ICRA,
	year={2016}}

@inproceedings{ritter2018scalable,
  title={A scalable laplace approximation for neural networks},
  author={Ritter, Hippolyt and Botev, Aleksandar and Barber, David},
  booktitle={6th International Conference on Learning Representations (ICLR)},
  year={2018},
}

@inproceedings{maddox2019simple,
  title={A simple baseline for bayesian uncertainty in deep learning},
  author={Maddox, Wesley J and Izmailov, Pavel and Garipov, Timur and Vetrov, Dmitry P and Wilson, Andrew Gordon},
  booktitle=NIPS,
  year={2019}
}

@inproceedings{sensoy2018evidential,
	title={Evidential deep learning to quantify classification uncertainty},
	author={Sensoy, Murat and Kaplan, Lance and Kandemir, Melih},
	booktitle=NIPS,
	year={2018}
}

@inproceedings{mcallister2017concrete,
	title={Concrete problems for autonomous vehicle safety: Advantages of bayesian deep learning},
	author={McAllister, Rowan and Gal, Yarin and Kendall, Alex and Van Der Wilk, Mark and Shah, Amar and Cipolla, Roberto and Weller, Adrian Vivian},
	year={2017},
	booktitle={Int. Joint Conf. on Artificial Intelligence}
}

@INPROCEEDINGS{liu2019itsc,  
author={S. {Liu} and K. {Koch} and B. {Gahr} and F. {Wortmann}}, 
booktitle=IEEE_ITSC,   
title={Brake Maneuver Prediction – An Inference Leveraging RNN Focus on Sensor Confidence},   
year={2019}, 
pages={3249-3255},}


@inproceedings{miller2018dropout,
  title={Dropout sampling for robust object detection in open-set conditions},
  author={Miller, Dimity and Nicholson, Lachlan and Dayoub, Feras and S{\"u}nderhauf, Niko},
  booktitle=IEEE_ICRA,
  year={2018}}
  
@inproceedings{miller2019evaluating,
  title={Evaluating merging strategies for sampling-based uncertainty techniques in object detection},
  author={Miller, Dimity and Dayoub, Feras and Milford, Michael and S{\"u}nderhauf, Niko},
  booktitle=IEEE_ICRA,
  year={2019},
}

@inproceedings{miller2019benchmarking,
  title={Benchmarking Sampling-based Probabilistic Object Detectors.},
  author={Miller, Dimity and S{\"u}nderhauf, Niko and Zhang, Haoyang and Hall, David and Dayoub, Feras},
  booktitle={CVPR Workshops},
  year={2019}
}

@inproceedings{feng2020labels,
	title={Labels Are Not Perfect: Improving Probabilistic Object Detection via Label Uncertainty},
	author={Feng, Di and Rosenbaum, Lars and Timm, Fabian and Dietmayer, Klaus},
	booktitle={Eur. Conf. Computer Vision Workshops},
	year={2020}
}

@article{feng2020labels2,
	title={Labels Are Not Perfect: Inferring Spatial Uncertainty in Object Detection},
	author={Feng, Di and Wang, Zining and Zhou, Yiyang and Zhan, Wei and Rosenbaum, Lars and Timm, Fabian and Dietmayer, Klaus and Tomizuka, Masayoshi},
	year={2020},
	journal={arXiv preprint arXiv:1910.02600},
    }


@inproceedings{gustafsson2020energy,
  author={Gustafsson, Fredrik K and Danelljan, Martin and Bhat, Goutam and Sch{\"o}n, Thomas B},
  title = {Energy-Based Models for Deep Probabilistic Regression},
  booktitle = ECCV,
  month = {August},
  year = {2020}
}

@article{feng2019can,
	title={Can We Trust You? On Calibration of a Probabilistic Object Detector for Autonomous Driving},
	author={Feng, Di and Rosenbaum, Lars and Gl{\"a}ser, Claudius and Timm, Fabian and Dietmayer, Klaus},
	journal=IEEE_IROS,
	year={2020}
}

@inproceedings{blundell2015weight,
	title={Weight uncertainty in neural networks},
	author={Blundell, Charles and Cornebise, Julien and Kavukcuoglu, Koray and Wierstra, Daan},
	booktitle=ICML,
	year={2015},
}

@inproceedings{graves2011practical,
	title={Practical variational inference for neural networks},
	author={Graves, Alex},
	booktitle=NIPS,
	year={2011}
}

@inproceedings{depeweg2018decomposition,
  title={Decomposition of Uncertainty in Bayesian Deep Learning for Efficient and Risk-sensitive Learning},
  author={Depeweg, S and Hernandez-Lobato, JM and Doshi-Velez, F and Udluft, S},
  booktitle=ICML,
  year={2018}
}

@inproceedings{feng2018towards,
	title={Towards Safe Autonomous Driving: Capture Uncertainty in the Deep Neural Network for Lidar 3D Vehicle Detection},
	author={Feng, Di and Rosenbaum, Lars and Dietmayer, Klaus},
	booktitle=IEEE_ITSC,
	pages={3266--3273},
	year={2018}}

@inproceedings{feng2018leveraging,
	title={Leveraging Heteroscedastic Aleatoric Uncertainties for Robust Real-Time LiDAR 3D Object Detection},
	author={Feng, Di and Rosenbaum, Lars and Timm, Fabian and Dietmayer, Klaus},
	booktitle=IEEE_IV,
	year={2019}
}

@inproceedings{feng2019deep,
	title={Deep Active Learning for Efficient Training of a LiDAR 3D Object Detector},
	author={Feng, Di and Wei, Xiao and Rosenbaum, Lars and Maki, Atsuto and Dietmayer, Klaus},
	booktitle=IEEE_IV,
	year={2019}
}

@article{feng2020leveraging,
	title={Leveraging Uncertainties for Deep Multi-modal Object Detection in Autonomous Driving},
	author={Feng, Di and Cao, Yifan and Rosenbaum, Lars and Timm, Fabian and Dietmayer, Klaus},
	journal=IEEE_IV,
	year={2020}
}

@inproceedings{harakeh2019bayesod,
  title={Bayesod: A bayesian approach for uncertainty estimation in deep object detectors},
  author={Harakeh, Ali and Smart, Michael and Waslander, Steven L},
  booktitle=IEEE_ICRA,
  year={2020}
  }

@inproceedings{he2019bounding,
  title={Bounding box regression with uncertainty for accurate object detection},
  author={He, Yihui and Zhu, Chenchen and Wang, Jianren and Savvides, Marios and Zhang, Xiangyu},
  booktitle=CVPR,
  year={2019}}
  
@inproceedings{meyer2019lasernet,
	title={{LaserNet}: An efficient probabilistic 3D object detector for autonomous driving},
	author={Meyer, Gregory P and Laddha, Ankit and Kee, Eric and Vallespi-Gonzalez, Carlos and Wellington, Carl K},
	booktitle=CVPR,
	year={2019}
}

@inproceedings{wirges2019capturing,
	title={Capturing object detection uncertainty in multi-layer grid maps},
	author={Wirges, Sascha and Reith-Braun, Marcel and Lauer, Martin and Stiller, Christoph},
	booktitle=IEEE_IV,
	year={2019}
}

@article{lin2018focal,
	title={Focal loss for dense object detection},
	author={Lin, Tsung-Yi and Goyal, Priyal and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr},
	journal=IEEE_J_PAMI,
	year={2018},
	publisher={IEEE},
}

@inproceedings{welling2011bayesian,
  title={Bayesian learning via stochastic gradient {Langevin} dynamics},
  author={Welling, Max and Teh, Yee W},
  booktitle=ICML,
  year={2011}
}

@inproceedings{yu2020bdd100k,
  title={BDD100K: A diverse driving dataset for heterogeneous multitask learning},
  author={Yu, Fisher and Chen, Haofeng and Wang, Xin and Xian, Wenqi and Chen, Yingying and Liu, Fangchen and Madhavan, Vashisht and Darrell, Trevor},
  booktitle=CVPR,
  year={2020}
}

@inproceedings{Geiger2012CVPR,
	author = {Andreas Geiger and Philip Lenz and Raquel Urtasun},
	title = {Are we ready for Autonomous Driving? The {KITTI} Vision Benchmark Suite},
	booktitle = CVPR,
	year = {2012},
}

@inproceedings{chen2014stochastic,
  title={Stochastic gradient hamiltonian monte carlo},
  author={Chen, Tianqi and Fox, Emily and Guestrin, Carlos},
  booktitle=ICML,
  pages={1683--1691},
  year={2014}
}

@inproceedings{willers2020safety,
  title={Safety Concerns and Mitigation Approaches Regarding the Use of Deep Learning in Safety-Critical Perception Tasks},
  author={Willers, Oliver and Sudholt, Sebastian and Raafatnia, Shervin and Abrecht, Stephanie},
  booktitle={International Conference on Computer Safety, Reliability, and Security},
  year={2020}
}

%% Arxiv
@article{amini2019deep,
	title={Deep Evidential Regression},
	author={Amini, Alexander and Schwarting, Wilko and Soleimany, Ava and Rus, Daniela},
	journal={arXiv preprint arXiv:1910.02600},
	year={2019}
}

@article{meyer2020laserflow,
  title={LaserFlow: Efficient and Probabilistic Object Detection and Motion Forecasting},
  author={Meyer, Gregory P and Charland, Jake and Pandey, Shreyash and Laddha, Ankit and Vallespi-Gonzalez, Carlos and Wellington, Carl K},
  journal={arXiv preprint arXiv:2003.05982},
  year={2020}
}

@article{chitta2018large,
  title={Large-scale visual active learning with deep probabilistic ensembles},
  author={Chitta, Kashyap and Alvarez, Jose M and Lesnikowski, Adam},
  journal={arXiv preprint arXiv:1811.03575},
  year={2018}
}

@article{lee2020localization,
  title={Localization Uncertainty Estimation for Anchor-Free Object Detection},
  author={Lee, Youngwan and Hwang, Joong-won and Kim, Hyung-Il and Yun, Kimin and Park, Joungyoul},
  journal={arXiv preprint arXiv:2006.15607},
  year={2020}
}

@article{meyer2019learning,
	title={Learning an Uncertainty-Aware Object Detector for Autonomous Driving},
	author={Meyer, Gregory P and Thakurdesai, Niranjan},
	journal={arXiv preprint arXiv:1910.11375},
	year={2019}
}

@article{walz2020uncertainty,
  title={Uncertainty depth estimation with gated images for 3D reconstruction},
  author={Walz, Stefanie and Gruber, Tobias and Ritter, Werner and Dietmayer, Klaus},
  journal={arXiv preprint arXiv:2003.05122},
  year={2020}
}

@article{cortinhal2020salsanext,
  title={SalsaNext: Fast Semantic Segmentation of LiDAR Point Clouds for Autonomous Driving},
  author={Cortinhal, Tiago and Tzelepis, George and Aksoy, Eren Erdal},
  journal={arXiv preprint arXiv:2003.03653},
  year={2020}
}

@inproceedings{filos2019systematic,
	title={A Systematic Comparison of Bayesian Deep Learning Robustness in Diabetic Retinopathy Tasks},
	author={Filos, Angelos and Farquhar, Sebastian and Gomez, Aidan N and Rudner, Tim GJ and Kenton, Zachary and Smith, Lewis and Alizadeh, Milad and de Kroon, Arnoud and Gal, Yarin},
	booktitle={Workshop on Bayesian Deep Learning (NeurIPS 2019)},
	year={2019}
}


@article{shao2018crowdhuman,
  title={Crowdhuman: A benchmark for detecting human in a crowd},
  author={Shao, Shuai and Zhao, Zijian and Li, Boxun and Xiao, Tete and Yu, Gang and Zhang, Xiangyu and Sun, Jian},
  journal={arXiv preprint arXiv:1805.00123},
  year={2018}
}

%% Misc
@article{kesten2019lyft,
  title={{Lyft Level 5 AV Dataset 2019}},
  author={Kesten, R and Usman, M and Houston, J and Pandya, T and Nadhamuni, K and Ferreira, A and Yuan, M and Low, B and Jain, A and Ondruska, P and others},
  journal={https://level5.lyft.com/dataset},
  year={2019}
}

@misc{Detectron2018,
	author ={Ross Girshick and Ilija Radosavovic and Georgia Gkioxari and Piotr Doll\'{a}r and Kaiming He},
	title = {Detectron},
	howpublished = {\url{https://github.com/facebookresearch/detectron}},
	year ={2018}
}


%% PhD 
@PhdThesis{neal1995bayesian,
	title={Bayesian learning for neural networks},
	author={Neal, Radford M},
	year={1995},
	school={University of Toronto}
}

@PhdThesis{Gal2016Uncertainty,
	title={Uncertainty in Deep Learning},
	author={Gal, Yarin},
	year={2016},
	school={University of Cambridge}
}

@InProceedings{10.1007/978-3-031-20080-9_37,
author="Li, Ruoqi
and Zhang, Chongyang
and Zhou, Hao
and Shi, Chao
and Luo, Yan",
editor="Avidan, Shai
and Brostow, Gabriel
and Ciss{\'e}, Moustapha
and Farinella, Giovanni Maria
and Hassner, Tal",
title="Out-of-Distribution Identification: Let Detector Tell Which {I} Am Not Sure",
booktitle="Computer Vision -- Proceedings of ECCV 2022",
year="2022",
publisher="Springer Nature Switzerland",
address="Cham",
pages="638--654",
abstract="The superior performance of object detectors is often established under the condition that the test samples are in the same distribution as the training data. However, in most practical applications, out-of-distribution (OOD) instances are inevitable and usually lead to detection uncertainty. In this work, the Feature structured OOD-IDentification (FOOD-ID) model is proposed to reduce the uncertainty of detection results by identifying the OOD instances. Instead of outputting each detection result directly, FOOD-ID uses a likelihood-based measuring mechanism to identify whether the feature satisfies the corresponding class distribution and outputs the OOD results separately. Specifically, the clustering-oriented feature structuration is firstly developed using class-specified prototypes and Attractive-Repulsive loss for more discriminative feature representation and more compact distribution. With the structured features space, the density distribution of all training categories is estimated based on a class-conditional normalizing flow, which is then used for the OOD identification in the test stage. The proposed FOOD-ID can be easily applied to various object detectors including anchor-based frameworks and anchor-free frameworks. Extensive experiments on the PASCAL VOC-IO dataset and an industrial defect dataset demonstrate that FOOD-ID achieves satisfactory OOD identification performance, with which the certainty of detection results is improved significantly.",
isbn="978-3-031-20080-9"
}

@article{DBLP:journals/corr/abs-2107-12248,
  author    = {Christian Henning and
               Francesco D'Angelo and
               Benjamin F. Grewe},
  title     = {Are Bayesian neural networks intrinsically good at out-of-distribution
               detection?},
  journal   = {CoRR},
  volume    = {abs/2107.12248},
  year      = {2021},
  url       = {https://arxiv.org/abs/2107.12248},
  eprinttype = {arXiv},
  eprint    = {2107.12248},
  timestamp = {Fri, 30 Jul 2021 13:03:06 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-12248.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2110-04286,
  author    = {Lo{\"{\i}}c Le Folgoc and
               Vasileios Baltatzis and
               Sujal Desai and
               Anand Devaraj and
               Sam Ellis and
               Octavio E. Martinez Manzanera and
               Arjun Nair and
               Huaqi Qiu and
               Julia A. Schnabel and
               Ben Glocker},
  title     = {Is {MC} Dropout Bayesian?},
  journal   = {CoRR},
  volume    = {abs/2110.04286},
  year      = {2021},
  url       = {https://arxiv.org/abs/2110.04286},
  eprinttype = {arXiv},
  eprint    = {2110.04286},
  timestamp = {Thu, 21 Oct 2021 16:20:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2110-04286.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{Diffusion,
  
  url = {https://arxiv.org/abs/2211.07740},
  
  author = {Graham, Mark S. and Pinaya, Walter H. L. and Tudosiu, Petru-Daniel and Nachev, Parashkev and Ourselin, Sebastien and Cardoso, M. Jorge},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Denoising Diffusion Models for Out-of-Distribution Detection},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{DBLP:journals/ijcv/BlumSNSC21,
  author    = {Hermann Blum and
               Paul{-}Edouard Sarlin and
               Juan I. Nieto and
               Roland Siegwart and
               Cesar Cadena},
  title     = {The Fishyscapes Benchmark: Measuring Blind Spots in Semantic Segmentation},
  journal   = {Int. J. Comput. Vis.},
  volume    = {129},
  number    = {11},
  pages     = {3119--3135},
  year      = {2021},
  doi       = {10.1007/s11263-021-01511-6},
  timestamp = {Wed, 03 Nov 2021 08:27:59 +0100},
  biburl    = {https://dblp.org/rec/journals/ijcv/BlumSNSC21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/eccv/0002LG020,
  author    = {Hongjie Zhang and
               Ang Li and
               Jie Guo and
               Yanwen Guo},
  title     = {Hybrid Models for Open Set Recognition},
  booktitle = {16th European Conference on Computer Vision, {ECCV} 2020 },
  pages     = {102--117},

  year      = {2020},
  timestamp = {Tue, 09 Feb 2021 15:29:44 +0100},
  biburl    = {https://dblp.org/rec/conf/eccv/0002LG020.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:journals/corr/abs-2107-11264,
  author    = {Sanghun Jung and
               Jungsoo Lee and
               Daehoon Gwak and
               Sungha Choi and
               Jaegul Choo},
  title     = {Standardized Max Logits: {A} Simple yet Effective Approach for Identifying
               Unexpected Road Obstacles in Urban-Scene Segmentation},
    booktitle = {{IEEE} International Conference on Computer Vision, {ICCV}
               },
  year      = {2021},
  timestamp = {Thu, 14 Oct 2021 09:16:56 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-11264.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/visapp/GrcicBS21,
  author    = {Matej Grcic and
               Petra Bevandic and
               Sinisa Segvic},
  title     = {Dense Open-set Recognition with Synthetic Outliers Generated by Real
               {NVP}},
  booktitle = {Proceedings of the 16th International Joint Conference on Computer
               Vision, Imaging and Computer Graphics Theory and Applications, {VISIGRAPP}
               2021, Volume 4: VISAPP, Online Streaming, February 8-10, 2021},
  pages     = {133--143},
  publisher = {{SCITEPRESS}},
  year      = {2021},
  doi       = {10.5220/0010260701330143},
  timestamp = {Tue, 02 Mar 2021 16:20:23 +0100},
  biburl    = {https://dblp.org/rec/conf/visapp/GrcicBS21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2108-09976,
  author    = {Zhilin Zhao and
               Longbing Cao and
               Kun{-}Yu Lin},
  title     = {Revealing Distributional Vulnerability of Explicit Discriminators
               by Implicit Generators},
  journal   = {CoRR},
  volume    = {abs/2108.09976},
  eprinttype = {arXiv},
  eprint    = {2108.09976},
  timestamp = {Wed, 10 Nov 2021 12:34:13 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2108-09976.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/NguyenYC15,
  author    = {Anh Mai Nguyen and
               Jason Yosinski and
               Jeff Clune},
  title     = {Deep neural networks are easily fooled: High confidence predictions
               for unrecognizable images},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, CVPR
               2015, Boston, MA, USA, June 7-12, 2015},
  pages     = {427--436},
  publisher = {{IEEE} Computer Society},
  year      = {2015},
  url       = {https://doi.org/10.1109/CVPR.2015.7298640},
  doi       = {10.1109/CVPR.2015.7298640},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/NguyenYC15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2010-05119,
  author    = {Ad{\'{\i}}n Ram{\'{\i}}rez Rivera and
               Adil Khan and
               Imad Eddine Ibrahim Bekkouch and
               Taimoor Shakeel Sheikh},
  title     = {Anomaly Detection based on Zero-Shot Outlier Synthesis and Hierarchical
               Feature Distillation},
  journal   = {CoRR},
  volume    = {abs/2010.05119},
  year      = {2020},
  url       = {https://arxiv.org/abs/2010.05119},
  archivePrefix = {arXiv},
  eprint    = {2010.05119},
  timestamp = {Tue, 20 Oct 2020 15:08:10 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2010-05119.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/ijcv/EveringhamGWWZ10,
  author    = {Mark Everingham and
               Luc Van Gool and
               Christopher K. I. Williams and
               John M. Winn and
               Andrew Zisserman},
  title     = {The Pascal Visual Object Classes {(VOC)} Challenge},
  journal   = {International Journal of Computer Vision},
  volume    = {88},
  number    = {2},
  pages     = {303--338},
  year      = {2010}
}
@inproceedings{DBLP:conf/icml/TanL19,
  author    = {Mingxing Tan and
               Quoc V. Le},
  editor    = {Kamalika Chaudhuri and
               Ruslan Salakhutdinov},
  title     = {EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks},
  booktitle = {Proceedings of the 36th International Conference on Machine Learning,
               {ICML} 2019},
  series    = {Proceedings of Machine Learning Research},
  volume    = {97},
  pages     = {6105--6114},
  year      = {2019}
}
@inproceedings{DBLP:conf/cvpr/RadosavovicKGHD20,
  author    = {Ilija Radosavovic and
               Raj Prateek Kosaraju and
               Ross B. Girshick and
               Kaiming He and
               Piotr Doll{\'{a}}r},
  title     = {Designing Network Design Spaces},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               CVPR 2020},
  pages     = {10425--10433},
  year      = {2020}
}
@inproceedings{DBLP:journals/corr/abs-2103-02603,
  author    = {K. J. Joseph and
               Salman Khan and
               Fahad Shahbaz Khan and
               Vineeth N. Balasubramanian},
  title     = {Towards Open World Object Detection},
  booktitle = {{IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               CVPR 2021},
  year      = {2021}
}

@article{DBLP:journals/corr/abs-1802-03426,
  author    = {Leland McInnes and
               John Healy},
  title     = {{UMAP:} Uniform Manifold Approximation and Projection for Dimension
               Reduction},
  journal   = {CoRR},
  volume    = {abs/1802.03426},
  year      = {2018},
  url       = {http://arxiv.org/abs/1802.03426},
  archivePrefix = {arXiv},
  eprint    = {1802.03426},
  timestamp = {Tue, 17 Sep 2019 14:15:10 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1802-03426.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/pami/RenHG017,
  author    = {Shaoqing Ren and
               Kaiming He and
               Ross B. Girshick and
               Jian Sun},
  title     = {Faster {R-CNN:} Towards Real-Time Object Detection with Region Proposal
               Networks},
  journal   = {{IEEE} Transactions Pattern Analysis and Machine Intelligence.},
  volume    = {39},
  number    = {6},
  pages     = {1137--1149},
  year      = {2017},
  timestamp = {Wed, 14 Nov 2018 10:51:18 +0100},
  biburl    = {https://dblp.org/rec/journals/pami/RenHG017.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/ZhangCDL18,
  author    = {Hongyi Zhang and
               Moustapha Ciss{\'{e}} and
               Yann N. Dauphin and
               David Lopez{-}Paz},
  title     = {mixup: Beyond Empirical Risk Minimization},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018},
  year      = {2018},
  timestamp = {Thu, 25 Jul 2019 14:25:50 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/ZhangCDL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2007-06096,
  author    = {Th{\'{e}}o Gu{\'{e}}nais and
               Dimitris Vamvourellis and
               Yaniv Yacoby and
               Finale Doshi{-}Velez and
               Weiwei Pan},
  title     = {BaCOUn: Bayesian Classifers with Out-of-Distribution Uncertainty},
  journal={arXiv preprint arXiv:2007.06096},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.06096},
  archivePrefix = {arXiv},
  eprint    = {2007.06096},
  timestamp = {Wed, 22 Jul 2020 12:09:15 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-06096.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-1910-04241,
   author    = {Sachin Vernekar and
               Ashish Gaurav and
               Vahdat Abdelzad and
               Taylor Denouden and
               Rick Salay and
               Krzysztof Czarnecki},
  title     = {Out-of-distribution Detection in Classifiers via Generation},
  journal={arXiv preprint arXiv:1910.04241},
  year={2019}
}
@inproceedings{DBLP:conf/iclr/LeeLLS18,
  author    = {Kimin Lee and
               Honglak Lee and
               Kibok Lee and
               Jinwoo Shin},
  title     = {Training Confidence-calibrated Classifiers for Detecting Out-of-Distribution
               Samples},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  timestamp = {Thu, 25 Jul 2019 14:25:57 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LeeLLS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@misc{chen2020informative,
    title={Informative Outlier Matters: Robustifying Out-of-distribution Detection Using Outlier Mining},
    author={Jiefeng Chen and Yixuan Li and Xi Wu and Yingyu Liang and Somesh Jha},
    year={2020},
    eprint={2006.15207},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
@inproceedings{DBLP:conf/iclr/HendrycksMD19,
  author    = {Dan Hendrycks and
               Mantas Mazeika and
               Thomas G. Dietterich},
  title     = {Deep Anomaly Detection with Outlier Exposure},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  url       = {https://openreview.net/forum?id=HyxCxhRcY7},
  timestamp = {Thu, 25 Jul 2019 14:25:52 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/HendrycksMD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/eccv/LinMBHPRDZ14,
  author    = {Tsung{-}Yi Lin and
               Michael Maire and
               Serge J. Belongie and
               James Hays and
               Pietro Perona and
               Deva Ramanan and
               Piotr Doll{\'{a}}r and
               C. Lawrence Zitnick},
  editor    = {David J. Fleet and
               Tom{\'{a}}s Pajdla and
               Bernt Schiele and
               Tinne Tuytelaars},
  title     = {Microsoft {COCO:} Common Objects in Context},
  booktitle = {Computer Vision - {ECCV} 2014 - 13th European Conference, Zurich,
               Switzerland, September 6-12, 2014, Proceedings, Part {V}},
  series    = {Lecture Notes in Computer Science},
  volume    = {8693},
  pages     = {740--755},
  publisher = {Springer},
  year      = {2014},
  url       = {https://doi.org/10.1007/978-3-319-10602-1\_48},
  doi       = {10.1007/978-3-319-10602-1\_48},
  timestamp = {Tue, 14 May 2019 10:00:45 +0200},
  biburl    = {https://dblp.org/rec/conf/eccv/LinMBHPRDZ14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/ijcv/KuznetsovaRAUKP20,
  author    = {Alina Kuznetsova and
               Hassan Rom and
               Neil Alldrin and
               Jasper R. R. Uijlings and
               Ivan Krasin and
               Jordi Pont{-}Tuset and
               Shahab Kamali and
               Stefan Popov and
               Matteo Malloci and
               Alexander Kolesnikov and
               Tom Duerig and
               Vittorio Ferrari},
  title     = {The Open Images Dataset {V4}},
  journal   = {Int. J. Comput. Vis.},
  volume    = {128},
  number    = {7},
  pages     = {1956--1981},
  year      = {2020},
  url       = {https://doi.org/10.1007/s11263-020-01316-z},
  doi       = {10.1007/s11263-020-01316-z},
  timestamp = {Fri, 20 Nov 2020 14:04:06 +0100},
  biburl    = {https://dblp.org/rec/journals/ijcv/KuznetsovaRAUKP20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/YuCWXCLMD20,
  author    = {Fisher Yu and
               Haofeng Chen and
               Xin Wang and
               Wenqi Xian and
               Yingying Chen and
               Fangchen Liu and
               Vashisht Madhavan and
               Trevor Darrell},
  title     = {{BDD100K:} {A} Diverse Driving Dataset for Heterogeneous Multitask
               Learning},
  booktitle = {{IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               CVPR 2020},
  pages     = {2633--2642},
  year      = {2020}
}
@article{DBLP:journals/pami/LinGGHD20,
  author    = {Tsung{-}Yi Lin and
               Priya Goyal and
               Ross B. Girshick and
               Kaiming He and
               Piotr Doll{\'{a}}r},
  title     = {Focal Loss for Dense Object Detection},
  journal   = {{IEEE} Trans. Pattern Anal. Mach. Intell.},
  volume    = {42},
  number    = {2},
  pages     = {318--327},
  year      = {2020},
  url       = {https://doi.org/10.1109/TPAMI.2018.2858826},
  doi       = {10.1109/TPAMI.2018.2858826},
  timestamp = {Sat, 30 May 2020 20:02:13 +0200},
  biburl    = {https://dblp.org/rec/journals/pami/LinGGHD20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1804-02748,
  author    = {Dima Damen and
               Hazel Doughty and
               Giovanni Maria Farinella and
               Sanja Fidler and
               Antonino Furnari and
               Evangelos Kazakos and
               Davide Moltisanti and
               Jonathan Munro and
               Toby Perrett and
               Will Price and
               Michael Wray},
  title     = {Scaling Egocentric Vision: The {EPIC-KITCHENS} Dataset},
  journal   = {CoRR},
  volume    = {abs/1804.02748},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.02748},
  archivePrefix = {arXiv},
  eprint    = {1804.02748},
  timestamp = {Sat, 23 Jan 2021 01:20:26 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1804-02748.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/GkioxariGDH18,
  author    = {Georgia Gkioxari and
               Ross B. Girshick and
               Piotr Doll{\'{a}}r and
               Kaiming He},
  title     = {Detecting and Recognizing Human-Object Interactions},
  booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
               CVPR 2018, Salt Lake City, UT, USA, June 18-22, 2018},
  pages     = {8359--8367},
  publisher = {{IEEE} Computer Society},
  year      = {2018},
  url       = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Gkioxari\_Detecting\_and\_Recognizing\_CVPR\_2018\_paper.html},
  doi       = {10.1109/CVPR.2018.00872},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/GkioxariGDH18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iccv/ZhangH17,
  author    = {Haoyang Zhang and
               Xuming He},
  title     = {Deep Free-Form Deformation Network for Object-Mask Registration},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017, Venice,
               Italy, October 22-29, 2017},
  pages     = {4261--4269},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {http://doi.ieeecomputersociety.org/10.1109/ICCV.2017.456},
  doi       = {10.1109/ICCV.2017.456},
  timestamp = {Wed, 23 Dec 2020 08:54:04 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/ZhangH17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/PhilbinCISZ07,
  author    = {James Philbin and
               Ondrej Chum and
               Michael Isard and
               Josef Sivic and
               Andrew Zisserman},
  title     = {Object retrieval with large vocabularies and fast spatial matching},
  booktitle = {2007 {IEEE} Computer Society Conference on Computer Vision and Pattern
               Recognition {(CVPR} 2007), 18-23 June 2007, Minneapolis, Minnesota,
               {USA}},
  publisher = {{IEEE} Computer Society},
  year      = {2007},
  url       = {https://doi.org/10.1109/CVPR.2007.383172},
  doi       = {10.1109/CVPR.2007.383172},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/PhilbinCISZ07.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/tmm/MengYYWT16,
  author    = {Jingjing Meng and
               Junsong Yuan and
               Jiong Yang and
               Gang Wang and
               Yap{-}Peng Tan},
  title     = {Object Instance Search in Videos via Spatio-Temporal Trajectory Discovery},
  journal   = {{IEEE} Trans. Multim.},
  volume    = {18},
  number    = {1},
  pages     = {116--127},
  year      = {2016},
  url       = {https://doi.org/10.1109/TMM.2015.2500734},
  doi       = {10.1109/TMM.2015.2500734},
  timestamp = {Thu, 01 Oct 2020 10:57:38 +0200},
  biburl    = {https://dblp.org/rec/journals/tmm/MengYYWT16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/nips/LiuWOL20,
  author    = {Weitang Liu and
               Xiaoyun Wang and
               John D. Owens and
               Yixuan Li},
  editor    = {Hugo Larochelle and
               Marc'Aurelio Ranzato and
               Raia Hadsell and
               Maria{-}Florina Balcan and
               Hsuan{-}Tien Lin},
  title     = {Energy-based Out-of-distribution Detection},
  booktitle = NIPS,
  year      = {2020},
  url       = {https://proceedings.neurips.cc/paper/2020/hash/f5496252609c43eb8a3d147ab9b9c006-Abstract.html},
  timestamp = {Tue, 19 Jan 2021 15:57:41 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/LiuWOL20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/cvpr/HsuSJK20,
  author    = {Yen{-}Chang Hsu and
               Yilin Shen and
               Hongxia Jin and
               Zsolt Kira},
  title     = {Generalized {ODIN:} Detecting Out-of-Distribution Image Without Learning
               From Out-of-Distribution Data},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               CVPR 2020, Seattle, WA, USA, June 13-19, 2020},
  pages     = {10948--10957},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/CVPR42600.2020.01096},
  doi       = {10.1109/CVPR42600.2020.01096},
  timestamp = {Tue, 11 Aug 2020 16:59:49 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/HsuSJK20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/nips/LeeLLS18,
  author    = {Kimin Lee and
               Kibok Lee and
               Honglak Lee and
               Jinwoo Shin},
  editor    = {Samy Bengio and
               Hanna M. Wallach and
               Hugo Larochelle and
               Kristen Grauman and
               Nicol{\`{o}} Cesa{-}Bianchi and
               Roman Garnett},
  title     = {A Simple Unified Framework for Detecting Out-of-Distribution Samples
               and Adversarial Attacks},
  booktitle = {NIPS 31: Annual Conference
               on Neural Information Processing Systems 2018, NeurIPS 2018, December
               3-8, 2018, Montr{\'{e}}al, Canada},
  pages     = {7167--7177},
  year      = {2018},
  url       = {https://proceedings.neurips.cc/paper/2018/hash/abdeb6f575ac5c6676b747bca8d09cc2-Abstract.html},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/LeeLLS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/pami/ZhouLKO018,
  author    = {Bolei Zhou and
               {\`{A}}gata Lapedriza and
               Aditya Khosla and
               Aude Oliva and
               Antonio Torralba},
  title     = {Places: {A} 10 Million Image Database for Scene Recognition},
  journal   = {{IEEE} Transactions Pattern Analysis and Machine Intelligence.},
  volume    = {40},
  number    = {6},
  pages     = {1452--1464},
  year      = {2018},
  doi       = {10.1109/TPAMI.2017.2723009},
  timestamp = {Wed, 14 Nov 2018 10:51:18 +0100},
  biburl    = {https://dblp.org/rec/journals/pami/ZhouLKO018.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/HendrycksD19,
  author    = {Dan Hendrycks and
               Thomas G. Dietterich},
  title     = {Benchmarking Neural Network Robustness to Common Corruptions and Perturbations},
  booktitle = { International Conference on Learning Representations, {ICLR} 2019},
  year      = {2019},
  url       = {https://openreview.net/forum?id=HJz6tiCqYm},
  timestamp = {Thu, 25 Jul 2019 14:25:46 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/HendrycksD19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1906-03509,
  author    = {Aristotelis{-}Angelos Papadopoulos and
               Mohammad Reza Rajati},
  title     = {Simultaneous Classification and Novelty Detection Using Deep Neural
               Networks},
  journal={arXiv preprint arXiv:1906.03509},
  year={2019}
}
@inproceedings{DBLP:journals/corr/KingmaB14,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  title     = {Adam: {A} Method for Stochastic Optimization},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015},
  year      = {2015},
  timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2106-03917,
  author    = {Jingyang Zhang and
               Nathan Inkawhich and
               Yiran Chen and
               Hai Li},
  title     = {Fine-grained Out-of-Distribution Detection with Mixup Outlier Exposure},
  journal   = {CoRR},
  volume    = {abs/2106.03917},
  year      = {2021},
  eprinttype = {arXiv},
  eprint    = {2106.03917},
  timestamp = {Thu, 10 Jun 2021 16:34:18 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2106-03917.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{bendale2016towards,
  title={Towards open set deep networks},
  author={Bendale, Abhijit and Boult, Terrance E},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1563--1572},
  year={2016}
}


@inproceedings{DBLP:conf/icml/SastryO20,
  author    = {Chandramouli Shama Sastry and
               Sageev Oore},
  title     = {Detecting Out-of-Distribution Examples with Gram Matrices},
  booktitle = {Proceedings of the 37th International Conference on Machine Learning,
               {ICML} 2020},
  volume    = {119},
  pages     = {8491--8501},
  year      = {2020},
  timestamp = {Tue, 15 Dec 2020 17:40:19 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/SastryO20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{netzer2011reading,
  title={Reading digits in natural images with unsupervised feature learning},
  author={Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y},
  year={2011},
  booktitle = {Proc. of NIPS Workshop on Deep Learning and Unsupervised Feature Learning, 2011}
}

@inproceedings{DBLP:conf/cvpr/CimpoiMKMV14,
  author    = {Mircea Cimpoi and
               Subhransu Maji and
               Iasonas Kokkinos and
               Sammy Mohamed and
               Andrea Vedaldi},
  title     = {Describing Textures in the Wild},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition,
               CVPR 2014},
  pages     = {3606--3613},
  year      = {2014}
}

@article{DBLP:journals/corr/abs-2003-08798,
  author    = {K. J. Joseph and
               Jathushan Rajasegaran and
               Salman H. Khan and
               Fahad Shahbaz Khan and
               Vineeth Balasubramanian and
               Ling Shao},
  title     = {Incremental Object Detection via Meta-Learning},
  journal={arXiv preprint arXiv:2003.08798},
  year={2020}
}
@inproceedings{DBLP:conf/cvpr/Perez-RuaZHX20,
  author    = {Juan{-}Manuel P{\'{e}}rez{-}R{\'{u}}a and
               Xiatian Zhu and
               Timothy M. Hospedales and
               Tao Xiang},
  title     = {Incremental Few-Shot Object Detection},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               CVPR 2020},
  pages     = {13843--13852},
  year      = {2020},
  doi       = {10.1109/CVPR42600.2020.01386},
  timestamp = {Tue, 11 Aug 2020 16:59:49 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/Perez-RuaZHX20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{cifar,
  author    = {Alex Krizhevsky and Geoffrey Hinton},
 title     = {Learning multiple layers of
features from tiny images},
volume={Technical Report},
  year      = {2009}
}
@inproceedings{DBLP:conf/bmvc/ZagoruykoK16,
  author    = {Sergey Zagoruyko and
               Nikos Komodakis},
  editor    = {Richard C. Wilson and
               Edwin R. Hancock and
               William A. P. Smith},
  title     = {Wide Residual Networks},
  booktitle = {Proceedings of the British Machine Vision Conference 2016, {BMVC}
               2016, York, UK, September 19-22, 2016},
  publisher = {{BMVA} Press},
  year      = {2016},
  url       = {http://www.bmva.org/bmvc/2016/papers/paper087/index.html},
  timestamp = {Wed, 03 Feb 2021 08:36:18 +0100},
  biburl    = {https://dblp.org/rec/conf/bmvc/ZagoruykoK16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iccv/ShmelkovSA17,
  author    = {Konstantin Shmelkov and
               Cordelia Schmid and
               Karteek Alahari},
  title     = {Incremental Learning of Object Detectors without Catastrophic Forgetting},
  booktitle = {{IEEE} International Conference on Computer Vision, {ICCV} 2017},
  pages     = {3420--3429},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICCV.2017.368},
  doi       = {10.1109/ICCV.2017.368},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iccv/ShmelkovSA17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/accv/RahmanKP18,
  author    = {Shafin Rahman and
               Salman H. Khan and
               Fatih Porikli},
  title     = {Zero-Shot Object Detection: Learning to Simultaneously Recognize and
               Localize Novel Concepts},
  booktitle = {Asian Conference on Computer
               Vision 2018},
  volume    = {11361},
  pages     = {547--563},
  year      = {2018},
  doi       = {10.1007/978-3-030-20887-5\_34},
  timestamp = {Mon, 03 Jun 2019 16:21:27 +0200},
  biburl    = {https://dblp.org/rec/conf/accv/RahmanKP18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/aaai/LiYZ0KZ19,
  author    = {Zhihui Li and
               Lina Yao and
               Xiaoqin Zhang and
               Xianzhi Wang and
               Salil S. Kanhere and
               Huaxiang Zhang},
  title     = {Zero-Shot Object Detection with Textual Descriptions},
  booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
               2019},
  pages     = {8690--8697},
  year      = {2019}
}
@article{DBLP:journals/ijcv/RahmanKP20,
  author    = {Shafin Rahman and
               Salman H. Khan and
               Fatih Porikli},
  title     = {Zero-Shot Object Detection: Joint Recognition and Localization of
               Novel Concepts},
  journal   = {International Journal of Computer Vision},
  volume    = {128},
  number    = {12},
  pages     = {2979--2999},
  year      = {2020},
  doi       = {10.1007/s11263-020-01355-6},
  timestamp = {Tue, 06 Oct 2020 17:44:10 +0200},
  biburl    = {https://dblp.org/rec/journals/ijcv/RahmanKP20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/wacv/0003DSZMCCAS20,
  author    = {David Hall and
               Feras Dayoub and
               John Skinner and
               Haoyang Zhang and
               Dimity Miller and
               Peter Corke and
               Gustavo Carneiro and
               Anelia Angelova and
               Niko S{\"{u}}nderhauf},
  title     = {Probabilistic Object Detection: Definition and Evaluation},
  booktitle = {{IEEE} Winter Conference on Applications of Computer Vision, {WACV}
               2020},
  pages     = {1020--1029},
  year      = {2020},
  timestamp = {Fri, 09 Apr 2021 18:46:49 +0200},
  biburl    = {https://dblp.org/rec/conf/wacv/0003DSZMCCAS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icra/MillerDMS19,
  author    = {Dimity Miller and
               Feras Dayoub and
               Michael Milford and
               Niko S{\"{u}}nderhauf},
  title     = {Evaluating Merging Strategies for Sampling-based Uncertainty Techniques
               in Object Detection},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019},
  pages     = {2348--2354},
  year      = {2019},
  timestamp = {Mon, 15 Jun 2020 17:08:48 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/MillerDMS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/icra/MillerNDS18,
  author    = {Dimity Miller and
               Lachlan Nicholson and
               Feras Dayoub and
               Niko S{\"{u}}nderhauf},
  title     = {Dropout Sampling for Robust Object Detection in Open-Set Conditions},
  booktitle = {{IEEE} International Conference on Robotics and Automation, {ICRA}
               2018},
  pages     = {1--7},
  year      = {2018},
  doi       = {10.1109/ICRA.2018.8460700},
  timestamp = {Fri, 27 Mar 2020 08:57:10 +0100},
  biburl    = {https://dblp.org/rec/conf/icra/MillerNDS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/corr/abs-2104-01328,
  author    = {Dimity Miller and
               Niko S{\"{u}}nderhauf and
               Michael Milford and
               Feras Dayoub},
  title     = {Uncertainty for Identifying Open-Set Errors in Visual Object Detection},
  journal={arXiv preprint arXiv:2104.01328},
  year={2021}
}
@inproceedings{DBLP:conf/wacv/DhamijaGVB20,
  author    = {Akshay Raj Dhamija and
               Manuel G{\"{u}}nther and
               Jonathan Ventura and
               Terrance E. Boult},
  title     = {The Overlooked Elephant of Object Detection: Open Set},
  booktitle = {{IEEE} Winter Conference on Applications of Computer Vision, {WACV}
               2020},
  pages     = {1010--1019},
  year      = {2020}
}
@inproceedings{DBLP:journals/corr/abs-2101-05036,
  title={Estimating and Evaluating Regression Predictive Uncertainty in Deep
               Object Detectors},
    author    = {Ali Harakeh and
               Steven L. Waslander},
  booktitle={International Conference on Learning Representations},
  year={2021}
}
@inproceedings{DBLP:conf/nips/Lakshminarayanan17,
  author    = {Balaji Lakshminarayanan and
               Alexander Pritzel and
               Charles Blundell},
  title     = {Simple and Scalable Predictive Uncertainty Estimation using Deep Ensembles},
  booktitle = NIPS,
  pages     = {6402--6413},
  year      = {2017},
}

@inproceedings{DBLP:conf/iclr/SerraAGSNL20,
  author    = {Joan Serr{\`{a}} and
               David {\'{A}}lvarez and
               Vicen{\c{c}} G{\'{o}}mez and
               Olga Slizovskaia and
               Jos{\'{e}} F. N{\'{u}}{\~{n}}ez and
               Jordi Luque},
  title     = {Input Complexity and Out-of-distribution Detection with Likelihood-based
               Generative Models},
  booktitle = {Proceedings of the International Conference on Learning Representations, {ICLR} 2020
               },
  year      = {2020},
  timestamp = {Thu, 18 Jun 2020 15:43:42 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/SerraAGSNL20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/nips/KingmaD18,
  author    = {Diederik P. Kingma and
               Prafulla Dhariwal},
  title     = {Glow: Generative Flow with Invertible 1x1 Convolutions},
  booktitle = {NIPS 2018, NeurIPS 2018},
  pages     = {10236--10245},
  year      = {2018},
  timestamp = {Thu, 21 Jan 2021 15:15:21 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/KingmaD18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/GrathwohlWJD0S20,
  author    = {Will Grathwohl and
               Kuan{-}Chieh Wang and
               J{\"{o}}rn{-}Henrik Jacobsen and
               David Duvenaud and
               Mohammad Norouzi and
               Kevin Swersky},
  title     = {Your classifier is secretly an energy based model and you should treat
               it like one},
  booktitle = {International Conference on Learning Representations, {ICLR} 2020},
  year      = {2020}
}

@inproceedings{DBLP:journals/corr/abs-1903-08689,
  author    = {Yilun Du and
               Igor Mordatch},
  title     = {Implicit Generation and Modeling with Energy Based Models},
  booktitle = {NIPS 2019, NeurIPS 2019},
  pages     = {3603--3613},
  year      = {2019}
}
@inproceedings{DBLP:conf/icml/GalG16,
  author    = {Yarin Gal and
               Zoubin Ghahramani},
  editor    = {Maria{-}Florina Balcan and
               Kilian Q. Weinberger},
  title     = {Dropout as a Bayesian Approximation: Representing Model Uncertainty
               in Deep Learning},
  booktitle = {Proceedings of the 33nd International Conference on Machine Learning,
               {ICML} 2016, New York City, NY, USA, June 19-24, 2016},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {48},
  pages     = {1050--1059},
  publisher = {JMLR.org},
  year      = {2016},
  url       = {http://proceedings.mlr.press/v48/gal16.html},
  timestamp = {Wed, 29 May 2019 08:41:46 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/GalG16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/cvpr/HuangLMW17,
  author    = {Gao Huang and
               Zhuang Liu and
               Laurens van der Maaten and
               Kilian Q. Weinberger},
  title     = {Densely Connected Convolutional Networks},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               CVPR 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {2261--2269},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.243},
  doi       = {10.1109/CVPR.2017.243},
  timestamp = {Wed, 16 Oct 2019 14:14:50 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/HuangLMW17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/NalisnickMTGL19,
  author    = {Eric T. Nalisnick and
               Akihiro Matsukawa and
               Yee Whye Teh and
               Dilan G{\"{o}}r{\"{u}}r and
               Balaji Lakshminarayanan},
  title     = {Do Deep Generative Models Know What They Don't Know?},
  booktitle = {International Conference on Learning Representations, {ICLR} 2019
               },
  year      = {2019},
  timestamp = {Thu, 25 Jul 2019 14:25:59 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/NalisnickMTGL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/HinzHW19,
  author    = {Tobias Hinz and
               Stefan Heinrich and
               Stefan Wermter},
  title     = {Generating Multiple Objects at Spatially Distinct Locations},
  booktitle = {International Conference on Learning Representations, {ICLR} 2019},
  year      = {2019},
  timestamp = {Thu, 25 Jul 2019 14:25:42 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/HinzHW19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{choi2018waic,
  title={Waic, but why? generative ensembles for robust anomaly detection},
  author={Choi, Hyunsun and Jang, Eric and Alemi, Alexander A},
  journal={arXiv preprint arXiv:1810.01392},
  year={2018}
}

@inproceedings{DBLP:conf/nips/RenLFSPDDL19,
  author    = {Jie Ren and
               Peter J. Liu and
               Emily Fertig and
               Jasper Snoek and
               Ryan Poplin and
               Mark A. DePristo and
               Joshua V. Dillon and
               Balaji Lakshminarayanan},
  title     = {Likelihood Ratios for Out-of-Distribution Detection},
  booktitle = {NIPS 2019, NeurIPS 2019},
  pages     = {14680--14691},
  year      = {2019},
  timestamp = {Thu, 21 Jan 2021 15:15:20 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/RenLFSPDDL19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/RiquelmeTS18,
  author    = {Carlos Riquelme and
               George Tucker and
               Jasper Snoek},
  title     = {Deep Bayesian Bandits Showdown: An Empirical Comparison of Bayesian
               Deep Networks for Thompson Sampling},
  booktitle = {International Conference on Learning Representations, {ICLR} 2018
               },
  year      = {2018},
  url       = {https://openreview.net/forum?id=SyYe6k-CW},
  timestamp = {Thu, 25 Jul 2019 14:25:48 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/RiquelmeTS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/aaai/MohseniPYW20,
  author    = {Sina Mohseni and
               Mandar Pitale and
               J. B. S. Yadawa and
               Zhangyang Wang},
  title     = {Self-Supervised Learning for Generalizable Out-of-Distribution Detection},
  booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
               2020, The Thirty-Second Innovative Applications of Artificial Intelligence
               Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
               Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
               February 7-12, 2020},
  pages     = {5216--5223},
  publisher = {{AAAI} Press},
  year      = {2020},
  url       = {https://aaai.org/ojs/index.php/AAAI/article/view/5966},
  timestamp = {Tue, 02 Feb 2021 08:01:02 +0100},
  biburl    = {https://dblp.org/rec/conf/aaai/MohseniPYW20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/nips/HendrycksMKS19,
  author    = {Dan Hendrycks and
               Mantas Mazeika and
               Saurav Kadavath and
               Dawn Song},
  title     = {Using Self-Supervised Learning Can Improve Model Robustness and Uncertainty},
  booktitle = {NIPS 2019, NeurIPS 2019},
  pages     = {15637--15648},
  year      = {2019}
}
@inproceedings{DBLP:conf/cvpr/0001AB19,
  author    = {Matthias Hein and
               Maksym Andriushchenko and
               Julian Bitterwolf},
  title     = {Why ReLU Networks Yield High-Confidence Predictions Far Away From
               the Training Data and How to Mitigate the Problem},
  booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, CVPR
               2019, Long Beach, CA, USA, June 16-20, 2019},
  pages     = {41--50},
  publisher = {Computer Vision Foundation / {IEEE}},
  year      = {2019},
  url       = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Hein\_Why\_ReLU\_Networks\_Yield\_High-Confidence\_Predictions\_Far\_Away\_From\_the\_CVPR\_2019\_paper.html},
  doi       = {10.1109/CVPR.2019.00013},
  timestamp = {Thu, 27 Aug 2020 07:31:34 +0200},
  biburl    = {https://dblp.org/rec/conf/cvpr/0001AB19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/LiangLS18,
  author    = {Shiyu Liang and
               Yixuan Li and
               R. Srikant},
  title     = {Enhancing The Reliability of Out-of-distribution Image Detection in
               Neural Networks},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  url       = {https://openreview.net/forum?id=H1VGkIxRZ},
  timestamp = {Thu, 22 Aug 2019 13:48:13 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LiangLS18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{DBLP:conf/iclr/HendrycksG17,
  author    = {Dan Hendrycks and
               Kevin Gimpel},
  title     = {A Baseline for Detecting Misclassified and Out-of-Distribution Examples
               in Neural Networks},
  booktitle = {5th International Conference on Learning Representations,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/forum?id=Hkg4TI9xl},
  timestamp = {Thu, 25 Jul 2019 14:25:55 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/HendrycksG17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icml/FilosTMRLG20,
  author    = {Angelos Filos and
               Panagiotis Tigas and
               Rowan McAllister and
               Nicholas Rhinehart and
               Sergey Levine and
               Yarin Gal},
  title     = {Can Autonomous Vehicles Identify, Recover From, and Adapt to Distribution
               Shifts?},
  booktitle = {Proceedings of the 37th International Conference on Machine Learning,
               {ICML} 2020, 13-18 July 2020, Virtual Event},
  series    = {Proceedings of Machine Learning Research},
  volume    = {119},
  pages     = {3145--3153},
  publisher = {{PMLR}},
  year      = {2020},
  url       = {http://proceedings.mlr.press/v119/filos20a.html},
  timestamp = {Fri, 05 Feb 2021 11:08:07 +0100},
  biburl    = {https://dblp.org/rec/conf/icml/FilosTMRLG20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-2007-04250,
  author    = {Tianshi Cao and
               Chinwei Huang and
               David Yu{-}Tung Hui and
               Joseph Paul Cohen},
  title     = {A Benchmark of Medical Out of Distribution Detection},
  journal   = {CoRR},
  volume    = {abs/2007.04250},
  year      = {2020},
  url       = {https://arxiv.org/abs/2007.04250},
  archivePrefix = {arXiv},
  eprint    = {2007.04250},
  timestamp = {Mon, 20 Jul 2020 14:20:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2007-04250.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{chen2020,
    title={Informative Outlier Matters: Robustifying Out-of-distribution Detection Using Outlier Mining},
    author={Chen, Jiefeng and Li, Yixuan and Wu, Xi and Liang, Yingyu and Jha, Somesh},
    booktitle={arXiv preprint arXiv:2006.15207},
    year={2020}
}

@inproceedings{mohseni2020self,
  title={Self-supervised learning for generalizable out-of-distribution detection},
  author={Mohseni, Sina and Pitale, Mandar and Yadawa, JBS and Wang, Zhangyang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={04},
  pages={5216--5223},
  year={2020}
}

@inproceedings{lee2020gradients,
  title={Gradients as a Measure of Uncertainty in Neural Networks},
  author={Lee, Jinsol and AlRegib, Ghassan},
  booktitle={2020 IEEE International Conference on Image Processing (ICIP)},
  pages={2416--2420},
  year={2020},
  organization={IEEE}
}

@inproceedings{zhou2016cvpr,
    author    = {Zhou, Bolei and Khosla, Aditya and Lapedriza, Agata and Oliva, Aude and Torralba, Antonio},
    title     = {Learning Deep Features for Discriminative Localization},
    booktitle = {Computer Vision and Pattern Recognition},
    year      = {2016}
}

@inproceedings{irvin2019chexpert,
  title={Chexpert: A large chest radiograph dataset with uncertainty labels and expert comparison},
  author={Irvin, Jeremy and Rajpurkar, Pranav and Ko, Michael and Yu, Yifan and Ciurea-Ilcus, Silviana and Chute, Chris and Marklund, Henrik and Haghgoo, Behzad and Ball, Robyn and Shpanskaya, Katie and others},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={590--597},
  year={2019}
}

@article{rajpurkar2017chexnet,
  title={Chexnet: Radiologist-level pneumonia detection on chest x-rays with deep learning},
  author={Rajpurkar, Pranav and Irvin, Jeremy and Zhu, Kaylie and Yang, Brandon and Mehta, Hershel and Duan, Tony and Ding, Daisy and Bagul, Aarti and Langlotz, Curtis and Shpanskaya, Katie and others},
  journal={arXiv preprint arXiv:1711.05225},
  year={2017}
}

@inproceedings{goodfellow2014explaining,
  author    = {Ian J. Goodfellow and
               Jonathon Shlens and
               Christian Szegedy},
  title     = {Explaining and Harnessing Adversarial Examples},
  booktitle = {International Conference on Learning Representations, {ICLR} 2015},
  year      = {2015},
}

@inproceedings{lee2018training,
  title={Training Confidence-calibrated Classifiers for Detecting Out-of-Distribution Samples},
  author={Lee, Kimin and Lee, Honglak and Lee, Kibok and Shin, Jinwoo},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@misc{papadopoulos2020,
    title={Outlier Exposure with Confidence Control for Out-of-Distribution Detection}, 
    author={Aristotelis-Angelos Papadopoulos and Mohammad Reza Rajati and Nazim Shaikh and Jiamian Wang},
    year={2020},
    eprint={1906.03509},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@inproceedings{kingma2014autoencoding,
  author    = {Diederik P. Kingma and
               Max Welling},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014},
  year      = {2014},
}

@inproceedings{dinh2017density,
  author    = {Laurent Dinh and
               Jascha Sohl{-}Dickstein and
               Samy Bengio},
  title     = {Density estimation using Real {NVP}},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017},
  year      = {2017},
}


@inproceedings{rezende2014stochastic,
  title={Stochastic backpropagation and approximate inference in deep generative models},
  author={Rezende, Danilo Jimenez and Mohamed, Shakir and Wierstra, Daan},
  booktitle={International conference on machine learning},
  pages={1278--1286},
  year={2014},
  organization={PMLR}
}


@inproceedings{oord2016conditional,
  title={Conditional image generation with PixelCNN decoders},
  author={Oord, A{\"a}ron van den and Kalchbrenner, Nal and Vinyals, Oriol and Espeholt, Lasse and Graves, Alex and Kavukcuoglu, Koray},
  booktitle={Proceedings of the 30th International Conference on Neural Information Processing Systems},
  pages={4797--4805},
  year={2016}
}

@inproceedings{nalisnick2018deep,
  title={Do Deep Generative Models Know What They Don't Know?},
  author={Nalisnick, Eric and Matsukawa, Akihiro and Teh, Yee Whye and Gorur, Dilan and Lakshminarayanan, Balaji},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{ren2019likelihood,
	title={Likelihood ratios for out-of-distribution detection},
	author={Ren, Jie and Liu, Peter J and Fertig, Emily and Snoek, Jasper and Poplin, Ryan and Depristo, Mark and Dillon, Joshua and Lakshminarayanan, Balaji},
	booktitle=NIPS,
	pages={14680--14691},
	year={2019}
}


@inproceedings{
serra2019input,
title={Input Complexity and Out-of-distribution Detection with Likelihood-based Generative Models},
author={Joan Serrà and David Álvarez and Vicenç Gómez and Olga Slizovskaia and José F. Núñez and Jordi Luque},
booktitle={Proceedings of the International Conference on Learning Representations},
year={2020}
}

@InProceedings{pope20a, 
    title = {Adversarial Robustness of Flow-Based Generative Models}, 
    author = {Pope, Phillip and Balaji, Yogesh and Feizi, Soheil}, 
    booktitle = {Proceedings of the Twenty Third International Conference on Artificial Intelligence and Statistics}, 
    pages = {3795--3805}, 
    year = {2020}, 
    editor = {Silvia Chiappa and Roberto Calandra}, 
    volume = {108}, 
    series = {Proceedings of Machine Learning Research}, 
    month = {26--28 Aug}, 
    publisher = {PMLR}
}


@misc{hendrycks2020scaling,
    title={Scaling Out-of-Distribution Detection for Real-World Settings}, 
    author={Dan Hendrycks and Steven Basart and Mantas Mazeika and Mohammadreza Mostajabi and Jacob Steinhardt and Dawn Song},
    year={2020},
    eprint={1911.11132},
    archivePrefix={arXiv},
    primaryClass={cs.CV}
}

@article{Roady2019,
  author = {Roady, Ryne and Hayes, Tyler and Kemker, Ronald and Gonzales, Ayesha and Kanan, Christopher},
  title     = {Are Out-of-Distribution Detection Methods Effective on Large-Scale Datasets?},
  journal   = {CoRR},
  volume    = {abs/1910.14034},
  year      = {2019},
  url       = {http://arxiv.org/abs/1910.14034},
  archivePrefix = {arXiv},
  eprint    = {1910.14034},
  timestamp = {Mon, 04 Nov 2019 09:10:30 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1910-14034.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{cimpoi14describing,
	Author    = {M. Cimpoi and S. Maji and I. Kokkinos and S. Mohamed and and A. Vedaldi},
	Title     = {Describing Textures in the Wild},
	Booktitle = {Proceedings of the {IEEE} Conf. on Computer Vision and Pattern Recognition (CVPR)},
	Year      = {2014}}
	
@article{zhou2017places,
	title={Places: A 10 million image database for scene recognition},
	author={Zhou, Bolei and Lapedriza, Agata and Khosla, Aditya and Oliva, Aude and Torralba, Antonio},
	journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
	volume={40},
	number={6},
	pages={1452--1464},
	year={2017},
	publisher={IEEE}
}

% inat
@inproceedings{van2018inaturalist,
  title={The inaturalist species classification and detection dataset},
  author={Van Horn, Grant and Mac Aodha, Oisin and Song, Yang and Cui, Yin and Sun, Chen and Shepard, Alex and Adam, Hartwig and Perona, Pietro and Belongie, Serge},
  booktitle={Proceedings of the IEEE Conference on Computer Cision and Pattern Recognition},
  pages={8769--8778},
  year={2018}
}

% sun
@inproceedings{xiao2010sun,
  title={Sun database: Large-scale scene recognition from abbey to zoo},
  author={Xiao, Jianxiong and Hays, James and Ehinger, Krista A and Oliva, Aude and Torralba, Antonio},
  booktitle={2010 IEEE computer society conference on computer vision and pattern recognition},
  pages={3485--3492},
  year={2010},
  organization={IEEE}
}

%% group-based learning
@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff},
  journal={arXiv preprint arXiv:1503.02531},
  year={2015}
}

@inproceedings{ahmed2016network,
  title={Network of experts for large-scale image categorization},
  author={Ahmed, Karim and Baig, Mohammad Haris and Torresani, Lorenzo},
  booktitle={European Conference on Computer Vision},
  pages={516--532},
  year={2016},
  organization={Springer}
}

@inproceedings{yan2015hd,
  title={HD-CNN: hierarchical deep convolutional neural networks for large scale visual recognition},
  author={Yan, Zhicheng and Zhang, Hao and Piramuthu, Robinson and Jagadeesh, Vignesh and DeCoste, Dennis and Di, Wei and Yu, Yizhou},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2740--2748},
  year={2015}
}

@article{warde2014self,
  title={Self-informed neural network structure learning},
  author={Warde-Farley, David and Rabinovich, Andrew and Anguelov, Dragomir},
  journal={arXiv preprint arXiv:1412.6563},
  year={2014}
}

@inproceedings{gross2017hard,
  title={Hard mixtures of experts for large scale weakly supervised vision},
  author={Gross, Sam and Ranzato, Marc'Aurelio and Szlam, Arthur},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6865--6873},
  year={2017}
}

%% large-scale pre-training
% Google BiT

@inproceedings{kolesnikov2020big,
  author    = {Alexander Kolesnikov and
               Lucas Beyer and
               Xiaohua Zhai and
               Joan Puigcerver and
               Jessica Yung and
               Sylvain Gelly and
               Neil Houlsby},
  title     = {Big Transfer (BiT): General Visual Representation Learning},
  booktitle = {ECCV 2020},
  year      = {2020},
}

% Instagram
@inproceedings{mahajan2018exploring,
  title={Exploring the limits of weakly supervised pretraining},
  author={Mahajan, Dhruv and Girshick, Ross and Ramanathan, Vignesh and He, Kaiming and Paluri, Manohar and Li, Yixuan and Bharambe, Ashwin and van der Maaten, Laurens},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={181--196},
  year={2018}
}

@inproceedings{joulin2016learning,
  title={Learning visual features from large weakly supervised data},
  author={Joulin, Armand and Van Der Maaten, Laurens and Jabri, Allan and Vasilache, Nicolas},
  booktitle={European Conference on Computer Vision},
  pages={67--84},
  year={2016},
  organization={Springer}
}

@inproceedings{sun2017revisiting,
  title={Revisiting unreasonable effectiveness of data in deep learning era},
  author={Sun, Chen and Shrivastava, Abhinav and Singh, Saurabh and Gupta, Abhinav},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={843--852},
  year={2017}
}

@inproceedings{sharif2014cnn,
  title={CNN features off-the-shelf: an astounding baseline for recognition},
  author={Sharif Razavian, Ali and Azizpour, Hossein and Sullivan, Josephine and Carlsson, Stefan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition workshops},
  pages={806--813},
  year={2014}
}

@inproceedings{girshick2014rich,
  title={Rich feature hierarchies for accurate object detection and semantic segmentation},
  author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jitendra},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={580--587},
  year={2014}
}

@inproceedings{pinheiro2015learning,
  title={Learning to segment object candidates},
  author={Pinheiro, Pedro OO and Collobert, Ronan and Doll{\'a}r, Piotr},
  booktitle=NIPS,
  pages={1990--1998},
  year={2015}
}

@inproceedings{jaderberg2015spatial,
  title={Spatial transformer networks},
  author={Jaderberg, Max and Simonyan, Karen and Zisserman, Andrew and others},
  booktitle=NIPS,
  pages={2017--2025},
  year={2015}
}

@inproceedings{li2017learning,
  title={Learning visual n-grams from web data},
  author={Li, Ang and Jabri, Allan and Joulin, Armand and van der Maaten, Laurens},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={4183--4192},
  year={2017}
}

@article{chen2017deeplab,
  title={Deeplab: Semantic image segmentation with deep convolutional nets, atrous convolution, and fully connected crfs},
  author={Chen, Liang-Chieh and Papandreou, George and Kokkinos, Iasonas and Murphy, Kevin and Yuille, Alan L},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={40},
  number={4},
  pages={834--848},
  year={2017},
  publisher={IEEE}
}

% kmeans
@inproceedings{macqueen1967some,
  title={Some methods for classification and analysis of multivariate observations},
  author={MacQueen, James and others},
  booktitle={Proceedings of the fifth Berkeley symposium on mathematical statistics and probability},
  volume={1},
  number={14},
  pages={281--297},
  year={1967},
  organization={Oakland, CA, USA}
}

%% hierachical softmax
@inproceedings{bengio2010label,
  title={Label embedding trees for large multi-class tasks},
  author={Bengio, Samy and Weston, Jason and Grangier, David},
  booktitle=NIPS,
  pages={163--171},
  year={2010}
}

@inproceedings{deng2011fast,
  title={Fast and balanced: Efficient label tree learning for large scale object recognition},
  author={Deng, Jia and Satheesh, Sanjeev and Berg, Alexander C and Li, Fei},
  booktitle=NIPS,
  pages={567--575},
  year={2011}
}

@inproceedings{liu2013probabilistic,
  title={Probabilistic label trees for efficient large scale image classification},
  author={Liu, Baoyuan and Sadeghi, Fereshteh and Tappen, Marshall and Shamir, Ohad and Liu, Ce},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={843--850},
  year={2013}
}

@inproceedings{deng2014large,
  title={Large-scale object classification using label relation graphs},
  author={Deng, Jia and Ding, Nan and Jia, Yangqing and Frome, Andrea and Murphy, Kevin and Bengio, Samy and Li, Yuan and Neven, Hartmut and Adam, Hartwig},
  booktitle={European conference on computer vision},
  pages={48--64},
  year={2014},
  organization={Springer}
}

@inproceedings{redmon2017yolo9000,
  title={YOLO9000: better, faster, stronger},
  author={Redmon, Joseph and Farhadi, Ali},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={7263--7271},
  year={2017}
}

%% large-scale OOD
@article{roady2019outofdistribution,
  author={Ryne Roady and Tyler L. Hayes and Ronald Kemker and Ayesha Gonzales and Christopher Kanan},
  title     = {Are Out-of-Distribution Detection Methods Effective on Large-Scale
               Datasets?},
  journal   = {CoRR},
  volume    = {abs/1910.14034},
  year      = {2019},
  url       = {http://arxiv.org/abs/1910.14034},
  archivePrefix = {arXiv},
  eprint    = {1910.14034},
  timestamp = {Mon, 04 Nov 2019 09:10:30 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1910-14034.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{hendrycks2019benchmark,
  title={A benchmark for anomaly segmentation},
  author={Hendrycks, Dan and Basart, Steven and Mazeika, Mantas and Mostajabi, Mohammadreza and Steinhardt, Jacob and Song, Dawn},
  journal={arXiv preprint arXiv:1911.11132},
  year={2019}
}

%% previous OOD methods

% mc dropout
@inproceedings{gal2016dropout,
  title={Dropout as a bayesian approximation: Representing model uncertainty in deep learning},
  author={Gal, Yarin and Ghahramani, Zoubin},
  booktitle={international conference on machine learning},
  pages={1050--1059},
  year={2016},
  organization={PMLR}
}

% MSP
@inproceedings{hendrycks2016baseline,
  author    = {Dan Hendrycks and
               Kevin Gimpel},
  title     = {A Baseline for Detecting Misclassified and Out-of-Distribution Examples
               in Neural Networks},
  booktitle = {International Conference on Learning Representations, {ICLR} 2017},
  year      = {2017},
}

% ODIN
@inproceedings{liang2018enhancing,
  title={Enhancing the reliability of out-of-distribution image detection in neural networks},
  author={Liang, Shiyu and Li, Yixuan and Srikant, Rayadurgam},
  booktitle={International Conference on Learning Representations, ICLR 2018},
  year={2018}
}

% Mahalanobis
@inproceedings{lee2018simple,
  title={A simple unified framework for detecting out-of-distribution samples and adversarial attacks},
  author={Lee, Kimin and Lee, Kibok and Lee, Honglak and Shin, Jinwoo},
  booktitle=NIPS,
  pages={7167--7177},
  year={2018}
}

% Energy
@article{liu2020energy,
title={Energy-based Out-of-distribution Detection},
author={Liu, Weitang and Wang, Xiaoyun and Owens, John and Li, Yixuan},
journal=NIPS,
year={2020}
}


% OE
@inproceedings{hendrycks2018deep,
  title={Deep Anomaly Detection with Outlier Exposure},
  author={Hendrycks, Dan and Mazeika, Mantas and Dietterich, Thomas},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

% deep ensembles


% a confidence branch
@article{devries2018learning,
  title={Learning confidence for out-of-distribution detection in neural networks},
  author={DeVries, Terrance and Taylor, Graham W},
  journal={arXiv preprint arXiv:1802.04865},
  year={2018}
}


%% datasets

% cifar


%% models
% resnet-v2
@inproceedings{he2016identity,
  title={Identity mappings in deep residual networks},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={European conference on computer vision},
  pages={630--645},
  year={2016},
  organization={Springer}
}

% group softmax paper
@inproceedings{li2020overcoming,
  title={Overcoming Classifier Imbalance for Long-Tail Object Detection With Balanced Group Softmax},
  author={Li, Yu and Wang, Tao and Kang, Bingyi and Tang, Sheng and Wang, Chunfeng and Li, Jintao and Feng, Jiashi},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10991--11000},
  year={2020}
}

@article{miller1995wordnet,
  title={WordNet: a lexical database for English},
  author={Miller, George A},
  journal={Communications of the ACM},
  volume={38},
  number={11},
  pages={39--41},
  year={1995},
  publisher={ACM New York, NY, USA}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}


@inproceedings{nguyen2015deep,
  title={Deep neural networks are easily fooled: High confidence predictions for unrecognizable images},
  author={Nguyen, Anh and Yosinski, Jason and Clune, Jeff},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={427--436},
  year={2015}
}

@inproceedings{hein2019relu,
  title={Why ReLU networks yield high-confidence predictions far away from the training data and how to mitigate the problem},
  author={Hein, Matthias and Andriushchenko, Maksym and Bitterwolf, Julian},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={41--50},
  year={2019}
}

@article{hendrycks2019benchmark,
  title={A benchmark for anomaly segmentation},
  author={Hendrycks, Dan and Basart, Steven and Mazeika, Mantas and Mostajabi, Mohammadreza and Steinhardt, Jacob and Song, Dawn},
  journal={arXiv preprint arXiv:1911.11132},
  year={2019}
}

@inproceedings{wang2016cnn,
  title={Cnn-rnn: A unified framework for multi-label image classification},
  author={Wang, Jiang and Yang, Yi and Mao, Junhua and Huang, Zhiheng and Huang, Chang and Xu, Wei},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2285--2294},
  year={2016}
}


@inproceedings{nam2014large,
  title={Large-scale multi-label text classification—revisiting neural networks},
  author={Nam, Jinseok and Kim, Jungi and Menc{\'\i}a, Eneldo Loza and Gurevych, Iryna and F{\"u}rnkranz, Johannes},
  booktitle={Joint european conference on machine learning and knowledge discovery in databases},
  pages={437--452},
  year={2014},
  organization={Springer}
}

@article{lakhani2017deep,
  title={Deep learning at chest radiography: automated classification of pulmonary tuberculosis by using convolutional neural networks},
  author={Lakhani, Paras and Sundaram, Baskaran},
  journal={Radiology},
  volume={284},
  number={2},
  pages={574--582},
  year={2017},
  publisher={Radiological Society of North America}
}

@article{huang2018added,
  title={Added value of computer-aided CT image features for early lung cancer diagnosis with small pulmonary nodules: a matched case-control study},
  author={Huang, Peng and Park, Seyoun and Yan, Rongkai and Lee, Junghoon and Chu, Linda C and Lin, Cheng T and Hussien, Amira and Rathmell, Joshua and Thomas, Brett and Chen, Chen and others},
  journal={Radiology},
  volume={286},
  number={1},
  pages={286--295},
  year={2018},
  publisher={Radiological Society of North America}
}


@article{tsoumakas2007multi,
  title={Multi-label classification: An overview},
  author={Tsoumakas, Grigorios and Katakis, Ioannis},
  journal={International Journal of Data Warehousing and Mining (IJDWM)},
  volume={3},
  number={3},
  pages={1--13},
  year={2007},
  publisher={IGI Global}
}
@inproceedings{DBLP:conf/nips/TackMJS20,
  author    = {Jihoon Tack and
               Sangwoo Mo and
               Jongheon Jeong and
               Jinwoo Shin},
  title     = {{CSI:} Novelty Detection via Contrastive Learning on Distributionally
               Shifted Instances},
  booktitle = {NIPS 33, NeurIPS 2020},
  year      = {2020}
}
@inproceedings{DBLP:conf/cvpr/SunYZLP20,
  author    = {Xin Sun and
               Zhenning Yang and
               Chi Zhang and
               Keck Voon Ling and
               Guohao Peng},
  title     = {Conditional {Gaussian} Distribution Learning for Open Set Recognition},
  booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
               CVPR 2020},
  pages     = {13477--13486},
  year      = {2020},
  url       = {https://openaccess.thecvf.com/content\_CVPR\_2020/html/Sun\_Conditional\_Gaussian\_Distribution\_Learning\_for\_Open\_Set\_Recognition\_CVPR\_2020\_paper.html},
  doi       = {10.1109/CVPR42600.2020.01349},
  timestamp = {Fri, 21 Jan 2022 09:17:12 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/SunYZLP20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:journals/corr/abs-2104-13921,
  author    = {Xiuye Gu and
               Tsung{-}Yi Lin and
               Weicheng Kuo and
               Yin Cui},
  title     = {Zero-Shot Detection via Vision and Language Knowledge Distillation},
  year      = {2022},
    booktitle={10th International Conference on Learning Representations, {ICLR} 2022},
}
@inproceedings{hsu2020generalized,
  title={Generalized odin: Detecting out-of-distribution image without learning from out-of-distribution data},
  author={Hsu, Yen-Chang and Shen, Yilin and Jin, Hongxia and Kira, Zsolt},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={10951--10960},
  year={2020}
}


@inproceedings{hinz2018generating,
  title={Generating Multiple Objects at Spatially Distinct Locations},
  author={Hinz, Tobias and Heinrich, Stefan and Wermter, Stefan},
  booktitle={International Conference on Learning Representations},
  year={2018}
}


@article{cao2020benchmark,
  title={A Benchmark of Medical Out of Distribution Detection},
  author={Cao, Tianshi and Huang, Chinwei and Hui, David Yu-Tung and Cohen, Joseph Paul},
  journal={arXiv preprint arXiv:2007.04250},
  year={2020}
}

@inproceedings{nus-wide-civr09,
  author={Tat-Seng Chua and Jinhui Tang and Richang Hong and Haojie Li and Zhiping Luo and Yan-Tao Zheng},
  booktitle={Proceedings of ACM Conf. on Image and Video Retrieval (CIVR'09)},
  posted-at={2009},
  title={NUS-WIDE: A Real-World Web Image Database from National University of Singapore},
  address={Santorini, Greece. },
  year={2009}
}

@article{lecun2006tutorial,
  title={A tutorial on energy-based learning},
  author={LeCun, Yann and Chopra, Sumit and Hadsell, Raia and Ranzato, M and Huang, F},
  journal={Predicting structured data},
  volume={1},
  number={0},
  year={2006}
}


@article{du2019implicit,
  title={Implicit generation and generalization in energy-based models},
  author={Du, Yilun and Mordatch, Igor},
  journal={arXiv preprint arXiv:1903.08689},
  year={2019}
}

@inproceedings{kingma2018glow,
  title={Glow: Generative flow with invertible 1x1 convolutions},
  author={Kingma, Durk P and Dhariwal, Prafulla},
  booktitle=NIPS,
  pages={10215--10224},
  year={2018}
}

@inproceedings{grathwohl2019your,
  title={Your classifier is secretly an energy based model and you should treat it like one},
  author={Grathwohl, Will and Wang, Kuan-Chieh and Jacobsen, Joern-Henrik and Duvenaud, David and Norouzi, Mohammad and Swersky, Kevin},
  booktitle={International Conference on Learning Representations},
  year={2019}
}


@article{feinman2017detecting,
  title={Detecting adversarial samples from artifacts},
  author={Feinman, Reuben and Curtin, Ryan R and Shintre, Saurabh and Gardner, Andrew B},
  journal={arXiv preprint arXiv:1703.00410},
  year={2017}
}

@inproceedings{salakhutdinov2010efficient,
  title={Efficient learning of deep Boltzmann machines},
  author={Salakhutdinov, Ruslan and Larochelle, Hugo},
  booktitle={Proceedings of the thirteenth international conference on artificial intelligence and statistics},
  pages={693--700},
  year={2010}
}

@article{ackley1985learning,
  title={A learning algorithm for Boltzmann machines},
  author={Ackley, David H and Hinton, Geoffrey E and Sejnowski, Terrence J},
  journal={Cognitive science},
  volume={9},
  number={1},
  pages={147--169},
  year={1985},
  publisher={Elsevier}
}

@inproceedings{ma2018characterizing,
  title={Characterizing adversarial subspaces using local intrinsic dimensionality},
  author={Ma, Xingjun and Li, Bo and Wang, Yisen and Erfani, Sarah M and Wijewickrema, Sudanthi and Schoenebeck, Grant and Song, Dawn and Houle, Michael E and Bailey, James},
  booktitle={6th International Conference on Learning Representations, ICLR 2018},
  year={2018}
}

@inproceedings{zhao2019energy,
  title={Energy-based generative adversarial networks},
  author={Zhao, Junbo and Mathieu, Michael and LeCun, Yann},
  booktitle={5th International Conference on Learning Representations, ICLR 2017},
  year={2019}
}


@article{ben2010theory,
  title={A theory of learning from different domains},
  author={Ben-David, Shai and Blitzer, John and Crammer, Koby and Kulesza, Alex and Pereira, Fernando and Vaughan, Jennifer Wortman},
  journal={Machine learning},
  volume={79},
  number={1-2},
  pages={151--175},
  year={2010},
  publisher={Springer}
}


@article{DBLP:journals/corr/YuZSSX15,
	title={Lsun: Construction of a large-scale image dataset using deep learning with humans in the loop},
	author={Yu, Fisher and Seff, Ari and Zhang, Yinda and Song, Shuran and Funkhouser, Thomas and Xiao, Jianxiong},
	journal={arXiv preprint arXiv:1506.03365},
	year={2015}
}
@article{DBLP:journals/corr/XuEZFKX15,
	title={Turkergaze: Crowdsourcing saliency with webcam based eye tracking},
	author={Xu, Pingmei and Ehinger, Krista A and Zhang, Yinda and Finkelstein, Adam and Kulkarni, Sanjeev R and Xiao, Jianxiong},
	journal={arXiv preprint arXiv:1504.06755},
	year={2015}
}
@inproceedings{davis2006relationship,
	title={The relationship between Precision-Recall and ROC curves},
	author={Davis, Jesse and Goadrich, Mark},
	booktitle={Proceedings of the 23rd international conference on Machine learning},
	pages={233--240},
	year={2006}
}
@article{fawcett2006introduction,
	title={An introduction to ROC analysis},
	author={Fawcett, Tom},
	journal={Pattern recognition letters},
	volume={27},
	number={8},
	pages={861--874},
	year={2006},
	publisher={Elsevier}
}
@book{manning1999foundations,
	title={Foundations of statistical natural language processing},
	author={Manning, Christopher D and Manning, Christopher D and Sch{\"u}tze, Hinrich},
	year={1999},
	publisher={MIT press}
}
@article{saito2015precision,
	title={The precision-recall plot is more informative than the ROC plot when evaluating binary classifiers on imbalanced datasets},
	author={Saito, Takaya and Rehmsmeier, Marc},
	journal={PloS one},
	volume={10},
	number={3},
	year={2015},
	publisher={Public Library of Science}
}

@article{madry2017towards,
	title={Towards deep learning models resistant to adversarial attacks},
	author={Madry, Aleksander and Makelov, Aleksandar and Schmidt, Ludwig and Tsipras, Dimitris and Vladu, Adrian},
	journal={arXiv preprint arXiv:1706.06083},
	year={2017}
}
@inproceedings{ghorbani2019interpretation,
	title={Interpretation of neural networks is fragile},
	author={Ghorbani, Amirata and Abid, Abubakar and Zou, James},
	booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
	volume={33},
	pages={3681--3688},
	year={2019}
}
@inproceedings{chen2019robust,
	title={Robust Attribution Regularization},
	author={Chen, Jiefeng and Wu, Xi and Rastogi, Vaibhav and Liang, Yingyu and Jha, Somesh},
	booktitle=NIPS,
	pages={14300--14310},
	year={2019}
}


@inproceedings{huang2017densely,
	title={Densely connected convolutional networks},
	author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages={4700--4708},
	year={2017}
}
@article{duchi2011adaptive,
	title={Adaptive subgradient methods for online learning and stochastic optimization},
	author={Duchi, John and Hazan, Elad and Singer, Yoram},
	journal={Journal of machine learning research},
	volume={12},
	number={Jul},
	pages={2121--2159},
	year={2011}
}
@article{kingma2014adam,
	title={Adam: A method for stochastic optimization},
	author={Kingma, Diederik P and Ba, Jimmy},
	journal={arXiv preprint arXiv:1412.6980},
	year={2014}
}
@article{loshchilov2016sgdr,
	title={Sgdr: Stochastic gradient descent with warm restarts},
	author={Loshchilov, Ilya and Hutter, Frank},
	journal={arXiv preprint arXiv:1608.03983},
	year={2016}
}
@inproceedings{kingma2013auto,
  author    = {Diederik P. Kingma and
               Max Welling},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {Proceedings of 2nd International Conference on Learning Representations, {ICLR} 2014}
}

@article{xiao2020likelihood,
  title={Likelihood Regret: An Out-of-Distribution Detection Score For Variational Auto-encoder},
  author={Xiao, Zhisheng and Yan, Qing and Amit, Yali},
  journal=NIPS,
  volume={33},
  year={2020}
}

@article{kirichenko2020normalizing,
  title={Why Normalizing Flows Fail to Detect Out-of-Distribution Data},
  author={Kirichenko, Polina and Izmailov, Pavel and Wilson, Andrew G},
  journal=NIPS,
  volume={33},
  year={2020}
}

  @article{morteza2022provable,
      title={Provable Guarantees for Understanding Out-of-distribution Detection}, 
      author={Morteza, Peyman and Li, Yixuan},
      journal={Proceedings of the AAAI Conference on Artificial Intelligence},
      year={2022}
}

@inproceedings{sun2021react,
  title={ReAct: Out-of-distribution Detection With Rectified Activations},
  author={Sun, Yiyou and Guo, Chuan and Li, Yixuan},
  booktitle=NIPS,
  year={2021}
}

@inproceedings{huang2021importance,
  title={On the Importance of Gradients for Detecting Distributional Shifts in the Wild},
  author={Huang, Rui and Geng, Andrew and Li, Yixuan},
  booktitle=NIPS,
  year={2021}
}

@article{DBLP:journals/corr/abs-2108-03614,
  author    = {Kumari Deepshikha and
               Sai Harsha Yelleni and
               P. K. Srijith and
               C. Krishna Mohan},
  title     = {Monte Carlo DropBlock for Modelling Uncertainty in Object Detection},
  journal   = {CoRR},
  volume    = {abs/2108.03614},
  year      = {2021},
  eprinttype = {arXiv},
  eprint    = {2108.03614},
  timestamp = {Wed, 11 Aug 2021 15:24:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2108-03614.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2108-11941,
  author    = {Jingkang Yang and
               Haoqi Wang and
               Litong Feng and
               Xiaopeng Yan and
               Huabin Zheng and
               Wayne Zhang and
               Ziwei Liu},
  title     = {Semantically Coherent Out-of-Distribution Detection},
  journal   = {CoRR},
  volume    = {abs/2108.11941},
  year      = {2021},
  url       = {https://arxiv.org/abs/2108.11941},
  eprinttype = {arXiv},
  eprint    = {2108.11941},
  timestamp = {Fri, 27 Aug 2021 15:02:29 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2108-11941.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:journals/corr/abs-2104-08381,
  title={Robust Object Detection via Instance-Level Temporal Cycle Confusion},
  author={Xin Wang and
               Thomas E. Huang and
               Benlin Liu and
               Fisher Yu and
               Xiaolong Wang and
               Joseph E. Gonzalez and
               Trevor Darrell},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
  year={2021}
}
@InProceedings{Besnier_2021_ICCV,
    author    = {Besnier, Victor and Bursuc, Andrei and Picard, David and Briot, Alexandre},
    title     = {Triggering Failures: Out-of-Distribution Detection by Learning From Local Adversarial Attacks in Semantic Segmentation},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2021},
    pages     = {15701-15710}
}
@article{DBLP:journals/corr/abs-2108-01634,
  author    = {Victor Besnier and
               Andrei Bursuc and
               David Picard and
               Alexandre Briot},
  title     = {Triggering Failures: Out-Of-Distribution detection by learning from
               local adversarial attacks in Semantic Segmentation},
  journal   = {CoRR},
  volume    = {abs/2108.01634},
  year      = {2021},
  url       = {https://arxiv.org/abs/2108.01634},
  eprinttype = {arXiv},
  eprint    = {2108.01634},
  timestamp = {Thu, 05 Aug 2021 14:27:08 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2108-01634.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2107-04517,
  author    = {Tobias Riedlinger and
               Matthias Rottmann and
               Marius Schubert and
               Hanno Gottschalk},
  title     = {Gradient-Based Quantification of Epistemic Uncertainty for Deep Object
               Detectors},
  journal   = {CoRR},
  volume    = {abs/2107.04517},
  year      = {2021},
  eprinttype = {arXiv},
  eprint    = {2107.04517},
  timestamp = {Tue, 20 Jul 2021 15:08:33 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-04517.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{DBLP:journals/corr/abs-2108-06753,
  author    = {Dahun Kim and
               Tsung{-}Yi Lin and
               Anelia Angelova and
               In So Kweon and
               Weicheng Kuo},
  title     = {Learning Open-World Object Proposals without Learning to Classify},
  journal   = {CoRR},
  volume    = {abs/2108.06753},
  year      = {2021},
  archivePrefix = {arXiv},
  eprint    = {2108.06753},
  timestamp = {Wed, 18 Aug 2021 19:45:42 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2108-06753.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/corr/abs-2002-05347,
  author    = {Xialei Liu and
               Hao Yang and
               Avinash Ravichandran and
               Rahul Bhotika and
               Stefano Soatto},
  title     = {Continual Universal Object Detection},
  journal   = {CoRR},
  volume    = {abs/2002.05347},
  year      = {2020},
  archivePrefix = {arXiv},
  eprint    = {2002.05347},
  timestamp = {Fri, 14 Feb 2020 12:07:41 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2002-05347.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{van2016conditional,
	title={Conditional image generation with pixelcnn decoders},
	author={Van den Oord, Aaron and Kalchbrenner, Nal and Espeholt, Lasse and Vinyals, Oriol and Graves, Alex and others},
	booktitle=NIPS,
	pages={4790--4798},
	year={2016}
}
@article{tabak2013family,
	title={A family of nonparametric density estimation algorithms},
	author={Tabak, Esteban G and Turner, Cristina V},
	journal={Communications on Pure and Applied Mathematics},
	volume={66},
	number={2},
	pages={145--164},
	year={2013},
	publisher={Wiley Online Library}
}
@article{mu2019mnist,
	title={Mnist-c: A robustness benchmark for computer vision},
	author={Mu, Norman and Gilmer, Justin},
	journal={arXiv preprint arXiv:1906.02337},
	year={2019}
}

@inproceedings{guo2017calibration,
  title={On calibration of modern neural networks},
  author={Guo, Chuan and Pleiss, Geoff and Sun, Yu and Weinberger, Kilian Q},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={1321--1330},
  year={2017},
  organization={JMLR. org}
}
@article{subramanya2017confidence,
	title={Confidence estimation in deep neural networks via density modelling},
	author={Subramanya, Akshayvarun and Srinivas, Suraj and Babu, R Venkatesh},
	journal={arXiv preprint arXiv:1707.07013},
	year={2017}
}
@inproceedings{malinin2018predictive,
	title={Predictive uncertainty estimation via prior networks},
	author={Malinin, Andrey and Gales, Mark},
	booktitle=NIPS,
	pages={7047--7058},
	year={2018}
}
@article{bevandic2018discriminative,
	title={Discriminative out-of-distribution detection for semantic segmentation},
	author={Bevandi{\'c}, Petra and Kre{\v{s}}o, Ivan and Or{\v{s}}i{\'c}, Marin and {\v{S}}egvi{\'c}, Sini{\v{s}}a},
	journal={arXiv preprint arXiv:1808.07703},
	year={2018}
}
@article{torralba200880,
	title={80 million tiny images: A large data set for nonparametric object and scene recognition},
	author={Torralba, Antonio and Fergus, Rob and Freeman, William T},
	journal={IEEE transactions on pattern analysis and machine intelligence},
	volume={30},
	number={11},
	pages={1958--1970},
	year={2008},
	publisher={IEEE}
}
@article{tsipras2018robustness,
	title={Robustness may be at odds with accuracy},
	author={Tsipras, Dimitris and Santurkar, Shibani and Engstrom, Logan and Turner, Alexander and Madry, Aleksander},
	journal={arXiv preprint arXiv:1805.12152},
	year={2018}
}
@article{athalye2018obfuscated,
	title={Obfuscated gradients give a false sense of security: Circumventing defenses to adversarial examples},
	author={Athalye, Anish and Carlini, Nicholas and Wagner, David},
	journal={arXiv preprint arXiv:1802.00420},
	year={2018}
}

@article{szegedy2013intriguing,
	title={Intriguing properties of neural networks},
	author={Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
	journal={arXiv preprint arXiv:1312.6199},
	year={2013}
}
@inproceedings{papernot2016limitations,
	title={The limitations of deep learning in adversarial settings},
	author={Papernot, Nicolas and McDaniel, Patrick and Jha, Somesh and Fredrikson, Matt and Celik, Z Berkay and Swami, Ananthram},
	booktitle={2016 IEEE European symposium on security and privacy (EuroS\&P)},
	pages={372--387},
	year={2016},
	organization={IEEE}
}
@inproceedings{hadsell2006dimensionality,
  title={Dimensionality reduction by learning an invariant mapping},
  author={Hadsell, Raia and Chopra, Sumit and LeCun, Yann},
  booktitle={2006 IEEE Computer Society Conference on Computer Vision and Pattern Recognition (CVPR'06)},
  volume={2},
  pages={1735--1742},
  year={2006},
  organization={IEEE}
}
@inproceedings{biggio2013evasion,
	title={Evasion attacks against machine learning at test time},
	author={Biggio, Battista and Corona, Igino and Maiorca, Davide and Nelson, Blaine and {\v{S}}rndi{\'c}, Nedim and Laskov, Pavel and Giacinto, Giorgio and Roli, Fabio},
	booktitle={Joint European conference on machine learning and knowledge discovery in databases},
	pages={387--402},
	year={2013},
	organization={Springer}
}


@article{kurakin2016adversarial,
	title={Adversarial examples in the physical world},
	author={Kurakin, Alexey and Goodfellow, Ian and Bengio, Samy},
	journal={arXiv preprint arXiv:1607.02533},
	year={2016}
}
@inproceedings{moosavi2016deepfool,
	title={Deepfool: a simple and accurate method to fool deep neural networks},
	author={Moosavi-Dezfooli, Seyed-Mohsen and Fawzi, Alhussein and Frossard, Pascal},
	booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
	pages={2574--2582},
	year={2016}
}


@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle=NIPS,
  pages={2672--2680},
  year={2014}
}

@inproceedings{ranzato2007unified,
  title={A unified energy-based framework for unsupervised learning},
  author={Ranzato, Marc’Aurelio and Boureau, Y-Lan and Chopra, Sumit and LeCun, Yann},
  booktitle={Proceedings of the Artificial Intelligence and Statistics},
  pages={371--379},
  year={2007}
}

@inproceedings{carlini2017adversarial,
	title={Adversarial examples are not easily detected: Bypassing ten detection methods},
	author={Carlini, Nicholas and Wagner, David},
	booktitle={Proceedings of the 10th ACM Workshop on Artificial Intelligence and Security},
	pages={3--14},
	year={2017}
}

@inproceedings{ranzato2007efficient,
  title={Efficient learning of sparse representations with an energy-based model},
  author={Ranzato, Marc'Aurelio and Poultney, Christopher and Chopra, Sumit and Cun, Yann L},
  booktitle=NIPS,
  pages={1137--1144},
  year={2007}
}

@article{meinke2019towards,
  title={Towards neural networks that provably know when they don't know},
  author={Meinke, Alexander and Hein, Matthias},
  journal={arXiv preprint arXiv:1909.12180},
  year={2019}
}


@inproceedings{geifman2019selectivenet,
  title={Selectivenet: A deep neural network with an integrated reject option},
  author={Geifman, Yonatan and El-Yaniv, Ran},
  booktitle={ICML},
  pages={2151--2159},
  year={2019},
  organization={PMLR}
}

@inproceedings{sehwag2019analyzing,
  title={Analyzing the robustness of open-world machine learning},
  author={Sehwag, Vikash and Bhagoji, Arjun Nitin and Song, Liwei and Sitawarin, Chawin and Cullina, Daniel and Chiang, Mung and Mittal, Prateek},
  booktitle={Proceedings of the 12th ACM Workshop on Artificial Intelligence and Security},
  pages={105--116},
  year={2019}
}
@article{stallkamp2012man,
	title={Man vs. computer: Benchmarking machine learning algorithms for traffic sign recognition},
	author={Stallkamp, Johannes and Schlipsing, Marc and Salmen, Jan and Igel, Christian},
	journal={Neural networks},
	volume={32},
	pages={323--332},
	year={2012},
	publisher={Elsevier}
}


@inproceedings{salimans2016weight,
  title={Weight normalization: A simple reparameterization to accelerate training of deep neural networks},
  author={Salimans, Tim and Kingma, Durk P},
  booktitle=NIPS,
  pages={901--909},
  year={2016}
}

@article{lecun2010mnist,
  title={MNIST handwritten digit database},
  author={LeCun, Yann and Cortes, Corinna and Burges, CJ},
  journal={ATT Labs [Online]. Available: http://yann.lecun.com/exdb/mnist},
  volume={2},
  year={2010}
}

@inproceedings{chen2019deep,
  title={Deep hierarchical multi-label classification of chest X-ray images},
  author={Chen, Haomin and Miao, Shun and Xu, Daguang and Hager, Gregory D and Harrison, Adam P},
  booktitle={Proceedings of International Conference on Medical Imaging with Deep Learning},
  pages={109--120},
  year={2019},
  organization={PMLR}
}

@article{zagoruyko2016wide,
  title={Wide residual networks},
  author={Zagoruyko, Sergey and Komodakis, Nikos},
  journal={arXiv preprint arXiv:1605.07146},
  year={2016}
}

@article{balescu1975equilibrium,
  title={Equilibrium and nonequilibrium statistical mechanics},
  author={Balescu, Radu},
  journal={STIA},
  volume={76},
  pages={32809},
  year={1975}
}


@inproceedings{cimpoi2014describing,
  title={Describing textures in the wild},
  author={Cimpoi, Mircea and Maji, Subhransu and Kokkinos, Iasonas and Mohamed, Sammy and Vedaldi, Andrea},
  booktitle=CVPR,
  pages={3606--3613},
  year={2014}
}


@Article{Everingham15,
   author = "Everingham, M. and Eslami, S. M. A. and Van~Gool, L. and Williams, C. K. I. and Winn, J. and Zisserman, A.",
   title = "The Pascal Visual Object Classes Challenge: A Retrospective",
   journal = "International Journal of Computer Vision",
   volume = "111",
   year = "2015",
   number = "1",
   month = jan,
   pages = "98--136",
}

@inproceedings{wang2017chestx,
  title={Chestx-ray8: Hospital-scale chest x-ray database and benchmarks on weakly-supervised classification and localization of common thorax diseases},
  author={Wang, Xiaosong and Peng, Yifan and Lu, Le and Lu, Zhiyong and Bagheri, Mohammadhadi and Summers, Ronald M},
  booktitle=CVPR,
  pages={2097--2106},
  year={2017}
}

@inproceedings{zhu2017learning,
  title={Learning spatial regularization with image-level supervisions for multi-label image classification},
  author={Zhu, Feng and Li, Hongsheng and Ouyang, Wanli and Yu, Nenghai and Wang, Xiaogang},
  booktitle=CVPR,
  pages={5513--5522},
  year={2017}
}

@article{gong2013deep,
  title={Deep convolutional ranking for multilabel image annotation},
  author={Gong, Yunchao and Jia, Yangqing and Leung, Thomas and Toshev, Alexander and Ioffe, Sergey},
  journal={arXiv preprint arXiv:1312.4894},
  year={2013}
}

@article{kullback1951information,
  title={On information and sufficiency},
  author={Kullback, Solomon and Leibler, Richard A},
  journal={The annals of mathematical statistics},
  volume={22},
  number={1},
  pages={79--86},
  year={1951},
  publisher={JSTOR}
}

@article{chen2019integration,
  title={Deep integration: A multi-label architecture for road scene recognition},
  author={Chen, Long and Zhan, Wujing and Tian, Wei and He, Yuhang and Zou, Qin},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={10},
  pages={4883--4898},
  year={2019},
  publisher={IEEE}
}

@inproceedings{breunig2000lof,
  title={LOF: identifying density-based local outliers},
  author={Breunig, Markus M and Kriegel, Hans-Peter and Ng, Raymond T and Sander, J{\"o}rg},
  booktitle={Proceedings of the 2000 ACM SIGMOD international conference on Management of data},
  pages={93--104},
  year={2000}
}

@inproceedings{liu2008isolation,
  title={Isolation forest},
  author={Liu, Fei Tony and Ting, Kai Ming and Zhou, Zhi-Hua},
  booktitle={2008 Eighth IEEE International Conference on Data Mining},
  pages={413--422},
  year={2008},
  organization={IEEE}
}

@article{papadopoulos2019outlier,
  title={Outlier exposure with confidence control for out-of-distribution detection},
  author={Papadopoulos, Aristotelis-Angelos and Rajati, Mohammad Reza and Shaikh, Nazim and Wang, Jiamian},
  journal={arXiv preprint arXiv:1906.03509},
  year={2019}
}

@InProceedings{Karen2013saliency,
    Author = {Karen Simonyan and Andrea Vedaldi and Andrew Zisserman},
    Title = {Deep Inside Convolutional Networks: Visualising Image Classification Models and Saliency Maps},
    booktitle    = "ICLR (workshop track)",
    year         = "2014",
}

@InProceedings{Jost2015gbp,
  author       = "J.T. Springenberg and A. Dosovitskiy and T. Brox and M. Riedmiller",
  title        = "Striving for Simplicity: The All Convolutional Net",
  booktitle    = "ICLR (workshop track)",
  year         = "2015",
}

@InProceedings{Selvaraju2017gradcam,
    author = {Selvaraju, Ramprasaath R. and Cogswell, Michael and Das, Abhishek and Vedantam, Ramakrishna and Parikh, Devi and Batra, Dhruv},
    title = {Grad-CAM: Visual Explanations From Deep Networks via Gradient-Based Localization},
    booktitle = {Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
    month = {Oct},
    year = {2017}
}

@InProceedings{Mukund2017intgrad, 
    title = {Axiomatic Attribution for Deep Networks}, 
    author = {Mukund Sundararajan and Ankur Taly and Qiqi Yan}, 
    booktitle = {Proceedings of the 34th International Conference on Machine Learning (ICML)}, 
    pages = {3319--3328}, 
    year = {2017}, 
}

@inproceedings{
    Marco2018deeplift,
    title={Towards better understanding of gradient-based attribution methods for Deep Neural Networks},
    author={Marco Ancona and Enea Ceolini and Cengiz Öztireli and Markus Gross},
    booktitle={Proceedings of the International Conference on Learning Representations},
    year={2018},
}

@INPROCEEDINGS{Krishna2017has,  
author={K. K. {Singh} and Y. J. {Lee}},  
booktitle={2017 IEEE International Conference on Computer Vision (ICCV)},   
title={Hide-and-Seek: Forcing a Network to be Meticulous for Weakly-Supervised Object and Action Localization},   year={2017},  volume={},  number={},  pages={3544-3553},}


@article{Choe2019adl,
	author = {Choe, Junsuk and Shim, Hyunjung},
	booktitle = {Computer Vision and Pattern Recognition (CVPR)},
	year = {2019},
	month = {08},
	pages = {},
	title = {Attention-based Dropout Layer for Weakly Supervised Object Localization}
}
@article{Yun2019cutmix,
	author = {Yun, Sangdoo and Han, Dongyoon and Oh, Seong Joon and Chun, Sanghyuk and Choe, Junsuk and Yoo, Youngjoon},
	booktitle = {2019 IEEE International Conference on Computer Vision (ICCV)},
	year = {2019},
	month = {05},
	pages = {},
	title = {CutMix: Regularization Strategy to Train Strong Classifiers with Localizable Features}
}

@article{Zhang2018acol,
	author = {Zhang, Xiaolin and Wei, Yunchao and Feng, Jiashi and Yang, Yi and Huang, Thomas},
	booktitle = CVPR,
	year = {2018},
	month = {04},
	pages = {},
	title = {Adversarial Complementary Learning for Weakly Supervised Object Localization}
}

@InProceedings{Zhang2018spg,
	author = {Zhang, Xiaolin and Wei, Yunchao and Kang, Guoliang and Yang, Yi and Huang, Thomas},
	title = {Self-produced Guidance for Weakly-supervised Object Localization},
	booktitle = {ECCV},
	month = {September},
	year = {2018}
}

@InProceedings{Choe2019wsol,
	author = {Choe, Junsuk and Shim, Hyunjung},
	title = {Attention-Based Dropout Layer for Weakly Supervised Object Localization},
	booktitle = CVPR,
	month = {June},
	year = {2019}
}


@article{kuznetsova2020open,
  title={The open images dataset v4},
  author={Kuznetsova, Alina and Rom, Hassan and Alldrin, Neil and Uijlings, Jasper and Krasin, Ivan and Pont-Tuset, Jordi and Kamali, Shahab and Popov, Stefan and Malloci, Matteo and Kolesnikov, Alexander and others},
  journal={International Journal of Computer Vision},
  pages={1--26},
  year={2020},
  publisher={Springer}
}

@inproceedings{
Eric2019ganknow,
title={Do Deep Generative Models Know What They Don't Know? },
author={Eric Nalisnick and Akihiro Matsukawa and Yee Whye Teh and Dilan Gorur and Balaji Lakshminarayanan},
booktitle={Proceedings of International Conference on Learning Representations},
year={2019},
}

@article{du2019implicit,
  title={Implicit generation and generalization in energy-based models},
  author={Du, Yilun and Mordatch, Igor},
  journal={arXiv preprint arXiv:1903.08689},
  year={2019}
}



@inproceedings{kingma2018glow,
  title={Glow: Generative flow with invertible 1x1 convolutions},
  author={Kingma, Durk P and Dhariwal, Prafulla},
  booktitle=NIPS,
  pages={10215--10224},
  year={2018}
}

@inproceedings{grathwohl2019your,
  title={Your classifier is secretly an energy based model and you should treat it like one},
  author={Grathwohl, Will and Wang, Kuan-Chieh and Jacobsen, Joern-Henrik and Duvenaud, David and Norouzi, Mohammad and Swersky, Kevin},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2019}
}


@article{Kevin,
  author    = {Dan Hendrycks and Kevin Gimpel},
  title     = {A Baseline for Detecting Misclassified and Out-of-Distribution Examples in Neural Networks},
  journal = {Proceedings of International Conference on Learning Representations},
  year = {2017},
}


@misc{
wang2021energybased,
title={Energy-based Out-of-distribution Detection for Multi-label Classification},
author={Haoran Wang and Weitang Liu and Alex Bocchieri and Yixuan Li},
year={2021},
journal={https://openreview.net/forum?id=KsN9p5qJN3}
}


@Article{Wang2020covid,
	author={Wang, Linda and Lin, Zhong Qiu and Wong, Alexander},
	title={COVID-Net: a tailored deep convolutional neural network design for detection of COVID-19 cases from chest X-ray images},
	journal={Scientific Reports},
	year={2020},
	month={Nov},
	day={11},
	volume={10},
	number={1},
	pages={19549},
	issn={2045-2322},
	doi={10.1038/s41598-020-76550-z},
	url={https://doi.org/10.1038/s41598-020-76550-z}
}

@inproceedings{
sehwag2021ssd,
title={{SSD}: A Unified Framework for Self-Supervised Outlier Detection},
author={Vikash Sehwag and Mung Chiang and Prateek Mittal},
booktitle={Proceedings of International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=v5gjXpmR8J}
}

@inproceedings{tack2020csi,
  title={CSI: Novelty Detection via Contrastive Learning on Distributionally Shifted Instances},
  author={Jihoon Tack and Sangwoo Mo and Jongheon Jeong and Jinwoo Shin},
  booktitle=NIPS,
  year={2020}
}

@inproceedings{pmlr-v137-wang20a,
  author    = {Ziyu Wang and
               Bin Dai and
               David P. Wipf and
               Jun Zhu},
  title     = {Further Analysis of Outlier Detection with Deep Generative Models},
  booktitle = NIPS,
  year      = {2020},
  timestamp = {Tue, 19 Jan 2021 15:57:19 +0100},
  biburl    = {https://dblp.org/rec/conf/nips/0006DWZ20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@article{bishop1994novelty,
  title={Novelty detection and neural network validation},
  author={Bishop, Christopher M},
  journal={IEE Proceedings-Vision, Image and Signal Processing},
  volume={141},
  number={4},
  pages={217--222},
  year={1994},
  publisher={IET}
}

@article{nalisnick2019detecting,
  title={Detecting out-of-distribution inputs to deep generative models using typicality},
  author={Nalisnick, Eric and Matsukawa, Akihiro and Teh, Yee Whye and Lakshminarayanan, Balaji},
  journal={arXiv preprint arXiv:1906.02994},
  year={2019}
}

@inproceedings{morningstar2021density,
  title={Density of states estimation for out of distribution detection},
  author={Morningstar, Warren and Ham, Cusuh and Gallagher, Andrew and Lakshminarayanan, Balaji and Alemi, Alex and Dillon, Joshua},
  booktitle={Proceedings of International Conference on Artificial Intelligence and Statistics},
  pages={3232--3240},
  year={2021},
  organization={PMLR}
}

@inproceedings{mahmood2020multiscale,
  title={Multiscale Score Matching for Out-of-Distribution Detection},
  author={Mahmood, Ahsan and Oliva, Junier and Styner, Martin Andreas},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2020}
}

@article{denouden2018improving,
  title={Improving reconstruction autoencoder out-of-distribution detection with mahalanobis distance},
  author={Denouden, Taylor and Salay, Rick and Czarnecki, Krzysztof and Abdelzad, Vahdat and Phan, Buu and Vernekar, Sachin},
  journal={arXiv preprint arXiv:1812.02765},
  year={2018}
}

@inproceedings{gong2019memorizing,
  title={Memorizing normality to detect anomaly: Memory-augmented deep autoencoder for unsupervised anomaly detection},
  author={Gong, Dong and Liu, Lingqiao and Le, Vuong and Saha, Budhaditya and Mansour, Moussa Reda and Venkatesh, Svetha and Hengel, Anton van den},
  booktitle=CVPR,
  pages={1705--1714},
  year={2019}
}

@techreport{lyudchik2016outlier,
  title={Outlier detection using autoencoders},
  author={Lyudchik, Olga},
  year={2016}
}

@article{pimentel2014review,
  title={A review of novelty detection},
  author={Pimentel, Marco AF and Clifton, David A and Clifton, Lei and Tarassenko, Lionel},
  journal={Signal Processing},
  volume={99},
  pages={215--249},
  year={2014},
  publisher={Elsevier}
}
@article{yang2021generalized,
  title={Generalized out-of-distribution detection: A survey},
  author={Yang, Jingkang and Zhou, Kaiyang and Li, Yixuan and Liu, Ziwei},
  journal={arXiv preprint arXiv:2110.11334},
  year={2021}
}
@inproceedings{havtorn2021hierarchical,
  title={Hierarchical vaes know what they don’t know},
  author={Havtorn, Jakob D and Frellsen, Jes and Hauberg, S{\o}ren and Maal{\o}e, Lars},
  booktitle={ICML},
  pages={4117--4128},
  year={2021},
  organization={PMLR}
}
@inproceedings{zhang2021understanding,
  title={Understanding failures in out-of-distribution detection with deep generative models},
  author={Zhang, Lily and Goldstein, Mark and Ranganath, Rajesh},
  booktitle={ICML},
  pages={12427--12436},
  year={2021},
  organization={PMLR}
}
@inproceedings{sohl2015deep,
  title={Deep unsupervised learning using nonequilibrium thermodynamics},
  author={Sohl-Dickstein, Jascha and Weiss, Eric and Maheswaranathan, Niru and Ganguli, Surya},
  booktitle={ICML},
  pages={2256--2265},
  year={2015},
  organization={PMLR}
}
@article{ho2020denoising,
  title={Denoising diffusion probabilistic models},
  author={Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
  journal=NIPS,
  volume={33},
  pages={6840--6851},
  year={2020}
}

@inproceedings{rombach2022high,
  title={High-resolution image synthesis with latent diffusion models},
  author={Rombach, Robin and Blattmann, Andreas and Lorenz, Dominik and Esser, Patrick and Ommer, Bj{\"o}rn},
  booktitle=CVPR,
  pages={10684--10695},
  year={2022}
}
@inproceedings{ronneberger2015u,
  title={U-net: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={Proceedings of International Conference on Medical image computing and computer-assisted intervention},
  pages={234--241},
  year={2015},
  organization={Springer}
}
@inproceedings{liu2021pseudo,
  title={Pseudo Numerical Methods for Diffusion Models on Manifolds},
  author={Liu, Luping and Ren, Yi and Lin, Zhijie and Zhao, Zhou},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2021}
}
@inproceedings{zhang2018unreasonable,
  title={The unreasonable effectiveness of deep features as a perceptual metric},
  author={Zhang, Richard and Isola, Phillip and Efros, Alexei A and Shechtman, Eli and Wang, Oliver},
  booktitle=CVPR,
  pages={586--595},
  year={2018}
}
@article{xiao2017fashion,
  title={Fashion-mnist: a novel image dataset for benchmarking machine learning algorithms},
  author={Xiao, Han and Rasul, Kashif and Vollgraf, Roland},
  journal={arXiv preprint arXiv:1708.07747},
  year={2017}
}
@inproceedings{liu2015faceattributes,
  title = {Deep Learning Face Attributes in the Wild},
  author = {Liu, Ziwei and Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
  booktitle = {ICCV},
  month = {December},
  year = {2015} 
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}
@article{kingma2018glow,
  title={Glow: Generative flow with invertible 1x1 convolutions},
  author={Kingma, Durk P and Dhariwal, Prafulla},
  journal=NIPS,
  volume={31},
  year={2018}
}
@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@inproceedings{ioffe2015batch,
  title={{Batch Normalization}: Accelerating deep network training by reducing internal covariate shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  booktitle={ICML},
  pages={448--456},
  year={2015},
  organization={PMLR}
}

@misc{dieleman2022diffusion,
  author = {Dieleman, Sander},
  title = {Diffusion models are autoencoders},
  url = {https://benanne.github.io/2022/01/31/diffusion.html},
  year = {2022}
}
@article{krizhevsky2014one,
  title={One weird trick for parallelizing convolutional neural networks},
  author={Krizhevsky, Alex},
  journal={arXiv preprint arXiv:1404.5997},
  year={2014}
}
@article{scikit-learn,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V.
         and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P.
         and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and
         Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
 journal={Journal of Machine Learning Research},
 volume={12},
 pages={2825--2830},
 year={2011}
}
@article{ramachandran2017searching,
  title={Searching for activation functions},
  author={Ramachandran, Prajit and Zoph, Barret and Le, Quoc V},
  journal={arXiv preprint arXiv:1710.05941},
  year={2017}
}
@inproceedings{xiao2021tackling,
  title={Tackling the Generative Learning Trilemma with Denoising Diffusion GANs},
  author={Xiao, Zhisheng and Kreis, Karsten and Vahdat, Arash},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2021}
}
@article{zhang2022fast,
  title={Fast Sampling of Diffusion Models with Exponential Integrator},
  author={Zhang, Qinsheng and Chen, Yongxin},
  journal={arXiv preprint arXiv:2204.13902},
  year={2022}
}
@inproceedings{kong2021fast,
  title={On Fast Sampling of Diffusion Probabilistic Models},
  author={Kong, Zhifeng and Ping, Wei},
  booktitle={Proceedings of ICML Workshop on Invertible Neural Networks, Normalizing Flows, and Explicit Likelihood Models},
  year={2021}
}
@inproceedings{mahalanobis1936generalized,
  title={On the generalized distance in statistics},
  author={Mahalanobis, Prasanta Chandra},
  year={1936},
  organization={National Institute of Science of India}
}
@article{salehi2021unified,
  title={A unified survey on anomaly, novelty, open-set, and out-of-distribution detection: Solutions and future challenges},
  author={Salehi, Mohammadreza and Mirzaei, Hossein and Hendrycks, Dan and Li, Yixuan and Rohban, Mohammad Hossein and Sabokrou, Mohammad},
  journal={arXiv preprint arXiv:2110.14051},
  year={2021}
}
@inproceedings{zong2018deep,
  title={Deep Autoencoding {Gaussian} Mixture Model for Unsupervised Anomaly Detection},
  author={Zong, Bo and Song, Qi and Min, Martin Renqiang and Cheng, Wei and Lumezanu, Cristian and Cho, Daeki and Chen, Haifeng},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2018}
}
@inproceedings{salimans2021progressive,
  title={Progressive Distillation for Fast Sampling of Diffusion Models},
  author={Salimans, Tim and Ho, Jonathan},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2021}
}
@article{song2020denoising,
  title={Denoising diffusion implicit models},
  author={Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
  journal={arXiv preprint arXiv:2010.02502},
  year={2020}
}
@article{vahdat2021score,
  title={Score-based generative modeling in latent space},
  author={Vahdat, Arash and Kreis, Karsten and Kautz, Jan},
  journal=NIPS,
  volume={34},
  pages={11287--11302},
  year={2021}
}
@article{dockhorn2022genie,
  title={GENIE: Higher-Order Denoising Diffusion Solvers},
  author={Dockhorn, Tim and Vahdat, Arash and Kreis, Karsten},
  journal={arXiv preprint arXiv:2210.05475},
  year={2022}
}
@inproceedings{watson2021learning,
  title={Learning fast samplers for diffusion models by differentiating through sample quality},
  author={Watson, Daniel and Chan, William and Ho, Jonathan and Norouzi, Mohammad},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2021}
}
@inproceedings{bao2021analytic,
  title={Analytic-DPM: an Analytic Estimate of the Optimal Reverse Variance in Diffusion Probabilistic Models},
  author={Bao, Fan and Li, Chongxuan and Zhu, Jun and Zhang, Bo},
  booktitle={Proceedings of International Conference on Learning Representations},
  year={2021}
}
@article{agarap2018deep,
  title={Deep learning using rectified linear units (relu)},
  author={Agarap, Abien Fred},
  journal={arXiv preprint arXiv:1803.08375},
  year={2018}
}

@INPROCEEDINGS{8953671,
  author={Li, Xiang and Chen, Shuo and Hu, Xiaolin and Yang, Jian},
  booktitle=CVPR, 
  title={Understanding the Disharmony Between Dropout and Batch Normalization by Variance Shift}, 
  year={2019},
  volume={},
  number={},
  pages={2677-2685},
  doi={10.1109/CVPR.2019.00279}}

@article{wang2022internimage,
  title={InternImage: Exploring Large-Scale Vision Foundation Models with Deformable Convolutions},
  author={Wang, Wenhai and Dai, Jifeng and Chen, Zhe and Huang, Zhenhang and Li, Zhiqi and Zhu, Xizhou and Hu, Xiaowei and Lu, Tong and Lu, Lewei and Li, Hongsheng and others},
  journal={arXiv preprint arXiv:2211.05778},
  year={2022}
}

@article{DBLP:journals/corr/abs-2012-07177,
  author    = {Golnaz Ghiasi and
               Yin Cui and
               Aravind Srinivas and
               Rui Qian and
               Tsung{-}Yi Lin and
               Ekin D. Cubuk and
               Quoc V. Le and
               Barret Zoph},
  title     = {Simple Copy-Paste is a Strong Data Augmentation Method for Instance
               Segmentation},
  journal   = {CoRR},
  volume    = {abs/2012.07177},
  year      = {2020},
  url       = {https://arxiv.org/abs/2012.07177},
  eprinttype = {arXiv},
  eprint    = {2012.07177},
  timestamp = {Sat, 02 Jan 2021 15:43:30 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2012-07177.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{dagli2021cppe5,
      title={CPPE-5: Medical Personal Protective Equipment Dataset}, 
      author={Rishit Dagli and Ali Mustufa Shaikh},
      year={2021},
      eprint={2112.09569},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{DBLP:journals/corr/abs-1711-05101,
  author    = {Ilya Loshchilov and
               Frank Hutter},
  title     = {Fixing Weight Decay Regularization in Adam},
  journal   = {CoRR},
  volume    = {abs/1711.05101},
  year      = {2017},
  url       = {http://arxiv.org/abs/1711.05101},
  eprinttype = {arXiv},
  eprint    = {1711.05101},
  timestamp = {Mon, 13 Aug 2018 16:48:18 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1711-05101.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{kingma2015variational,
  title={Variational dropout and the local reparameterization trick},
  author={Kingma, Durk P and Salimans, Tim and Welling, Max},
  journal=NIPS,
  volume={28},
  year={2015}
}

@inproceedings{louizos2017multiplicative,
  title={Multiplicative normalizing flows for variational bayesian neural networks},
  author={Louizos, Christos and Welling, Max},
  booktitle=ICML,
  pages={2218--2227},
  year={2017},
  organization={PMLR}
}

@article{wu2018deterministic,
  title={Deterministic variational inference for robust bayesian neural networks},
  author={Wu, Anqi and Nowozin, Sebastian and Meeds, Edward and Turner, Richard E and Hernandez-Lobato, Jose Miguel and Gaunt, Alexander L},
  journal={arXiv preprint arXiv:1810.03958},
  year={2018}
}

@ARTICLE{9525313,
  author={Feng, Di and Harakeh, Ali and Waslander, Steven L. and Dietmayer, Klaus},
  journal={IEEE Transactions on Intelligent Transportation Systems}, 
  title={A Review and Comparative Study on Probabilistic Object Detection in Autonomous Driving}, 
  year={2022},
  volume={23},
  number={8},
  pages={9961-9980},
  doi={10.1109/TITS.2021.3096854}}

@article{sze2017efficient,
  title={Efficient processing of deep neural networks: A tutorial and survey},
  author={Sze, Vivienne and Chen, Yu-Hsin and Yang, Tien-Ju and Emer, Joel S},
  journal={Proceedings of the IEEE},
  volume={105},
  number={12},
  pages={2295--2329},
  year={2017},
  publisher={Ieee}
}

@INPROCEEDINGS{9922026,
  author={Huang, Chengjie and Nguyen, Van Duong and Abdelzad, Vahdat and Mannes, Christopher Gus and Rowe, Luke and Therien, Benjamin and Salay, Rick and Czarnecki, Krzysztof},
  booktitle={Proceedings of the 2022 IEEE 25th International Conference on Intelligent Transportation Systems (ITSC)}, 
  title={Out-of-Distribution Detection for LiDAR-based 3D Object Detection}, 
  year={2022},
  volume={},
  number={},
  pages={4265-4271},
  doi={10.1109/ITSC55140.2022.9922026}}

@article{DBLP:journals/corr/abs-1708-02182,
  author    = {Stephen Merity and
               Nitish Shirish Keskar and
               Richard Socher},
  title     = {Regularizing and Optimizing {LSTM} Language Models},
  journal   = {CoRR},
  volume    = {abs/1708.02182},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.02182},
  eprinttype = {arXiv},
  eprint    = {1708.02182},
  timestamp = {Mon, 13 Aug 2018 16:47:54 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1708-02182.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{9933263,
  author={Santana, Misael Alpizar and Calinescu, Radu and Paterson, Colin},
  booktitle={Proceedings of the 2022 18th European Dependable Computing Conference (EDCC)}, 
  title={Risk-aware Real-time Object Detection}, 
  year={2022},
  volume={},
  number={},
  pages={105-108},
  doi={10.1109/EDCC57035.2022.00026}}

@article{rasmussen1995practical,
  title={A practical Monte Carlo implementation of Bayesian learning},
  author={Rasmussen, Carl},
  journal={Advances in Neural Information Processing Systems},
  volume={8},
  year={1995}
}

@INPROCEEDINGS{10224150,
  author={Zhang, Tianhao and Wang, Shenglin and Bouaynaya, Nidhal and Calinescu, Radu and Mihaylova, Lyudmila},
  booktitle={Proc. of the 26th International Conference on Information Fusion}, 
  title={Out-of-distribution Object Detection through Bayesian Uncertainty Estimation}, 
  year={2023},
  volume={},
  number={},
  pages={1-8},
  doi={10.23919/FUSION52260.2023.10224150}}

@inproceedings{müller2023transformers,
  title		= {Transformers Can Do Bayesian Inference},
  author	= {S. M{\"u}ller and N. Hollmann and S. Arango and J. Grabocka and F. Hutter},
  booktitle = {Proceedings of International Conference on Learning Representations},
  year = {2022},
  url	= {https://openreview.net/forum?id=KSugKcbNf9}
}

@InProceedings{Zhang_2022_CVPR,
  author = {Zhang, Chongzhi and Zhang, Mingyuan and Zhang, Shanghang and Jin, Daisheng and Zhou, Qiang and Cai, Zhongang and Zhao, Haiyu and Liu, Xianglong and Liu, Ziwei},
  title = {Delving Deep Into the Generalization of Vision Transformers Under Distribution Shifts},
  booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  month = {June},
  year = {2022},
  pages = {7277-7286}
}

@inproceedings{du2023dream,
      title={Dream the Impossible: Outlier Imagination with Diffusion Models}, 
      author={Xuefeng Du and Yiyou Sun and Xiaojin Zhu and Yixuan Li },
      booktitle={Advances in Neural Information Processing Systems},
      year = {2023}
}

@misc{hollmann2023tabpfn,
      title={TabPFN: A Transformer That Solves Small Tabular Classification Problems in a Second}, 
      author={Noah Hollmann and Samuel Müller and Katharina Eggensperger and Frank Hutter},
      year={2023},
      eprint={2207.01848},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{liu2021swin,
  author    = {Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  title     = {Swin Transformer: Hierarchical Vision Transformer Using Shifted Windows},
  booktitle = {Proceedings of ICCV 2021},
  year      = {2021},
  month     = {October},
}

@inproceedings{he2022masked,
  title={Masked autoencoders are scalable vision learners},
  author={He, Kaiming and Chen, Xinlei and Xie, Saining and Li, Yanghao and Doll{\'a}r, Piotr and Girshick, Ross},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={16000--16009},
  year={2022}
}

@inproceedings{zhu2021deformable,
title={Deformable {\{}DETR{\}}: Deformable Transformers for End-to-End Object Detection},
author={Xizhou Zhu and Weijie Su and Lewei Lu and Bin Li and Xiaogang Wang and Jifeng Dai},
booktitle={International Conference on Learning Representations},
year={2021}
}

@article{paul2021vision,
  title={Vision transformers are robust learners},
  author={Paul, Sayak and Chen, Pin-Yu},
  journal={arXiv preprint arXiv:2105.07581},
  year={2021}
}

@article{bai2021transformers,
  title={Are Transformers More Robust Than CNNs?},
  author={Bai, Yutong and Mei, Jieru and Yuille, Alan and Xie, Cihang},
  journal={arXiv preprint arXiv:2111.05464},
  year={2021}
}

@article{caron2021emerging,
  title={Emerging properties in self-supervised vision transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J{\'e}gou, Herv{\'e} and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  journal={arXiv preprint arXiv:2104.14294},
  year={2021}
}

@article{naseer2021intriguing,
  title={Intriguing Properties of Vision Transformers},
  author={Naseer, Muzammal and Ranasinghe, Kanchana and Khan, Salman and Hayat, Munawar and Khan, Fahad Shahbaz and Yang, Ming-Hsuan},
  journal={arXiv preprint arXiv:2105.10497},
  year={2021}
}


@InProceedings{pmlr-v202-bai23a,
  title = 	 {Feed Two Birds with One Scone: Exploiting Wild Data for Both Out-of-Distribution Generalization and Detection},
  author =       {Bai, Haoyue and Canal, Gregory and Du, Xuefeng and Kwon, Jeongyeol and Nowak, Robert D and Li, Yixuan},
  booktitle = 	 {Proceedings of the 40th International Conference on Machine Learning},
  pages = 	 {1454--1471},
  year = 	 {2023},
  editor = 	 {Krause, Andreas and Brunskill, Emma and Cho, Kyunghyun and Engelhardt, Barbara and Sabato, Sivan and Scarlett, Jonathan},
  volume = 	 {202},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {23--29 Jul},
  publisher =    {PMLR},
  pdf = 	 {https://proceedings.mlr.press/v202/bai23a/bai23a.pdf},
  url = 	 {https://proceedings.mlr.press/v202/bai23a.html},
  abstract = 	 {Modern machine learning models deployed in the wild can encounter both covariate and semantic shifts, giving rise to the problems of out-of-distribution (OOD) generalization and OOD detection respectively. While both problems have received significant research attention lately, they have been pursued independently. This may not be surprising, since the two tasks have seemingly conflicting goals. This paper provides a new unified approach that is capable of simultaneously generalizing to covariate shifts while robustly detecting semantic shifts. We propose a margin-based learning framework that exploits freely available unlabeled data in the wild that captures the environmental test-time OOD distributions under both covariate and semantic shifts. We show both empirically and theoretically that the proposed margin constraint is the key to achieving both OOD generalization and detection. Extensive experiments show the superiority of our framework, outperforming competitive baselines that specialize in either OOD generalization or OOD detection. Code is publicly available at https://github.com/deeplearning-wisc/scone.}
}

@ARTICLE{10088164,
  author={Liu, Yang and Zhang, Yao and Wang, Yixin and Hou, Feng and Yuan, Jin and Tian, Jiang and Zhang, Yang and Shi, Zhongchao and Fan, Jianping and He, Zhiqiang},
  journal={IEEE Transactions on Neural Networks and Learning Systems}, 
  title={A Survey of Visual Transformers}, 
  year={2023},
  volume={},
  number={},
  pages={1-21},
  doi={10.1109/TNNLS.2022.3227717}}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, Lukasz and Polosukhin, Illia},
  journal={Advances in Neural Information Processing Systems},
  volume={30},
  year={2017}
}

@inproceedings{chen2020generative,
  title={Generative pretraining from pixels},
  author={Chen, Mark and Radford, Alec and Child, Rewon and Wu, Jeffrey and Jun, Heewoo and Luan, David and Sutskever, Ilya},
  booktitle={International Conference on Machine Learning},
  pages={1691--1703},
  year={2020},
  organization={PMLR}
}

@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

@inproceedings{DBLP:conf/eccv/CarionMSUKZ20,
  author    = {Nicolas Carion and
               Francisco Massa and
               Gabriel Synnaeve and
               Nicolas Usunier and
               Alexander Kirillov and
               Sergey Zagoruyko},
  title     = {End-to-End Object Detection with Transformers},
  booktitle = {Computer Vision - {ECCV} 2020 - 16th European Conference, Glasgow,
               UK, August 23-28, 2020, Proceedings, Part {I}},
  series    = {Lecture Notes in Computer Science},
  volume    = {12346},
  pages     = {213--229},
  publisher = {Springer},
  year      = {2020}
}

@article{dong2021cswin,
	title={CSWin Transformer: A General Vision Transformer Backbone with Cross-Shaped Windows},
	author={Dong, Xiaoyi and Bao, Jianmin and Chen, Dongdong and Zhang, Weiming and Yu, Nenghai and Yuan, Lu and Chen, Dong and Guo, Baining},
	journal={arXiv:2107.00652},
	year={2021}
}

@article{wang2020end,
  title={End-to-End Video Instance Segmentation with Transformers},
  author={Wang, Yuqing and Xu, Zhaoliang and Wang, Xinlong and Shen, Chunhua and Cheng, Baoshan and Shen, Hao and Xia, Huaxia},
  journal={arXiv preprint arXiv:2011.14503},
  year={2020}
}

@article{chen2020pre,
  title={Pre-trained image processing transformer},
  author={Chen, Hanting and Wang, Yunhe and Guo, Tianyu and Xu, Chang and Deng, Yiping and Liu, Zhenhua and Ma, Siwei and Xu, Chunjing and Xu, Chao and Gao, Wen},
  journal={arXiv preprint arXiv:2012.00364},
  year={2020}
}

 @inproceedings{wang2023learning,
      title={Learning to Augment Distributions for Out-of-Distribution Detection}, 
      author={Qizhou Wang and Zhen Fang and Yonggang Zhang and Feng Liu and Yixuan Li and Bo Han},
      booktitle={Advances in Neural Information Processing Systems},
      year = {2023}
}

@inproceedings{tao2023nonparametric,
  title={Non-Parametric Outlier Synthesis},
  author={Tao, Leitian and Du, Xuefeng and Zhu, Xiaojin and Li, Yixuan},
  booktitle={Proceedings of the International Conference on Learning Representations},
  year={2023}
}

@inproceedings{du2022siren,
  title={SIREN: Shaping Representations for Detecting Out-of-Distribution Objects},
  author={Du, Xuefeng and Gozum, Gabriel and Ming, Yifei and Li, Yixuan},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022}
}

@inproceedings{ming2022delving,
  title={Delving into Out-of-Distribution Detection with Vision-Language Representations},
  author={Ming, Yifei and Cai, Ziyang and Gu, Jiuxiang and Sun, Yiyou and Li, Wei and Li, Yixuan},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022}
}

@article{zhang2023openood,
    title={OpenOOD v1.5: Enhanced Benchmark for Out-of-Distribution Detection},
    author={Zhang, Jingyang and Yang, Jingkang and Wang, Pengyun and Wang, Haoqi and Lin, Yueqian and Zhang, Haoran and Sun, Yiyou and Du, Xuefeng and Zhou, Kaiyang and Zhang, Wayne and Li, Yixuan and Liu, Ziwei and Chen, Yiran and Hai, Li},
    journal={arXiv preprint arXiv:2306.09301},
    year={2023},
}

@inproceedings{
vaze2022openset,
title={Open-Set Recognition: A Good Closed-Set Classifier is All You Need},
author={Sagar Vaze and Kai Han and Andrea Vedaldi and Andrew Zisserman},
booktitle={International Conference on Learning Representations},
year={2022},
url={https://openreview.net/forum?id=5hLP5JY9S2d}
}

@inproceedings{
bitterwolf2023ninco,
title={In or Out? Fixing ImageNet Out-of-Distribution Detection Evaluation},
author={Julian Bitterwolf and Maximilian Mueller and Matthias Hein},
booktitle=ICML,
year={2023},
url={https://proceedings.mlr.press/v202/bitterwolf23a.html}
}


@inproceedings{haoqi2022vim,
title = {ViM: Out-Of-Distribution with Virtual-logit Matching},
author = {Wang, Haoqi and Li, Zhizhong and Feng, Litong and Zhang, Wayne},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
year = {2022}
}

@article{park2022matteformer,
  title={MatteFormer: Transformer-Based Image Matting via Prior-Tokens},
  author={Park, GyuTae and Son, SungJoon and Yoo, JaeYoung and Kim, SeHo and Kwak, Nojun},
  journal={arXiv preprint arXiv:2203.15662},
  year={2022}
}

@inproceedings{xixi2023GEN,
title = {GEN: Pushing the Limits of Softmax-Based Out-of-Distribution Detection},
author = {Liu, Xixi and Lochman, Yaroslava and Chrsitopher, Zach},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
year = {2023}
}

@inproceedings{sun2022out,
  title={Out-of-distribution Detection with Deep Nearest Neighbors},
  author={Sun, Yiyou and Ming, Yifei and Zhu, Xiaojin and Li, Yixuan},
  booktitle={Proceedings of the International Conference on Machine Learning},
  pages={20827--20840},
  year={2022}
}

@article{danielsson1980euclidean,
  title={Euclidean distance mapping},
  author={Danielsson, Per-Erik},
  journal={Computer Graphics and image processing},
  volume={14},
  number={3},
  pages={227--248},
  year={1980},
  publisher={Elsevier}
}

@inproceedings{du2022towards,
      title={VOS: Learning What You Don’t Know by Virtual Outlier Synthesis}, 
      author={Du, Xuefeng and Wang, Zhaoning and Cai, Mu and Li, Yixuan},
      booktitle={Proceedings of the International Conference on Learning Representations},
      year={2022}
}

@misc{li2021localvit,
      title={LocalViT: Bringing Locality to Vision Transformers}, 
      author={Yawei Li and Kai Zhang and Jiezhang Cao and Radu Timofte and Luc Van Gool},
      year={2021},
      eprint={2104.05707},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{xu2021vitae,
      title={ViTAE: Vision Transformer Advanced by Exploring Intrinsic Inductive Bias}, 
      author={Yufei Xu and Qiming Zhang and Jing Zhang and Dacheng Tao},
      year={2021},
      eprint={2106.03348},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{jelassi2022vision,
  title={Vision transformers provably learn spatial structure},
  author={Jelassi, Samy and Sander, Michael and Li, Yuanzhi},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={37822--37836},
  year={2022}
}

@inproceedings{wang2022vim,
  title={ViM: Out-Of-Distribution with Virtual-logit Matching},
  author={Wang, Haoqi and Li, Zhizhong and Feng, Litong and Zhang, Wayne},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4921--4930},
  year={2022}
}

@article{d2021out,
  title={On out-of-distribution detection with Bayesian neural networks},
  author={D'Angelo, Francesco and Henning, Christian},
  journal={arXiv preprint arXiv:2110.06020},
  year={2021}
}


@InProceedings{pmlr-v80-wang18i,
  title = 	 {Adversarial Distillation of {B}ayesian Neural Network Posteriors},
  author =       {Wang, Kuan-Chieh and Vicol, Paul and Lucas, James and Gu, Li and Grosse, Roger and Zemel, Richard},
  booktitle = 	 {Proceedings of the 35th International Conference on Machine Learning},
  pages = 	 {5190--5199},
  year = 	 {2018},
  editor = 	 {Dy, Jennifer and Krause, Andreas},
  volume = 	 {80},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {10--15 Jul},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v80/wang18i/wang18i.pdf},
  url = 	 {https://proceedings.mlr.press/v80/wang18i.html},
  abstract = 	 {Bayesian neural networks (BNNs) allow us to reason about uncertainty in a principled way. Stochastic Gradient Langevin Dynamics (SGLD) enables efficient BNN learning by drawing samples from the BNN posterior using mini-batches. However, SGLD and its extensions require storage of many copies of the model parameters, a potentially prohibitive cost, especially for large neural networks. We propose a framework, Adversarial Posterior Distillation, to distill the SGLD samples using a Generative Adversarial Network (GAN). At test-time, samples are generated by the GAN. We show that this distillation framework incurs no loss in performance on recent BNN applications including anomaly detection, active learning, and defense against adversarial attacks. By construction, our framework distills not only the Bayesian predictive distribution, but the posterior itself. This allows one to compute quantities such as the approximate model variance, which is useful in downstream tasks. To our knowledge, these are the first results applying MCMC-based BNNs to the aforementioned applications.}
}

@article{wang2021bayesian,
  title={Bayesian OOD detection with aleatoric uncertainty and outlier exposure},
  author={Wang, Xi and Aitchison, Laurence},
  journal={arXiv preprint arXiv:2102.12959},
  year={2021}
}

@misc{huang2022vision,
      title={Vision Transformer with Super Token Sampling}, 
      author={Huaibo Huang and Xiaoqiang Zhou and Jie Cao and Ran He and Tieniu Tan},
      year={2022},
      eprint={2211.11167},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{fayyaz2022adaptive,
  title={Adaptive token sampling for efficient vision transformers},
  author={Fayyaz, Mohsen and Koohpayegani, Soroush Abbasi and Jafari, Farnoush Rezaei and Sengupta, Sunando and Joze, Hamid Reza Vaezi and Sommerlade, Eric and Pirsiavash, Hamed and Gall, J{\"u}rgen},
  booktitle={European Conference on Computer Vision},
  pages={396--414},
  year={2022},
  organization={Springer}
}

@article{chang2023survey,
  title={A survey on evaluation of large language models},
  author={Chang, Yupeng and Wang, Xu and Wang, Jindong and Wu, Yuan and Yang, Linyi and Zhu, Kaijie and Chen, Hao and Yi, Xiaoyuan and Wang, Cunxiang and Wang, Yidong and others},
  journal={ACM Transactions on Intelligent Systems and Technology},
  year={2023},
  publisher={ACM New York, NY}
}

@article{kirillov2023segany,
  title={Segment Anything},
  author={Kirillov, Alexander and Mintun, Eric and Ravi, Nikhila and Mao, Hanzi and Rolland, Chloe and Gustafson, Laura and Xiao, Tete and Whitehead, Spencer and Berg, Alexander C. and Lo, Wan-Yen and Doll{\'a}r, Piotr and Girshick, Ross},
  journal={arXiv:2304.02643},
  year={2023}
}

@article{bai2023sequential,
  title={Sequential modeling enables scalable learning for large vision models},
  author={Bai, Yutong and Geng, Xinyang and Mangalam, Karttikeya and Bar, Amir and Yuille, Alan and Darrell, Trevor and Malik, Jitendra and Efros, Alexei A},
  journal={arXiv preprint arXiv:2312.00785},
  year={2023}
}

@inproceedings{NEURIPS2023_7a92bcde,
 author = {Valmeekam, Karthik and Marquez, Matthew and Olmo, Alberto and Sreedharan, Sarath and Kambhampati, Subbarao},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {A. Oh and T. Neumann and A. Globerson and K. Saenko and M. Hardt and S. Levine},
 pages = {38975--38987},
 publisher = {Curran Associates, Inc.},
 title = {PlanBench: An Extensible Benchmark for Evaluating Large Language Models on Planning and Reasoning about Change},
 url = {https://proceedings.neurips.cc/paper_files/paper/2023/file/7a92bcdede88c7afd108072faf5485c8-Paper-Datasets_and_Benchmarks.pdf},
 volume = {36},
 year = {2023}
}

@article{mao2023cross,
  title={Cross-entropy loss functions: Theoretical analysis and applications},
  author={Mao, Anqi and Mohri, Mehryar and Zhong, Yutao},
  journal={arXiv preprint arXiv:2304.07288},
  year={2023}
}

@inproceedings{park2023nearest,
  title={Nearest Neighbor Guidance for Out-of-Distribution Detection},
  author={Park, Jaewoo and Jung, Yoon Gyo and Teoh, Andrew Beng Jin},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1686--1695},
  year={2023}
}

@article{hendrycks2019scaling,
  title={Scaling out-of-distribution detection for real-world settings},
  author={Hendrycks, Dan and Basart, Steven and Mazeika, Mantas and Mostajabi, Mohammadreza and Steinhardt, Jacob and Song, Dawn},
  journal={arXiv preprint arXiv:1911.11132},
  year={2019}
}

@inproceedings{touvron2021training,
  title={Training data-efficient image transformers \& distillation through attention},
  author={Touvron, Hugo and Cord, Matthieu and Douze, Matthijs and Massa, Francisco and Sablayrolles, Alexandre and J{\'e}gou, Herv{\'e}},
  booktitle={International conference on machine learning},
  pages={10347--10357},
  year={2021},
  organization={PMLR}
}

@inproceedings{singh2022revisiting,
  title={Revisiting weakly supervised pre-training of visual perception models},
  author={Singh, Mannat and Gustafson, Laura and Adcock, Aaron and de Freitas Reis, Vinicius and Gedik, Bugra and Kosaraju, Raj Prateek and Mahajan, Dhruv and Girshick, Ross and Doll{\'a}r, Piotr and Van Der Maaten, Laurens},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={804--814},
  year={2022}
}

@article{fort2021exploring,
  title={Exploring the limits of out-of-distribution detection},
  author={Fort, Stanislav and Ren, Jie and Lakshminarayanan, Balaji},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={7068--7081},
  year={2021}
}

@article{koner2021oodformer,
  title={Oodformer: Out-of-distribution detection transformer},
  author={Koner, Rajat and Sinhamahapatra, Poulami and Roscher, Karsten and G{\"u}nnemann, Stephan and Tresp, Volker},
  journal={arXiv preprint arXiv:2107.08976},
  year={2021}
}

@article{vaze2021open,
  title={Open-set recognition: A good closed-set classifier is all you need},
  author={Vaze, Sagar and Han, Kai and Vedaldi, Andrea and Zisserman, Andrew},
  journal={arXiv preprint arXiv:2110.06207},
  year={2021}
}

@article{dhamija2018reducing,
  title={Reducing network agnostophobia},
  author={Dhamija, Akshay Raj and G{\"u}nther, Manuel and Boult, Terrance},
  journal={Advances in Neural Information Processing Systems},
  volume={31},
  year={2018}
}

@article{LIU2025110947,
title = {Outlier detection using local density and global structure},
journal = {Pattern Recognition},
volume = {157},
pages = {110947},
year = {2025},
issn = {0031-3203},
doi = {https://doi.org/10.1016/j.patcog.2024.110947},
url = {https://www.sciencedirect.com/science/article/pii/S0031320324006988},
author = {Huawen Liu and Shichao Zhang and Zongda Wu and Xuelong Li},
keywords = {Outlier detection, Potential energy, Data density, Data hub, Random walk},
abstract = {Outlier detection, a critical process for enhancing data quality, has been applied to a broad spectrum of real-world applications. This study introduces a novel and effective outlier detection method that incorporates both local density and global structural information. Specifically, we employ the concept of potential energy, a well-established principle in physics, to represent local densities or neighbor distributions of data. Additionally, we also exploit the notion of hubness, a measure explored in network science, to further capture global structural information of data. To facilitate this, we construct a strongly connected digraph by introducing a virtual node along with an associated set of virtual edges. This digraph underpins a tailored Markov random walk process that is used to estimate the hubness scores of data objects. Subsequently, the importance degrees of data objects are estimated according to their potential energies and hubness scores. The data objects with lower importance degrees are deemed to be outliers. Extensive experiments conducted on thirteen publicly accessible real-world datasets against nine popular outlier detection algorithms show that the proposed method achieved encouraging and competitive performance in comparing the state-of-the-art outlier detection algorithms.}
}

@article{ZHANG2024109979,
title = {A vision transformer for fine-grained classification by reducing noise and enhancing discriminative information},
journal = {Pattern Recognition},
volume = {145},
pages = {109979},
year = {2024},
issn = {0031-3203},
doi = {https://doi.org/10.1016/j.patcog.2023.109979},
author = {Zi-Chao Zhang and Zhen-Duo Chen and Yongxin Wang and Xin Luo and Xin-Shun Xu},
keywords = {Vision transformer, Complementary information integration, Region attention, Fine-grained image recognition},
abstract = {Recently, several Vision Transformer (ViT) based methods have been proposed for Fine-Grained Visual Classification (FGVC). These methods significantly surpass existing CNN-based ones, demonstrating the effectiveness of ViT in FGVC tasks. However, there are some limitations when applying ViT directly to FGVC. First, ViT needs to split images into patches and calculate the attention of every pair, which may result in heavy noise calculation during the training phase and unsatisfying performance when handling fine-grained images with complex backgrounds and small objects. Second, complementary information is important for FGVC, but a standard ViT works by using the class token in the final layer for classification which is not enough to extract comprehensive fine-grained information at different levels. Third, the class token fuses the information of all patches in the same manner, in other words, the class token treats each patch equally. However, the discriminative parts should be more critical. To address these issues, we propose ACC-ViT including three novel components, i.e., Attention Patch Combination (APC), Critical Regions Filter (CRF), and Complementary Tokens Integration (CTI). Thereinto, APC pieces informative patches from two images to generate a new image to mitigate the noisy calculation and reinforce the differences between images. CRF emphasizes tokens corresponding to discriminative regions to generate a new class token for subtle feature learning. To extract comprehensive information, CTI integrates complementary information captured by class tokens in different ViT layers. We conduct comprehensive experiments on four widely used datasets and the results demonstrate that ACC-ViT can achieve competitive performance. The source code is available at https://github.com/Hector0426/fine-grained-image-classification-with-vit.}
}

@article{DING2023109532,
title = {An enhanced vision transformer with wavelet position embedding for histopathological image classification},
journal = {Pattern Recognition},
volume = {140},
pages = {109532},
year = {2023},
issn = {0031-3203},
doi = {https://doi.org/10.1016/j.patcog.2023.109532},
author = {Meidan Ding and Aiping Qu and Haiqin Zhong and Zhihui Lai and Shuomin Xiao and Penghui He},
keywords = {Histopathological image classification, Vision transformer, Convolutional neural network, Wavelet position embedding, External multi-head attention},
abstract = {Histopathological image classification is a fundamental task in pathological diagnosis workflow. It remains a huge challenge due to the complexity of histopathological images. Recently, hybrid methods combining convolutional neural networks(CNN) with vision transformers(ViT) are proposed to this field. These methods can well represent the global and local contextual information and achieve excellent classification performances. However, the downsampling operation like max-pooling which ignores the sampling theorem transmits the jagged artifacts into transformer, which would lead to an aliasing phenomenon. It makes the subsequent feature maps focus on the incorrect regions and influences the final classification results. In this work, we propose an enhanced vision transformer with wavelet position embedding to tackle this challenge. In particular, a wavelet position embedding module, which introduces the wave transform into position embedding, is employed to enhance the smoothness of discontinuous feature information by decomposing sequences into amplitude and phase in pathological feature maps. In addition, an external multi-head attention is proposed to replace self-attention in the transformer block with two linear layers. It reduces the cost of computation and excavates potential correlations between different samples. We evaluate the proposed method on three public histopathological classification challenging datasets, and perform a quantitative comparison with previous state-of-the-art methods. The results empirically demonstrate that our method achieves the best accuracy. Furthermore, it has the least parameters and a very low FLOPs. In conclusion, the enhanced vision transformer shows high classification performances and demonstrates significant potential for assisting pathologists in pathological diagnosis.}
}

@inproceedings{odin18iclr,
  title={Enhancing the reliability of out-of-distribution image detection in neural networks},
  author={Liang, Shiyu and Li, Yixuan and Srikant, Rayadurgam},
  booktitle={ICLR},
  year={2018}
}

@article{HUA2025111111,
title = {Weakly Supervised Underwater Object Real-time Detection Based on High-resolution Attention Class Activation Mapping and Category Hierarchy},
journal = {Pattern Recognition},
volume = {159},
pages = {111111},
year = {2025},
issn = {0031-3203},
doi = {https://doi.org/10.1016/j.patcog.2024.111111},
url = {https://www.sciencedirect.com/science/article/pii/S0031320324008628},
author = {Xia Hua and Xiaopeng Cui and Xinghua Xu and Shaohua Qiu and Zhong Li},
keywords = {Underwater image, weakly supervised object detection, hierarchical network, Class Activation Mapping, network attention},
abstract = {Recently, deep learning-based underwater object detection technology has achieved remarkable success. However, the accuracy and completeness of dataset instance annotation are crucial for its success. The quality of underwater images is low, severe objects clustering, and occlusion, acquiring object's annotations demands substantial time and labor costs, while mis annotation and missed annotation can also degrade model performance and limit their application in practical scenarios. To address this issue, this paper presents a novel weakly supervised underwater object real-time detection method, which is divided into two subtasks: weakly supervised object localization and real-time object detection. In the weakly supervised object localization task, we design a novel category hierarchy structure network that integrates the high-resolution attention-class activation mapping algorithm to obtain high-quality object class activation maps, weaken background interference, and obtain more complete object regions. The parameterized spatial loss module is devised to enable the model to escape from local optimal solutions, thus accurately and efficiently obtaining object pseudo-detection annotation boxes. For the real-time object detection task, the single-stage detector YOLOv7 is selected as the basic detection model, and an object perception loss function is designed based on the class activation map to jointly supervise the training process. A method for filtering noisy pseudo-supervision information is proposed to enhance the pseudo-supervision information involved in training. Ablation experiments and multi-method comparison experiments were conducted on the URPC and RUOD datasets, and the results verify the effectiveness of the proposed strategy, and our model exhibits significant advantages in detection performance and detection efficiency compared to current mainstream and advanced models.}
}

@article{XIE2024110172,
title = {GhostFormer: Efficiently amalgamated CNN-transformer architecture for object detection},
journal = {Pattern Recognition},
volume = {148},
pages = {110172},
year = {2024},
issn = {0031-3203},
doi = {https://doi.org/10.1016/j.patcog.2023.110172},
url = {https://www.sciencedirect.com/science/article/pii/S0031320323008695},
author = {Xin Xie and Dengquan Wu and Mingye Xie and Zixi Li},
keywords = {Object detection, Lightweight network design, Feature extraction, CNN-transformer},
abstract = {The lightweight network model has gradually evolved into an important research direction in object detection. Network lightweight design has a variety of research methods, such as quantization, knowledge distillation, and neural architecture search. However, these methods either fail to break through the performance bottleneck of the model itself or require massive training costs. In order to solve these problems, a new object detection model based on CNN-Transformer hybrid feature extraction network called GhostFormer is proposed from the perspective of lightweight network structure design. GhostFormer makes full use of the advantages of local modeling of CNN and global modeling of Transformer, not only effectively reducing the complexity of the convolution model but also breaking through the limitation of Transformer’s lack of inductive bias. Finally, better transfer results are obtained in downstream tasks. Experiments show that the model is less than half as computationally expensive as YOLOv7 on the Pascal VOC dataset, with only about 3 % mAP@0.5 loss, and 9.7% mAP@0.5:0.95 improvement on the MS COCO dataset compared with GhostNet.}
}

@article{zhang2024morphoseg,
  title={MorphoSeg: An Uncertainty-Aware Deep Learning Method for Biomedical Segmentation of Complex Cellular Morphologies},
  author={Tianhao Zhang and Heather J McCourty and Berardo M Sanchez-Tafolla and Anton Nikolaev and Lyudmila S Mihaylova},
  journal={arXiv preprint arXiv:2409.17110},
  year={2024}
}

@article{GUO2024110491,
title = {UCTNet: Uncertainty-guided CNN-Transformer hybrid networks for medical image segmentation},
journal = {Pattern Recognition},
volume = {152},
pages = {110491},
year = {2024},
issn = {0031-3203},
doi = {https://doi.org/10.1016/j.patcog.2024.110491},
url = {https://www.sciencedirect.com/science/article/pii/S0031320324002425},
author = {Xiayu Guo and Xian Lin and Xin Yang and Li Yu and Kwang-Ting Cheng and Zengqiang Yan},
keywords = {CNN-Transformer hybrid, Uncertainty, Functional overlap, Masked self-attention, Medical image segmentation},
abstract = {Transformer, born for long-range dependency establishment, has been widely studied as a complementary of convolutional neural networks (CNNs) in medical image segmentation. However, existing CNN-Transformer hybrid approaches simply pursue implicit feature fusion without considering their underlying functional overlap. Medical images typically follow stable anatomical structures, making convolution capable of handling most segmentation targets. Without differentiation, enforcing transformers to operate self-attention for all image patches would result in severe redundancy, hindering global feature extraction. In this paper, we propose a simple yet effective hybrid network named UCTNet where transformers only focus on establishing global dependency for CNN’s unreliable regions predicted through uncertainty estimation. In this way, CNN and transformer are explicitly fused to minimize functional overlap. More importantly, with fewer regions to handle, UCTNet is of better convergence to learn more robust feature representations for hard examples. Extensive experiments on publicly-available datasets demonstrate the superiority of UCTNet against the state-of-the-art approaches, achieving 89.44%, 92.91%, and 91.15% in Dice similarity coefficient on Synapse, ACDC, and ISIC2018 respectively. Furthermore, such a CNN-Transformer hybrid strategy is highly extendable to other frameworks without introducing additional computational burdens. Code is available at https://github.com/innocence0206/UCTNet.}
}

@inproceedings{confgan18nipsw,
  title={Building robust classifiers through generation of confident out of distribution examples},
  author={Sricharan, Kumar and Srivastava, Ashok},
  booktitle={NeurIPS-W},
  year={2018}
}

@inproceedings{du2022unknown,
      title={Unknown-Aware Object Detection: Learning What You Don’t Know from Videos in the Wild}, 
      author={Du, Xuefeng and Wang, Xin and Gozum, Gabriel and Li, Yixuan},
      booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
      year={2022}
}

==> sec/0_abstract.tex <==
% \begin{abstract}
% Vision Transformers (ViTs) have shown remarkable performance in various vision tasks, yet their efficacy in Out-of-Distribution (OOD) detection remains underexplored. In this work, we introduce the Prior-augmented Vision Transformer (\model), a novel framework that merges empirical evidence from an In-Distribution (ID) dataset with encoded prior knowledge, offering a scalable solution for enhancing OOD robustness. This innovative approach enables \model to effectively differentiate between ID and OOD data, thus improving its detection capabilities. In addition, we introduce a novel OOD detection measurement, termed Prior Cross Entropy (PCE), which effectively gauges the discrepancy between the model's output probabilities and the prior distribution, further enriching our framework's capability in OOD detection. This metric not only strengthens OOD detection but also confirms the practicality and scalability of \model in tackling real-world challenges in computer vision, especially those involving distribution variances. Extensive quantitative and qualitative evaluations on prominent OOD benchmarks like CIFA100 and IMAGENET demonstrate that \model significantly surpasses existing state-of-the-art methods in OOD detection. This underscores \model's potential as a versatile and effective tool in advancing the field of computer vision research.
% \end{abstract}

\begin{abstract}
% Vision Transformers (ViTs) have shown remarkable performance in various vision tasks, yet their robustness and inductive bias concerning data distribution shifts remain underexplored. In this work, we propose the Prior-augmented Vision Transformer (\model), a novel and scalable framework for Out-of-Distribution (OOD) detection. 
% Comparing to existing state-of-the-art OOD detection methods, \model innovatively integrates empirical prior evidence from the In-Distribution (ID) dataset with encoded prior knowledge, enhancing OOD robustness in ViT models without requiring additional data modeling, generation methods, or structural modifications. \model detect the OOD data by modelling the differences between the prior logits output by a pre-trained model on ID data  and the predicted class through the prior guidance. Our extensive experiments on large-scale ImageNet benchmark demonstrate that \model provides a significant performance improvement compared to the existing state-of-the-art OOD detection methods. Furthermore, through detailed analyses, ablation studies, and discussions, we elucidate how \model can serve as a strategic planning tool for targeting specific challenges in managing large vision models, opening new avenues in the domain of OOD detection.

Vision Transformers (ViTs) have achieved remarkable success over various vision tasks, yet their robustness against data distribution shifts and inherent inductive biases remain underexplored. To enhance the robustness of ViT models for image Out-of-Distribution (OOD) detection, we introduce a novel and generic framework named Prior-augmented Vision Transformer (\model). \model identifies OOD samples by quantifying the divergence between the predicted class logits and the prior logits obtained from pre-trained models. Unlike existing state-of-the-art OOD detection methods, \model shapes the decision boundary between ID and OOD by utilizing the proposed prior guide confidence, without requiring additional data modeling, generation methods, or structural modifications. Extensive experiments on the large-scale ImageNet benchmark demonstrate that \model significantly outperforms existing state-of-the-art OOD detection methods. Additionally, through comprehensive analyses, ablation studies, and discussions, we show how \model can strategically address specific challenges in managing large vision models, paving the way for new advancements in OOD detection.

% precisely differentiate OOD from ID data by evaluating the entropy disparity between encoded prior knowledge and the model's output probabilities through our proposed Prior Cross Entropy score. 


% We demonstrate that our proposed \model shown good performance on on large-scale OOD benchmarks, including CIFAR-100 and IMAGENET. 

% proving the efficacy and versatility of \model. 

\end{abstract}

% \begin{abstract}
% Vision Transformers (ViTs) have demonstrated remarkable performance across various vision tasks, yet their robustness and inductive biases in response to data distribution shifts remain underexplored. In this work, we introduce the Prior-Augmented Vision Transformer (\model), a novel and scalable framework for Out-of-Distribution (OOD) detection. \model innovatively integrates empirical prior evidence from the In-Distribution (ID) dataset with encoded prior knowledge, enhancing OOD robustness in ViT models without requiring additional data modeling, generation methods, or structural modifications, unlike existing state-of-the-art OOD detection methods. Our comprehensive experiments on large-scale OOD benchmarks, including CIFAR-100 and IMAGENET, demonstrate that \model excels by employing a Prior Cross Entropy (PCE) strategy. This approach precisely distinguishes OOD from ID data by quantifying the entropy difference between encoded prior knowledge and the model's output probabilities. Furthermore, through in-depth analyses, ablation studies, and discussions, we highlight \model's potential as a strategic tool for addressing specific challenges in managing large vision models, thereby paving new paths in OOD detection research.
% \end{abstract}
% \begin{abstract}
% Vision Transformers (ViTs) have demonstrated exceptional performance across a range of vision tasks, yet their robustness and inductive biases in response to data distribution shifts remain insufficiently explored. In this work, we introduce the Prior-Augmented Vision Transformer (\model), a novel and scalable framework for Out-of-Distribution (OOD) detection. Unlike existing state-of-the-art methods, \model seamlessly integrates empirical prior evidence from the In-Distribution (ID) dataset with encoded prior knowledge, thus enhancing OOD robustness in ViT models without the need for additional data modeling, generation techniques, or structural changes. Our comprehensive experiments on major OOD benchmarks, including CIFAR-100 and IMAGENET, show that \model effectively distinguishes OOD from ID data by quantifying the entropy difference between encoded prior knowledge and the model's output probabilities via a Prior Cross Entropy (PCE) method. Moreover, through in-depth analyses, ablation studies, and discussions, we highlight how \model acts as a strategic tool for addressing specific challenges in managing large vision models, thereby paving new pathways in OOD detection research.
% \end{abstract}


==> sec/3_method_copy.tex <==
\begin{figure*}[t]
    \centering
	% \includegraphics[width=\textwidth,trim=1.3 1.3 1.3 1.3,clip]{fig/method.pdf}
    \includegraphics[width= 1.0\textwidth]{fig/model2.pdf} 
    \caption{Framework of our proposed \model. \model is trained on ID data $\mathcal{D}_{\text{in}}^{\text{train}}$ with a prior token $\mathbf{T}_{\text{prior}}$ containing the prior knowledge $\mathbf{p}$, indicated by green blocks and arrows. 
    Orange blocks represent the inference process with OOD data  $\mathcal{D}_{\text{out}}^{\text{test}}$. The prior model $\theta_{prior}$ supplies priors for the prior token. PCE is employed to differentiate between ID and OOD data. Other components, including position embeddings, the classification (cls) token and the flattening of image patches follow the implementation of the vanilla ViT~\cite{dosovitskiy2020image}.} 
    \label{fig:method}
\end{figure*}

\section{Methodology} \label{sec:method}
% This section lays the foundation of our approach, starting with the problem setup (Section.~\ref{sec:preli}) to establish the necessary background. We then offer a comprehensive overview of our \model (Section.~\ref{sec:overview}), detailing its architecture and functionality with Figure.~\ref{fig:method}. Finally, we explore our OOD scoring mechanism, particularly emphasizing the role of the PCE score in differentiating OOD instances (Section.~\ref{sec:PCE}).


% \subsection{Problem Setup} \label{sec:preli}
% In the context of image classification, let $\mathcal{X} = \mathbb{R}^d$ represent the input space, with $\mathcal{Y} = \{1, \ldots, K\}$ as the finite set of possible labels. The training dataset $\mathcal{D}_{\text{in}}^{\text{train}} = \{(\mathbf{x}_i, y_i)\}_{i=1}^n$ comprises pairs $(\mathbf{x}_i, y_i)$ where $\mathbf{x}_i \in \mathcal{X}$ is an image and $y_i \in \mathcal{Y}$ its associated label. In the context of an image classification task, the classification function denoted as $f_\theta: \mathcal{X} \rightarrow \mathbb{R}^d$, initialized by parameter $\theta$, is trained to predict a label $\widehat{y}$ for each image $\mathbf{x}$.

% % where $\widehat{y} = \argmax_{k} f_\theta^{(k)}(\mathbf{x})$ and $f_\theta^{(k)}$ represents the output for the $k$-th class.

% For testing, we use the dataset $\mathcal{D}_{\text{out}}^{\text{test}} = \{(\mathbf{x}_j, y_j)\}_{j=1}^m$ to evaluate the model's performance on unseen data. The objective is to train a model $f_\theta$ to distinguish OOD inputs, characterized by labels $y \notin \mathcal{Y}$. This can be achieved by building a detector $f$ such that $f(x_{1},...,x_{n})=1$ for all $i$, where $p(x_{i})\geq \delta$, and $f(x_{1},...,x_{n})=0$ for all $i$ where  $p(x_{i})\leq \delta$, with $\delta$ being the threshold defining the model's capability boundary. OOD detection is essentially a binary classification problem where, at test time, the goal is to determine whether an input is ID or OOD. We define a function $g_\theta: \mathcal{X} \rightarrow \{\text{in}, \text{out}\}$ for this mapping, which classifies inputs as either ID or OOD.
% \subsection{Problem Formulation} \label{sec:preli}
% In the context of image classification, let $\mathcal{X} = \mathbb{R}^d$ denote the input space, and $\mathcal{Y} = \{1, \ldots, K\}$ the finite set of possible labels for $K$ classes. The training dataset, $\mathcal{D}_{\text{in}}^{\text{train}} = \{(\mathbf{x}_i, y_i)\}_{i=1}^n$, consists of pairs $(\mathbf{x}_i, y_i)$ with a classification function $f_\theta: \mathcal{X} \rightarrow \mathbb{R}^K$ predicting class scores. The predicted label $\widehat{y}$ is obtained as $\widehat{y} = \argmax_{k} f_\theta^{(k)}(\mathbf{x})$, signifying the selection of the class with the highest score.

% For unseen data testing, the objective extends to training a model capable of distinguishing OOD inputs $\mathcal{D}_{\text{out}}^{\text{test}} = \{(\mathbf{x}_j, y_j)\}_{j=1}^m$, characterized by labels $y \notin \mathcal{Y}$. To achieve this, a binary classification approach is proposed where a detector $g_\theta: \mathcal{X} \rightarrow \{\text{in}, \text{out}\}$ is introduced. This function distinguishes between ID data and OOD data based on a defined threshold $\gamma$, which establishes the model's confidence threshold for classifying inputs as either ID or OOD.

\subsection{Preliminaries} \label{sec:preli}
In the context of image classification, let \( \mathcal{X} = \mathbb{R}^d \) represent the input space, and \( \mathcal{Y} = \{1, \ldots, K\} \) denote the finite set of labels for \( K \) classes. The training dataset \( \mathcal{D}_{\text{in}}^{\text{train}} = \{(\mathbf{x}_i, y_i)\}_{i=1}^n \) consists of pairs \( (\mathbf{x}_i, y_i) \), where a classification function \( f_\theta: \mathcal{X} \rightarrow \mathbb{R}^K \) predicts class scores. The predicted label \( \widehat{y} \) is obtained as \( \widehat{y} = \argmax_{k} f_\theta^{(k)}(\mathbf{x}) \), corresponding to the class with the highest score.

For testing on unseen data, the objective is to train a model capable of distinguishing OOD inputs \( \mathcal{D}_{\text{out}}^{\text{test}} = \{(\mathbf{x}_j, y_j)\}_{j=1}^m \), where labels \( y_j \) do not belong to \( \mathcal{Y} \). To this end, a binary classification approach, also known as The decision rule for OOD detection, is employed:

\begin{equation}
    \mathbf{x} = \left\{
    \begin{array}{ll}
        \text{ID} & \text{if } S(\mathbf{x};\theta) \geq \gamma, \\
        \text{OOD} & \text{if } S(\mathbf{x};\theta) < \gamma,
    \end{array}
    \right.
    \label{eq:ood_rule}
\end{equation}

\noindent where the threshold \( \gamma \) is selected to ensure high classification accuracy for ID data, typically set at 95\%. The score \( S(\mathbf{x};\theta) \), also known as 'confidence', represents the classifier-based detection score.


% For testing, the dataset $\mathcal{D}_{\text{out}}^{\text{test}} = \{(\mathbf{x}_j, y_j)\}_{j=1}^m$ is utilized to assess the model's performance on unseen data. The objective extends to training a model capable of distinguishing OOD inputs, characterized by labels $y \notin \mathcal{Y}$. To achieve this, a binary classification approach is proposed where a detector $g_\theta: \mathcal{X} \rightarrow \{\text{in}, \text{out}\}$ is introduced. This function distinguishes between In-Distribution (ID) and OOD data based on a defined threshold $\gamma$, which establishes the model's confidence threshold for classifying inputs as either ID or OOD.

% \subsection{Prior-augmented Vision Transformer} \label{sec:overview}
% The architecture of PViT is illustrated in Figure.~\ref{fig:method}. 
% The frameworks is following the vanilla ViT~\cite{dosovitskiy2020image}.
% The foundational ViT processes a sequence of flattened 2D patches $\mathbf{x}_p \in \mathbb{R}^{N \times (P^2 \cdot C)}$, obtained from the image $\mathbf{x} \in \mathbb{R}^{H \times W \times C}$ through a mapping to patch embeddings. Here, $(H, W)$ denotes the resolution of the original image, $C$ represents the number of channels, $(P, P)$ specifies the resolution of each patch, and $N = \frac{HW}{P^2}$ is the number of patches, serving as the effective sequence length for the Transformer. 
% An additional learnable embedding, $\mathbf{z}_0^0 = \mathbf{x}_{\text{class}}$, is appended to the patch sequence, with its final state at the output of the Transformer encoder, $\mathbf{z}_L^0$, acting as the image representation $\mathbf{y}$.

% In our proposed method, the prior knowledge \(\pi\) is encoded as logits vector \(\mathbf{p}\), where each element \(p_i = \log \left( \frac{P(i)}{1 - P(i)} \right)\) for each class \(i\) in a set of \(K\) classes. These logits are obtained from a pre-trained model, parameterized by \(\theta_{\text{prior}}\), serving as the prior model. The prior model uses the ID training data \(\mathcal{D}_{\text{in}}^{\text{train}} = \{(\mathbf{x}_i, y_i)\}_{i=1}^n\) to compute the logits vector \(\mathbf{p}\), where \(f_{\theta_{\text{prior}}}(y_i|\mathcal{D}_{\text{in}}^{\text{train}})\) calculates the logits for the prior distribution. The overall training and testing process is summurized in Algorithm~\ref{alg:prior-augmented}.

\subsection{Prior-augmented Vision Transformer} \label{sec:overview}
The architecture of PViT is illustrated in Figure.~\ref{fig:method}. The implemntation of PViT is following the foundational structure of the vanilla ViT~\cite{dosovitskiy2020image}. The conventional ViT transforms an input image $\mathbf{x} \in \mathbb{R}^{H \times W \times C}$ into a sequence of flattened 2D patches $\mathbf{x}_p \in \mathbb{R}^{N \times (P^2 \cdot C)}$, where $(H, W)$ is the resolution of the original image, $C$ is the number of channels, $(P, P)$ defines the resolution of each patch, and $N = \frac{HW}{P^2}$ represents the total number of patches, effectively determining the sequence length for the Transformer. Same with the implementation of the vanilla ViT, a learnable embedding $\mathbf{z}_0^0$, which is initially set to $\mathbf{x}_{\text{class}}$, is serverd as the class embedding aimimg to capture the global image representation and is updated throughout the transformer layers. Its final state, $\mathbf{z}_L^0 \in \mathbb{R}^{1 \times D}$, after $L$ layers of the Transformer encoder, serves as the aggregated image representation, denoted by $\mathbf{y} \in \mathbb{R}^{D}$. Here, $D$ is the dimensionality of the embedding space, and $L$ indicates the number of Transformer layers.

Given a prior model $f_{\theta_{\text{prior}}}$ parameterized by $\theta_{\text{prior}}$, we use the function $f_{\theta_{\text{prior}}}(y_i|\mathcal{D}_{\text{in}}^{\text{train}})$ to compute the logits vector $\mathbf{p} \in \mathbb{R}^{K}$. Each element $p_i = \log \left( \frac{P(i)}{1 - P(i)} \right)$ represents the log odds of the prior probability $P(i)$ for each class $i$ in a set of $K$ classes. The choice of the prior model is flexible; it can be either a ViT or a CNN, contingent upon its proficiency in delivering relatively accurate estimations on images that act as priors for \model. 
% In our empirical investigations, we opted for both ResNet and ViT as exemplars of prior models, with detailed considerations and results delineated in Section.~\ref{sec:training_details}. %The training and testing procedures are summarized in Algorithm~\ref{alg:prior-augmented}.

% Our method encodes prior knowledge $\pi$ into a logits vector $\mathbf{p} \in \mathbb{R}^{K}$, where each element $p_i = \log \left( \frac{P(i)}{1 - P(i)} \right)$ for each class $i$ within a set of $K$ classes. These logits are derived from a pre-trained model parameterized by $\theta_{\text{prior}}$, referred to as the prior model, utilizing the ID training dataset $\mathcal{D}_{\text{in}}^{\text{train}} = \{(\mathbf{x}_i, y_i)\}_{i=1}^n$. The choice of the prior model is flexible; it can be either a ViT or a CNN, contingent upon its proficiency in delivering relatively accurate estimations on images that act as priors for \model. In our empirical investigations, we opted for both ResNet and ViT as exemplars of prior models, with detailed considerations and results delineated in Section.~\ref{sec:training_details}. The training and testing procedures are summarized in Algorithm~\ref{alg:prior-augmented}.
% The function $f_{\theta_{\text{prior}}}(y_i|\mathcal{D}_{\text{in}}^{\text{train}})$ computes the logits vector $\mathbf{p}$, representing the prior distribution over the classes.

% \vspace{1mm}
% \begin{algorithm}[htbp]
% % \SetAlgoLined
% \textbf{Input:} ID training data $\mathcal{D}_{\text{in}}^{\text{train}} = \{(\mathbf{x}_i, y_i)\}_{i=1}^n$, initial model parameters $\theta$ for learning the image-conditioned latent space, a prior model $f_{\theta_{\text{prior}}}$ for providing the prior logits vector $\mathbf{p}$ based on the ID data, OOD test data $\mathcal{D}_{\text{out}}^{\text{test}} = \{(\mathbf{x}_j)\}_{j=1}^m$. \\
% \textbf{Output:} A model $f_\theta$ that provides the predicted classes given the input image and the priors. \\
% \textbf{Phase 1: Training the \model.} \\
%     1. Feed the ID training data $\mathcal{D}_{\text{in}}^{\text{train}}$ into the prior model $\theta_{\text{prior}}$ to obtain the prior logits vector $\mathbf{p} = f_{\theta_{\text{prior}}}(y_i|\mathcal{D}_{\text{in}}^{\text{train}})$. \\
%     2. Embed the prior logits vector $\mathbf{p}$ as an extra token $\mathbf{t}_{\text{prior}}$ by Eq.~\eqref{eq:token}, replicate it across the batch to form $\mathbf{T}_{\text{prior}}$ to ensure dimensional consistency through Eq.~\eqref{eq:rep}, and concatenate it with the positionally embedded image tokens $\mathbf{E}_{\text{pos}}$. Train the \model using the feed-forward processes defined from Eq.~\eqref{eq:start} to Eq.~\eqref{eq:loss}. \\
% \textbf{Phase 2: Inference for OOD detection.} \\
%     1. Feed the \model with the OOD test data $\mathcal{D}_{\text{out}}^{\text{test}}$ along with the predicted prior logits vector $\mathbf{p}$ computed by $f_{\theta_{\text{prior}}}(y_i|\mathcal{D}_{\text{out}}^{\text{test}})$. \\
%     2. Calculate the OOD score $S(\mathbf{x}_j;\theta)$ for each test sample using Eq.~\eqref{eq:ood_score}. \\
%     3. Classify the data as ID or OOD using the OOD scoring rule defined in Eq.~\eqref{eq:ood_rule}.
%  \caption{\model: OOD Detection by Prior-augmented Vision Transformer}
%  \label{alg:prior-augmented}
% \end{algorithm}
% The performance of the model is then evaluated on Out-of-Distribution (OOD) test data $\mathcal{D}_{\text{out}}^{\text{test}} = \{(\mathbf{x}_j, y_j)\}_{j=1}^m$.
\vspace{2mm}
\noindent\textbf{Prior Token Integration.} Incorporating contextual priors into the ViT architecture, we present a methodology for injecting logits from a pre-trained image classification model as a distinct entity, termed the \textit{prior token}. This token $\mathbf{t}_{\text{prior}} \in \mathbb{R}^{1 \times D}$ is designed to augment the transformer with additional, non-spatial context, thereby enriching the model's inference capabilities without perturbing the spatial coherence of the input image patches. 

Given an input image, the model first computes patch embeddings $\mathbf{E}_{\text{patches}} \in \mathbb{R}^{N \times D}$, where $N$ represents the number of patches. A class token $\mathbf{t}_{\text{cls}} \in \mathbb{R}^{1 \times D}$ is then prepended to this sequence of embeddings. Positional encodings $\mathbf{P}_{\text{pos}} \in \mathbb{R}^{(N+1) \times D}$ are added to provide the sequence with spatial information, resulting in the final sequence of embeddings $\mathbf{E}_{\text{pos}} = [\mathbf{t}_{\text{cls}}; \mathbf{E}_{\text{patches}}] + \mathbf{P}_{\text{pos}}$ To integrate prior knowledge, the logits vector $\mathbf{p} \in \mathbb{R}^{C}$ from a pre-trained classifier is normalized using the softmax function. These normalized logits are then mapped into the embedding dimension $D$ to form the prior token $\mathbf{t}_{\text{prior}}$:

% $\mathbf{E}_{\text{pos}}$,
% defined as:

% \begin{equation}
% \mathbf{E}_{\text{pos}} = [\mathbf{t}_{\text{cls}}; \mathbf{E}_{\text{patches}}] + \mathbf{P}_{\text{pos}}.
% \end{equation}
% and $D$ is the embedding dimension
% To integrate prior knowledge, the logits vector $\mathbf{p} \in \mathbb{R}^{C}$ from a pre-trained classifier is normalized using the softmax function. These normalized logits are then mapped into the embedding dimension $D$ to form the prior token $\mathbf{t}_{\text{prior}}$:
% \begin{equation}
% \mathbf{t}_{\text{prior}} = \mathbf{W}_{\text{proj}} \cdot \text{softmax}(\mathbf{p}),
% \end{equation}
%
\begin{equation}
\mathbf{t}_{\text{prior}} = \mathbf{W}_{\text{proj}} \cdot (\mathbf{p}),
\label{eq:token}
\end{equation}
%
\noindent where $\mathbf{W}_{\text{proj}} \in \mathbb{R}^{D \times C}$ is a projection matrix designed to transform the class-wise priors into the embedding space, aligning them dimensionally with the patch embeddings. This transformation facilitates the incorporation of class-specific prior knowledge into the model.

The prior token is scaled by a factor $\alpha \in \mathbb{R}$, a hyperparameter, to modulate the influence of prior knowledge relative to the embeddings from the input image. This scaling aims to balance the model's attention between the prior token and the image-derived embeddings, optimizing the model's performance. An extensive ablation study on $\alpha$'s impact is detailed in Section~\ref{sec:scale}. The scaled prior token $\mathbf{t}_{\text{prior}}$ is then replicated across the batch, resulting in:
\begin{equation}
\mathbf{T}_{\text{prior}} = \alpha \cdot \mathbf{t}_{\text{prior}} \otimes \mathbf{1}_{B \times 1 \times D},
\label{eq:rep}
\end{equation}
where $B$ denotes the batch size, ensuring that each instance in the batch is augmented with the transformed prior knowledge.

% Given an input image, the model first computes patch embeddings $\mathbf{E}_{\text{patches}} \in \mathbb{R}^{N \times D}$, where $N$ is the number of patches and $D$ is the embedding dimension. A class token $\mathbf{t}_{\text{cls}} \in \mathbb{R}^{1 \times D}$ is then prepended to this sequence of embeddings. Positional encodings $\mathbf{P}_{\text{pos}} \in \mathbb{R}^{(N+1) \times D}$ are subsequently added to endow the sequence with spatial information. This results in the final sequence of embeddings $\mathbf{E}_{\text{pos}}$, defined as:
% \begin{equation}
% \mathbf{E}_{\text{pos}} = [\mathbf{t}_{\text{cls}}; \mathbf{E}_{\text{patches}}] + \mathbf{P}_{\text{pos}}.
% \end{equation}

% The integration of prior knowledge into the model involves normalizing the logits vector $\mathbf{p} \in \mathbb{R}^{C}$ from a pre-trained classifier using the softmax function. These normalized logits are then projected into the embedding space to form the prior token $\mathbf{t}_{\text{prior}}$:
% \begin{equation}
% \mathbf{t}_{\text{prior}} = \mathbf{W}_{\text{proj}} \cdot \text{softmax}(\mathbf{p}),
% \end{equation}

% where $\mathbf{W}_{\text{proj}} \in \mathbb{R}^{C \times D}$ is the projection matrix used for transform the priors into the same dimentions as the patch inputs, where the . 

% The prior token is scaled by a factor $\alpha \in \mathbb{R}$, set as a hyperparameter, to balance the \model's attention between the prior token and other input tokens, optimizing performance. A comprehensive ablation study on $\alpha$ is presented in Section.~\ref{sec:scale}. The token $\mathbf{t}_{\text{prior}}$ is then replicated across the batch of data:
% \begin{equation}
% \mathbf{T}_{\text{prior}} = \alpha \cdot \mathbf{t}_{\text{prior}} \otimes \mathbf{1}_{B \times 1 \times D},
% \end{equation}

where $B$ denotes the batch size. The operation $\otimes$ represents the outer product with a vector of ones, effectively broadcasting $\mathbf{t}_{\text{prior}}$ across the batch. This broadcasting results in $\mathbf{T}_{\text{prior}}$, which encapsulates the prior token for the entire batch.
Finally, the batch-level prior token $\mathbf{T}_{\text{prior}}$ is appended to the positionally encoded sequence to form the complete input $\mathbf{T} = [\mathbf{E}_{\text{pos}}; \mathbf{T}_{\text{prior}}]$ for the Transformer.
% \begin{equation}
% \mathbf{T} = [\mathbf{E}_{\text{pos}}; \mathbf{T}_{\text{prior}}].
% \end{equation}

The concatenated sequence $\mathbf{T}$ is processed through the Transformer encoder layers to yield the final representations. Our model follows the architecture of the vanilla ViT~\cite{dosovitskiy2020image}, employing multi-headed self-attention (MSA)~\cite{vaswani2017attention} (Eq.~\eqref{eq:MSA}) and multi-layer perceptron (MLP) blocks (Eq.~\eqref{eq:MLP}). Layer normalization (LN) is applied before each block (Eq.~\eqref{eq:final_representation}), as described in the following equations:
\begin{align}
    \mathbf{Z}_0 &= \mathbf{T}, \label{eq:start}\\
    \mathbf{Z}^\prime_{\ell} &= \text{MSA}(\text{LN}(\mathbf{Z}_{\ell-1})) + \mathbf{Z}_{\ell-1}, \quad \ell = 1 \ldots L, \label{eq:MSA} \\ 
    \mathbf{Z}_{\ell} &= \text{MLP}(\text{LN}(\mathbf{Z}^\prime_{\ell})) + \mathbf{Z}^\prime_{\ell}, \quad \ell = 1 \ldots L,  \label{eq:MLP} \\
    \mathbf{Y} &= \text{LN}(\mathbf{Z}_L[0]),  \label{eq:final_representation}
\end{align}

\noindent where $\mathbf{Z}_L[0]$ represents the final layer's class token representation. The output $\mathbf{Y} \in \mathbb{R}^{D}$ serves as the input to a classifier head for the task at hand.

% In the context of image classification, the primary training objective for \model is to minimize the divergence between the model's predicted distribution and the true label distribution. This goal is achieved through cross-entropy minimization, formulated as:

% \begin{equation}
%     \theta^* = \arg\min_{\theta} - \sum_{i=1}^n \log P_{\text{\model}}(y_i | x_i, D, \pi; \theta),
%     \label{eq:loss}
% \end{equation}

% where \( \theta \) denotes the parameters of \model, \( y_i \) represents the true labels, \( x_i \) the input data, \( D \) the dataset, and \( \pi \) the prior information. 

In the context of image classification, the primary training objective for \model is to minimize the divergence between the model's predicted distribution and the true label distribution. Our overall training objective is achieved through the minimization of the cross-entropy loss function~\( \mathcal{L}_\text{CE} \), which is formulated as:

\begin{equation}
    \mathcal{L}_\text{CE} = -\sum_{i=1}^n \log P_{\text{\model}}(y_i | x_i, \mathcal{D}, \pi; \theta),
    \label{eq:loss}
\end{equation}

% The optimal model parameters \( \theta^* \) are obtained by minimizing this loss function:

% \begin{equation}
%     \theta^* = \arg\min_{\theta} \mathcal{L}_\text{CE}(\theta),
% \end{equation}

\noindent where \( \theta \) represents the parameters of \model, \( y_i \) the true labels, \( x_i \) the input data, \( \mathcal{D} \) the dataset, and \( \pi \) the prior information. 


\subsection{Prior Guide Energy for OOD Detection} \label{sec:PCE}
Given a base confidence score function \( S_{\text{base}}(\mathbf{x}; \theta) \), we propose a Prior Guide Energy (PGE) method to effectively differentiate between ID and OOD data by incorporating prior knowledge:

\begin{equation}
    S_{\text{PGE}}(\mathbf{x}; \theta) = S_{\text{base}}(\mathbf{x}; \theta) \cdot G(\mathbf{x}; \theta, \theta_{\text{prior}}),
    \label{eq:overall_score}
\end{equation}

\noindent where \( G(\mathbf{x}; \theta, \theta_{\text{prior}}) \) is the \textit{guidance term}, designed to measure the similarity between the prior embeddings and the outputs of \model. Cross entropy, widely recognized as an effective and direct method for training targets in classification tasks, is introduced here as the optimal guidance term by taking the prior logits and the predicted class as inputs:

\begin{equation}
    G(\mathbf{x}; \theta, \theta_{\text{prior}}) = -\sum_{k=1}^{K} y_k \log\left(q_k(\mathbf{x}; \theta_{\text{prior}})\right),
    \label{eq:guidance_term}
\end{equation}

\noindent where \( q_k(\mathbf{x}; \theta_{\text{prior}}) \) is the probability of class \( k \) based on the prior logits, and \( y_k \) is the predicted class by \model. This guidance term measures the dissimilarity between the model’s predictions and the prior distribution. A higher cross entropy score indicates greater alignment with the prior distribution, suggesting that the data are likely ID, while a lower score suggests potential OOD data. Cross entropy is one of the guidance terms we introduced; other optional guidance terms for measuring similarity are discussed in the Ablation Study section.

For the base confidence score, we use the Free Energy~\cite{liu2020energy}:
\begin{equation}
    S_{\text{base}}(\mathbf{x}; \theta) = -\log \sum_{k=1}^{K} e^{f_k(\mathbf{x}; \theta)},
\end{equation}

\noindent where \( f_k(\mathbf{x}) \) are the logits for class \( k \) output by the pre-trained prior model. Free Energy has been shown to be effective for OOD detection~\cite{liu2020energy}, as it provides a confidence measure in the model's predictions. High energy indicates low confidence (a more spread-out distribution), while low energy indicates high confidence (a more peaked distribution).

\begin{prop}
\label{thm:theory}
Let \( S_{\text{PGE}}(\mathbf{x}; \theta) = S_{\text{base}}(\mathbf{x}; \theta) \cdot G(\mathbf{x}; \theta, \theta_{\text{prior}}) \). If \( \mathbf{x} \in D_{\text{in}} \), then \( S_{\text{PGE}}(\mathbf{x}; \theta) \) is high, i.e., \( S_{\text{PGE}}(\mathbf{x}; \theta) > \gamma \), where \( \gamma \) is a threshold value. Conversely, if \( \mathbf{x} \in D_{\text{out}} \), then \( S_{\text{PGE}}(\mathbf{x}; \theta) \) is low, i.e., \( S_{\text{PGE}}(\mathbf{x}; \theta) < \gamma \).
\end{prop}

This proposition asserts that a high PGE score indicates ID data, while a low PGE score indicates OOD data. This behavior is due to the alignment between predicted logits and the prior distribution, as captured by the cross entropy term. The Free Energy component provides a confidence measure, with higher energy indicating lower confidence and vice versa. Detailed proof is provided in the Appendix.

% This proposition states that the higher PGE score indicating the ID and lower indicationg the OOD. That can be simply because A higher cross entropy score indicates that the predicted logits are more aligned with the prior distribution, suggesting that the data are likely ID. Conversely, a lower cross entropy score suggests a deviation from the prior distribution, indicating potential OOD data. The Free Energy has been proven effective for OOD detection~\cite{liu2020energy}, as it provides a measure of confidence in the model's predictions. High energy indicates less confidence (a more spread-out distribution), while low energy indicates high confidence (a more peaky distribution).  Proof is given in the Appendix.


% To further enhance the ability to differentiate ID data from OOD data, we introduce a confidence partition known as the Free Energy $E(\mathbf{x};\theta) = -\log \sum_{k=1}^K e^{f_k(\mathbf{x};\theta_\text{prior})}$, where \( f_k(\mathbf{x};\text{prior}) \) are the logits output by the prior model for class \( k \). The Free Energy has been proven effective for OOD detection~\cite{liu2020energy}, as it provides a measure of confidence in the model's predictions. High energy indicates less confidence (a more spread-out distribution), while low energy indicates high confidence (a more peaky distribution).


% Compared to a standard Cross Entropy loss, ECE measures the dissimilarity between the prior distribution and the model's predicted probability distribution.: 
% \begin{equation}
%     S_{\text{ECE}}(\mathbf{x};\theta) = S_{\text{}}(\mathbf{x};\theta) \cdot E(\mathbf{x};\theta),
%     \label{eq:overall_score}
% \end{equation} 
% %
% \begin{equation}
%     S_{\text{ECE}}(\mathbf{x};\theta) = -\sum_{k=1}^K p_{\theta, \text{prior},k}(\mathbf{x}) \log q_k(\mathbf{x};\theta),
%     \label{eq:ood_score}
% \end{equation}

% Compared to a standard Cross Entropy loss, ECE measures the dissimilarity between the prior distribution and the model's predicted probability distribution. A lower ECE score indicates that the predicted logits are more aligned with the prior distribution, suggesting that the data are likely ID. Conversely, a higher ECE score suggests a deviation from the prior distribution, indicating potential OOD data. More details of the ablation study on OOD scores are presented in Section~\ref{sec:score}.

% Formally, the ECE score is defined as:
% \begin{equation}
%     S_{\text{ECE}}(\mathbf{x};\theta) = -\sum_{k=1}^K p_{\theta, \text{prior},k}(\mathbf{x}) \log q_k(\mathbf{x};\theta),
%     \label{eq:ood_score}
% \end{equation}
% \noindent where \( p_{\theta, \text{prior},k}(\mathbf{x}) \) denotes the prior probability of class \( k \) given the input \( \mathbf{x} \), as determined by the prior model. \( q_k(\mathbf{x};\theta) \) is the predicted probability of class \( k \) by \model, given the input \( \mathbf{x} \) and model parameters \( \theta \). The sum runs over all \( K \) classes, providing a comprehensive measure of the divergence between the prior and the predicted distributions.

% To further enhance the ability to differentiate ID data from OOD data, we introduce a confidence partition known as the Free Energy $E(\mathbf{x};\theta) = -\log \sum_{k=1}^K e^{f_k(\mathbf{x};\theta_\text{prior})}$, where \( f_k(\mathbf{x};\text{prior}) \) are the logits output by the prior model for class \( k \). The Free Energy has been proven effective for OOD detection~\cite{liu2020energy}, as it provides a measure of confidence in the model's predictions. High energy indicates less confidence (a more spread-out distribution), while low energy indicates high confidence (a more peaky distribution).\\

\noindent\textbf{Proposition: Cross Entropy \& Free Energy (CEFE) Guided Score Derivation}

\textit{Let \( q_k(\mathbf{x};\theta) \) be the predicted probability  obtained from the softmax function applied to the model's logits \( f_k(\mathbf{x};\theta) \). The CEFE score \( S_{\text{CEFE}}(\mathbf{x};\theta) \) is given by the following expression:}
\begin{equation}
    \text{score} = -z_k \log(\sum_{j=1}^{n} e^{z_j}) + \left(\log(\sum_{j=1}^{n} e^{z_j})\right)^2.
\end{equation}
\textit{which captures the relationship between the predicted class logits and the overall uncertainty.}\\

\textit{Proof:} Consider the predicted probability \( q_k(\mathbf{x};\theta) \) derived from the softmax function:

\begin{equation}
    q_k(\mathbf{x};\theta) = \frac{e^{f_k(\mathbf{x};\theta)}}{\sum_{j=1}^K e^{f_j(\mathbf{x};\theta)}}.
\end{equation}

The PCE score \( S_{\text{PCE}}(\mathbf{x};\theta) \) is initially expressed as the negative cross-entropy:

\begin{equation}
    S_{\text{PCE}}(\mathbf{x};\theta) = -\sum_{i=1}^{n} y_i \log\left(\frac{e^{z_i}}{\sum_{j=1}^{n} e^{z_j}}\right).
\end{equation}

Simplifying the expression using logarithmic properties, we have:

\begin{equation}
    = -\sum_{i=1}^{n} y_i (z_i - \log(\sum_{j=1}^{n} e^{z_j})).
\end{equation}

The cross-entropy loss can be decomposed into two terms:

\begin{equation}
    = -\sum_{i=1}^{n} y_i z_i + \sum_{i=1}^{n} y_i \log(\sum_{j=1}^{n} e^{z_j}).
\end{equation}

Since \( y_i \) is a one-hot vector, only the term for the true class label \( k \) is non-zero:

\begin{equation}
    = -z_k + \log(\sum_{j=1}^{n} e^{z_j}).
\end{equation}

Incorporating the energy term into the score, we obtain:

\begin{equation}
    \text{score} = \left(-z_k + \log(\sum_{j=1}^{n} e^{z_j})\right) \times \log(\sum_{j=1}^{n} e^{z_j}).
\end{equation}

Expanding this expression results in:

\begin{equation}
    = -z_k \log(\sum_{j=1}^{n} e^{z_j}) + \left(\log(\sum_{j=1}^{n} e^{z_j})\right)^2.
\end{equation}

\textbf{Interpretation:}

The term \( -z_k \log(\sum_{j=1}^{n} e^{z_j}) \) combines the logit of the true class \( z_k \) with the uncertainty from the log-sum-exp of all logits, highlighting how the true class logit is penalized by the overall uncertainty. The quadratic term \( \left(\log(\sum_{j=1}^{n} e^{z_j})\right)^2 \) emphasizes the role of uncertainty, as higher uncertainty results in a larger penalty, aiding in distinguishing OOD samples by boosting their scores due to inherently higher uncertainty.

Thus, the PCE score serves as a reliable indicator of whether the input data aligns with the known distribution or represents an anomaly.

\qed













% The overall OOD score can be represented as:

% \begin{equation}
%     S(\mathbf{x};\theta) = S_{\text{PCE}}(\mathbf{x};\theta) \cdot E(\mathbf{x};\theta),
%     \label{eq:overall_score}
% \end{equation}

% \noindent \textbf{Derivation}
% The predicted probability \( q_k(\mathbf{x};\theta) \) can be obtained from the softmax function applied to the model's logits \( f_k(\mathbf{x};\theta) \):
% \begin{equation}
%     q_k(\mathbf{x};\theta) = \frac{e^{f_k(\mathbf{x};\theta)}}{\sum_{j=1}^K e^{f_j(\mathbf{x};\theta)}}.
% \end{equation}

% \begin{equation}
%     S_{\text{PCE}}(\mathbf{x};\theta) = -\sum_{i=1}^{n} y_i \log\left(\frac{e^{z_i}}{\sum_{j=1}^{n} e^{z_j}}\right).
% \end{equation}

% Simplify this expression:

% \begin{equation}
%     = -\sum_{i=1}^{n} y_i (z_i - \log(\sum_{j=1}^{n} e^{z_j})).
% \end{equation}

% The cross-entropy loss can be split into two terms:

% \begin{equation}
%     = -\sum_{i=1}^{n} y_i z_i + \sum_{i=1}^{n} y_i \log(\sum_{j=1}^{n} e^{z_j}).
% \end{equation}

% Since \( y_i \) is a one-hot vector, only the term corresponding to the true class label \( k \) will be non-zero:

% \begin{equation}
%     = -z_k + \log(\sum_{j=1}^{n} e^{z_j}).
% \end{equation}

% Now, incorporate the energy term into the score:

% \begin{equation}
%     \text{score} = \left(-z_k + \log(\sum_{j=1}^{n} e^{z_j})\right) \times \log(\sum_{j=1}^{n} e^{z_j}).
% \end{equation}

% Expanding this expression:

% \begin{equation}
%     = -z_k \log(\sum_{j=1}^{n} e^{z_j}) + \left(\log(\sum_{j=1}^{n} e^{z_j})\right)^2.
% \end{equation}

% \textbf{Interpretation}

% The derived expression shows the following:

% \( -z_k \log(\sum_{j=1}^{n} e^{z_j}) \): This term combines the logit of the true class \( z_k \) with the uncertainty represented by the log-sum-exp of all logits. It highlights how much the true class logit is penalized by the overall uncertainty.

% \( \left(\log(\sum_{j=1}^{n} e^{z_j})\right)^2 \): This quadratic term emphasizes the role of uncertainty. Higher uncertainty results in a larger penalty, which helps in distinguishing OOD samples by boosting their scores due to their inherently higher uncertainty.


% For the OOD detection, ID and OOD samples are distinguished using the following decision rule:
% \begin{equation}
%     G(\hat{\mathbf{x}})=\left\{\begin{array}{ll}
% 1 & \text{if } S(\hat{\mathbf{x}};\theta) \geq \gamma, \\
% 0 & \text{if } S(\hat{\mathbf{x}};\theta) < \gamma,
% \end{array}\right.
% \label{eq:ood_rule}
% \end{equation}
% \noindent where \( G(\hat{\mathbf{x}})=1 \) indicates that the input is ID, while \( G(\hat{\mathbf{x}})=0 \) designates OOD data. The threshold \( \gamma \) is chosen to ensure a high classification accuracy for ID data, such as 95\%.


==> sec/checklist.tex <==
\section{Reproducibility Checklist}
\begin{enumerate}

\item This paper:
\begin{enumerate}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced \answerYes{Yes}

    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \answerYes{Yes, see the Methods and the Appendix.}

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \answerYes{Yes, see the Methods and the Appendix.}
\end{enumerate}
    
\item Does this paper make theoretical contributions? \answerYes{Yes, see the Methods and the Appendix.}

If yes, please complete the list below.
\begin{enumerate}
    \item All assumptions and restrictions are stated clearly and formally. \answerYes{Yes, see the Methods and the Appendix.}

    \item All novel claims are stated formally (e.g., in theorem statements). \answerYes{Yes, see the Methods and the Appendix.} 

    \item Proofs of all novel claims are included. (yes/partial/no) \answerYes{Yes, see the Methods and the Appendix.}

    \item Proof sketches or intuitions are given for complex and/or novel results.  \answerYes{Partial, see the Methods and the Appendix.}

    \item Appropriate citations to theoretical tools used are given. \answerYes{Yes, see the Methods and the Appendix.}
    
    \item All theoretical claims are demonstrated empirically to hold. \answerYes{Yes, see the Methods and the Appendix.}

    \item All experimental code used to eliminate or disprove claims is included. \answerYes{Yes.}
\end{enumerate}

\item Does this paper rely on one or more datasets? \answerYes{Yes.}

If yes, please complete the list below.
\begin{enumerate}
    \item A motivation is given for why the experiments are conducted on the selected datasets \answerYes{Yes.}
    
    \item All novel datasets introduced in this paper are included in a data appendix. \answerNA{NA}
    
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerNA{NA}
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes{Yes.}
    
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes{Yes, all datasets used in this paper are public avaiable.}
    
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerNA{NA}
\end{enumerate}

\item Does this paper include computational experiments? \answerYes{Yes}

If yes, please complete the list below.
\begin{enumerate}
    \item Any code required for pre-processing data is included in the appendix. \answerYes{Yes, all code, along with instructions and checkpoints are provided in the Appendix to ensure reproducibility}

    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerYes{Yes, all code, along with instructions and checkpoints are provided in the Appendix to ensure reproducibility}
    
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{Yes}
    
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \answerYes{Yes, see the readme in the code repo.}
    
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerYes{Yes, all code, along with instructions and checkpoints are provided in the Appendix to ensure reproducibility}
    
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes{Yes, all code, along with instructions and checkpoints are provided in the Appendix to ensure reproducibility}
    
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes{Yes, see the Experiments.}

    \item This paper states the number of algorithm runs used to compute each reported result. \answerYes{Yes, all the results presented require a single run.}
    
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes{Yes, see the Experiments and the Appendix.}
    
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \answerNo{No, our evaluation process follows the common benchmarking practices in the field.}
    
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes{Yes, see the Experiments and the Appendix.}
    
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes{Yes, see the Experiments and the Appendix.}
    
    
\end{enumerate}

\end{enumerate}

==> tab/cifar100.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}



% \begin{tabular}{lcccccccccccccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{Methods}}           & \multicolumn{2}{c}{\textsc{CIFAR10}}           & \multicolumn{2}{c}{\textsc{Texture}}           & \multicolumn{2}{c}{\textsc{SVHN}}              & \multicolumn{2}{c}{\textsc{Places365}}         & \multicolumn{2}{c}{\textsc{LSUN}}              & \multicolumn{2}{c}{\textsc{iSUN}}              & \multicolumn{2}{c}{Mean}              \\ \cline{2-15} 
% \multicolumn{1}{c}{}                                   &  { \tiny FPR95$\downarrow$} &  { \tiny AUROC$\uparrow$} &  { \tiny FPR95$\downarrow$} &  { \tiny AUROC$\uparrow$} &  { \tiny FPR95$\downarrow$} &   { \tiny AUROC$\uparrow$} &  { \tiny FPR95$\downarrow$} &  { \tiny AUROC$\uparrow$} &  { \tiny FPR95$\downarrow$} &  { \tiny AUROC$\uparrow$} &  { \tiny FPR95$\downarrow$} &  { \tiny AUROC$\uparrow$} &  { \tiny FPR95$\downarrow$} &  { \tiny AUROC $\uparrow$} \\ \hline
% MSP~\cite{hendrycks2016baseline} & 85.94             & 65.86             & 80.81             & 78.62             & 84.93             & 70.49             & 80.47             & 70.59             & 76.54             & 80.96             & 75.04             & 78.34             & 80.62             & 74.14             \\
% ODIN~\cite{liang2018enhancing}   & 86.87             & 66.97             & 73.28             & 81.71             & 91.19             & 62.64             & 78.71             & 77.54             & 75.71             & 78.12             & \textbf{53.64}             & 85.62             & 76.57             & 75.43             \\
% Mahalanobis~\cite{lee2018simple} & 82.45             & 66.32             & 63.46             & 81.79             & 89.82             & 65.09             & 77.14             & \textbf{78.46}             & 64.28             & 81.78             & 58.68             & \textbf{88.41}             & 72.64             & 76.97             \\
% Energy~\cite{liu2020energy}      & 85.04             & 67.54             & 80.13             & 77.81             & 71.32             & 77.03             & 80.05             & 69.50             & 84.43             & 75.77             & 73.49             & 82.04             & 79.08             & 74.95             \\
% KNN~\cite{sun2022out}            & 82.53             & 64.14             & 75.60             & 78.05             & 78.96             & 75.55             & 81.49             & 77.63             & 62.82             & \textbf{84.88}             & 69.31             & 77.66             & 75.12             & 76.32             \\
% GEN~\cite{xixi2023GEN}           & 84.93             & 68.32             & 77.42             & 71.12             & 85.14             & 72.10             & 81.31             & 69.30             & 79.19             & 77.51             & 71.51             & 81.16             & 79.92             & 73.25             \\ 
% \midrule
% \textbf{PViT (Ours)}                                            &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   \\
 
% PCE + ResNet-18                                         & 86.16             & \textbf{68.72}             & 79.74             & 72.59             & 79.24             & \textbf{78.28}             & 83.09             & 72.40             & 80.69             & 76.47             & 81.53             & 74.73             & 81.74             & 73.87             \\
 
% PCE + ViT                                              & \textbf{74.94}             & 68.05             & \textbf{51.91}             & \textbf{87.15}             & \textbf{64.51}             & 78.13             & \textbf{71.71}             & 73.94             & \textbf{61.94}             & 78.80             & 69.14             & 77.28             & \textbf{65.69}             & \textbf{77.23}            
% \\
% \bottomrule
% \end{tabular}

% % \rowcolor[HTML]{EFEFEF} 

==> tab/cifar100_append.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{tabular}{lccccccccccccccc}
\toprule
\multicolumn{2}{l}{OOD Datasets} & \multicolumn{2}{c}{\textsc{cifar10}} & \multicolumn{2}{c}{\textsc{textures}} & \multicolumn{2}{c}{\textsc{places}} & \multicolumn{2}{c}{\textsc{lsun}} & \multicolumn{2}{c}{\textsc{sun}} & \multicolumn{2}{c}{\textsc{svhn}} & \multicolumn{2}{c}{Mean} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16}
\multicolumn{2}{l}{Metrics} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} \\ 

Methods & Model & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} \\ 
\midrule
MSP & ResNet18 & 79.98 & 78.68 & 80.02 & 78.14 & 82.52 & 73.34 & 74.51 & 82.58 & 74.15 & 82.06 & 79.46 & 80.20 & 78.44 & 79.17 \\
MaxLogit & ResNet18 & 79.36 & 79.35 & 78.76 & 79.33 & 82.17 & 73.53 & 72.87 & 85.25 & 70.45 & 84.72 & 77.69 & 83.20 & 76.88 & 80.90 \\
Energy & ResNet18 & 79.62 & 79.17 & 77.75 & 79.30 & 82.62 & 73.36 & 72.19 & 85.42 & 67.35 & 85.12 & 76.82 & 83.52 & 76.06 & 80.98 \\
SSD & ResNet18 & 92.94 & 55.31 & 79.04 & 71.07 & 92.41 & 58.98 & 94.16 & 55.67 & 77.66 & 71.67 & 90.39 & 68.12 & 87.77 & 63.47 \\
ViM & ResNet18 & 93.57 & 54.50 & 82.73 & 66.53 & 92.61 & 56.53 & 93.98 & 53.60 & 77.59 & 68.25 & 85.64 & 69.28 & 87.69 & 61.45 \\
KNN & ResNet18 & 99.96 & 31.84 & 99.50 & 49.82 & 99.15 & 42.16 & 99.99 & 38.49 & 99.80 & 46.62 & 99.92 & 48.26 & 99.72 & 42.87 \\
NNGuide & ResNet18 & 80.02 & 78.46 & 75.85 & 80.23 & 81.52 & 74.46 & 70.82 & 85.81 & 62.36 & 86.44 & 80.64 & 82.94 & 75.20 & 81.39 \\
\rowcolor[HTML]{EFEFEF} PViT + CE & ResNet18 &  81.68 &  78.99 &  78.72 &  79.10 &  87.12 &  71.17 &  92.18 &  77.56 &  65.02 &  85.09 &  73.87 &  83.57 &  79.77 &  79.25 \\
\rowcolor[HTML]{EFEFEF} PViT + KL & ResNet18 &  84.74 &  77.29 &  86.79 &  76.04 &  90.68 &  70.64 &  89.02 &  78.14 &  75.80 &  80.59 &  84.17 &  79.08 &  85.20 &  76.96 \\
\rowcolor[HTML]{EFEFEF} PViT + ED & ResNet18 &  86.88 &  76.89 &  81.28 &  77.90 &  83.09 &  71.32 &  88.73 &  76.84 &  71.73 &  83.63 &  79.68 &  81.04 &  81.90 &  77.94 \\
\midrule
MSP & ViT & 75.42 & 77.62 & 69.89 & 81.82 & 80.98 & 75.94 & 72.79 & 82.31 & 76.83 & 81.32 & 77.99 & 80.81 & 75.65 & 79.97 \\
MaxLogit & ViT & 57.49 & 83.65 & 40.04 & 90.13 & 69.07 & 84.14 & 48.79 & 89.77 & 62.44 & 87.15 & 50.08 & 89.86 & 54.65 & 87.45 \\
Energy & ViT & 57.45 & 83.68 & 39.82 & 90.19 & 69.17 & 84.18 & 48.79 & 89.82 & 62.77 & 87.18 & 49.93 & 89.92 & 54.66 & 87.50 \\
SSD & ViT & 54.77 & 87.85 & 24.45 & 94.79 & 62.65 & 85.45 & 41.31 & 92.31 & 73.65 & 86.45 & 43.32 & 89.46 & 50.03 & 89.39 \\
ViM & ViT & 54.23 & 87.89 & 23.10 & 95.03 & 59.48 & 86.28 & 37.97 & 92.80 & 71.90 & 86.74 & 49.86 & 88.18 & 49.42 & 89.49 \\
KNN & ViT & 99.03 & 43.72 & 99.20 & 49.68 & 99.86 & 36.98 & 99.98 & 38.56 & 99.99 & 30.09 & 99.98 & 41.39 & 99.67 & 40.07 \\
NNGuide & ViT & 59.12 & 80.49 & 41.93 & 85.85 & 70.88 & 80.87 & 54.04 & 83.51 & 66.71 & 82.09 & 52.10 & 85.62 & 57.46 & 83.07 \\
\rowcolor[HTML]{EFEFEF} PViT + CE & ViT &  64.97 &  82.20 &  47.00 &  89.31 &  77.74 &  81.29 &  58.43 &  87.99 &  75.74 &  84.11 &  66.36 &  87.62 &  65.04 &  85.42 \\
\rowcolor[HTML]{EFEFEF} PViT + KL & ViT &  76.96 &  78.43 &  64.93 &  83.83 &  83.95 &  76.10 &  78.66 &  82.35 &  77.45 &  81.90 &  74.19 &  81.79 &  76.02 &  80.73 \\
\rowcolor[HTML]{EFEFEF} PViT + ED & ViT &  67.36 &  79.37 &  48.78 &  88.33 &  77.08 &  80.25 &  60.25 &  86.04 &  75.57 &  83.98 &  68.27 &  83.98 &  66.22 &  83.66 \\
\bottomrule
\end{tabular}

% \begin{tabular}{lccccccccccccccc}
% \toprule
% \multicolumn{2}{l}{OOD Datasets} & \multicolumn{2}{c}{\textsc{cifar10}} & \multicolumn{2}{c}{\textsc{textures}} & \multicolumn{2}{c}{\textsc{places}} & \multicolumn{2}{c}{\textsc{lsun}} & \multicolumn{2}{c}{\textsc{sun}} & \multicolumn{2}{c}{\textsc{svhn}} & \multicolumn{2}{c}{Mean} \\ 
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16}
% \multicolumn{2}{l}{Metrics} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} & \small{FPR95} & \small{AUROC} \\ 

% Methods & Model & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} & \small{$\downarrow$} & \small{$\uparrow$} \\ 
% \midrule
% MSP & ResNet18 & 79.98 & 78.68 & 80.02 & 78.14 & 82.52 & 73.34 & 74.51 & 82.58 & 74.15 & 82.06 & 79.46 & 80.20 & 78.44 & 79.17 \\
% MaxLogit & ResNet18 & 79.36 & 79.35 & 78.76 & 79.33 & 82.17 & 73.53 & 72.87 & 85.25 & 70.45 & 84.72 & 77.69 & 83.20 & 76.88 & 80.90 \\
% Energy & ResNet18 & 79.62 & 79.17 & 77.75 & 79.30 & 82.62 & 73.36 & \textbf{72.19} & 85.42 & \textbf{67.35} & 85.12 & 76.82 & 83.52 & \textbf{76.06} & 80.98 \\
% SSD & ResNet18 & 92.94 & 55.31 & 79.04 & 71.07 & 92.41 & 58.98 & 94.16 & 55.67 & 77.66 & 71.67 & 90.39 & 68.12 & 87.77 & 63.47 \\
% ViM & ResNet18 & 93.57 & 54.50 & 82.73 & 66.53 & 92.61 & 56.53 & 93.98 & 53.60 & 77.59 & 68.25 & 85.64 & 69.28 & 87.69 & 61.45 \\
% KNN & ResNet18 & 99.96 & 31.84 & 99.50 & 49.82 & 99.15 & 42.16 & 99.99 & 38.49 & 99.80 & 46.62 & 99.92 & 48.26 & 99.72 & 42.87 \\
% NNGuide & ResNet18 & 80.02 & 78.46 & \textbf{75.85} & 80.23 & \textbf{81.52} & 74.46 & 70.82 & \textbf{85.81} & 62.36 & \textbf{86.44} & 80.64 & \textbf{82.94} & 75.20 & \textbf{81.39} \\
% \rowcolor[HTML]{EFEFEF} PViT + CE & ResNet18 & 81.68 & 78.99 & 78.72 & 79.10 & 87.12 & 71.17 & 92.18 & 77.56 & 65.02 & 85.09 & 73.87 & 83.57 & 79.77 & 79.25 \\
% \rowcolor[HTML]{EFEFEF} PViT + KL & ResNet18 & 84.74 & 77.29 & 86.79 & 76.04 & 90.68 & 70.64 & 89.02 & 78.14 & 75.80 & 80.59 & 84.17 & 79.08 & 85.20 & 76.96 \\
% \rowcolor[HTML]{EFEFEF} PViT + ED & ResNet18 & 86.88 & 76.89 & 81.28 & 77.90 & 83.09 & 71.32 & 88.73 & 76.84 & 71.73 & 83.63 & 79.68 & 81.04 & 81.90 & 77.94 \\
% \midrule
% MSP & ViT & 75.42 & 77.62 & 69.89 & 81.82 & 80.98 & 75.94 & 72.79 & 82.31 & 76.83 & 81.32 & 77.99 & 80.81 & 75.65 & 79.97 \\
% MaxLogit & ViT & 57.49 & 83.65 & 40.04 & 90.13 & 69.07 & 84.14 & 48.79 & 89.77 & 62.44 & 87.15 & 50.08 & 89.86 & 54.65 & 87.45 \\
% Energy & ViT & \textbf{57.45} & \textbf{83.68} & \textbf{39.82} & 90.19 & 69.17 & 84.18 & 48.79 & \textbf{89.82} & 62.77 & 87.18 & 49.93 & \textbf{89.92} & 54.66 & \textbf{87.50} \\
% SSD & ViT & 54.77 & 87.85 & 24.45 & \textbf{94.79} & 62.65 & 85.45 & 41.31 & 92.31 & 73.65 & 86.45 & \textbf{43.32} & 89.46 & 50.03 & 89.39 \\
% ViM & ViT & 54.23 & 87.89 & \textbf{23.10} & 95.03 & \textbf{59.48} & \textbf{86.28} & \textbf{37.97} & 92.80 & 71.90 & 86.74 & 49.86 & 88.18 & 49.42 & 89.49 \\
% KNN & ViT & 99.03 & 43.72 & 99.20 & 49.68 & 99.86 & 36.98 & 99.98 & 38.56 & 99.99 & 30.09 & 99.98 & 41.39 & 99.67 & 40.07 \\
% NNGuide & ViT & 59.12 & 80.49 & 41.93 & 85.85 & 70.88 & 80.87 & 54.04 & 83.51 & 66.71 & 82.09 & 52.10 & 85.62 & 57.46 & 83.07 \\
% \rowcolor[HTML]{EFEFEF} PViT + CE & ViT & 64.97 & 82.20 & 47.00 & 89.31 & 77.74 & 81.29 & 58.43 & 87.99 & 75.74 & 84.11 & 66.36 & 87.62 & 65.04 & 85.42 \\
% \rowcolor[HTML]{EFEFEF} PViT + KL & ViT & 76.96 & 78.43 & 64.93 & 83.83 & 83.95 & 76.10 & 78.66 & 82.35 & 77.45 & 81.90 & 74.19 & 81.79 & 76.02 & 80.73 \\
% \rowcolor[HTML]{EFEFEF} PViT + ED & ViT & 67.36 & 79.37 & 48.78 & 88.33 & 77.08 & 80.25 & 60.25 & 86.04 & 75.57 & 83.98 & 68.27 & 83.98 & 66.22 & 83.66 \\
% \bottomrule
% \end{tabular}


==> tab/cifar10_1.tex <==
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{OOD Dataset}} & \multicolumn{2}{c}{Energy} & \multicolumn{2}{c}{KL} & \multicolumn{2}{c}{Cross Entropy} & \multicolumn{2}{c}{Euclidean Distance} \\ 
\cmidrule{2-9}
&  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} &  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} &  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} &  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} \\
\midrule
\textsc{Texture} & 0.95  & 99.65 & 48.10 & 90.37 & 1.06  & 99.18 & 11.89 & 96.63 \\
\textsc{SVHN}          & 30.25 & 93.18 & 71.21 & 69.92 & 22.54 & 94.50 & 45.93 & 77.21 \\
\textsc{Places365}     & 7.59  & 97.71 & 46.99 & 83.43 & 10.60 & 97.07 & 22.43 & 89.52 \\
\textsc{LSUN\_C}       & 11.50 & 97.57 & 51.62 & 82.03 & 13.90 & 96.54 & 24.55 & 89.83 \\
\textsc{LSUN\_Resize}  & 43.53 & 89.36 & 79.69 & 51.58 & 42.02 & 91.10 & 54.41 & 68.40 \\
\textsc{iSUN}          & 37.44 & 90.19 & 77.18 & 55.88 & 36.66 & 91.43 & 54.07 & 70.98 \\
\textsc{CIFAR100}      & 33.71 & 89.95 & 74.89 & 66.06 & 33.20 & 90.41 & 50.33 & 74.63 \\
\midrule
Mean Test Results & 23.57 & 93.94 & 64.24 & 71.32 & 22.86 & 94.32 & 37.66 & 81.03 \\
\bottomrule
\end{tabular}











==> tab/cifar10_2.tex <==
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{OOD Dataset}} & \multicolumn{2}{c}{Energy} & \multicolumn{2}{c}{KL} & \multicolumn{2}{c}{Cross Entropy} & \multicolumn{2}{c}{Euclidean Distance} \\ 
\cmidrule{2-9}
&  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} &  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} &  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} &  \small{FPR95$\downarrow$} &  \small{AUROC$\uparrow$} \\
\midrule
\textsc{Texture}       & 0.67  & 99.74 & 0.78  & 99.18 & 0.84  & 99.55 & 0.78 & 99.29 \\
\textsc{SVHN}          & 25.61 & 94.43 & 24.05 & 95.00 & 25.06 & 95.64 & 24.83 & 93.31 \\
\textsc{Places365}     & 9.43  & 95.96 & 10.88 & 96.02 & 8.31  & 97.89 & 8.48  & 96.67 \\
\textsc{LSUN\_C}       & 11.16 & 96.34 & 15.07 & 95.24 & 13.45 & 97.34 & 11.50 & 97.25 \\
\textsc{LSUN\_Resize}  & 39.62 & 88.06 & 45.48 & 87.55 & 39.45 & 93.62 & 38.73 & 89.92 \\
\textsc{iSUN}          & 37.22 & 87.95 & 43.75 & 87.99 & 37.00 & 93.85 & 34.60 & 90.55 \\
\textsc{CIFAR100}      & 34.21 & 89.54 & 36.27 & 87.72 & 31.36 & 93.01 & 34.65 & 88.79 \\
\midrule
Mean Test Results & 24.56 & 93.15 & 22.54 & 92.67 & 22.21 & 95.84 & 23.38 & 93.33 \\
\bottomrule
\end{tabular}


==> tab/imagenet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}}            & \multicolumn{2}{c}{\textsc{SSB-hard}}         & \multicolumn{2}{c}{\textsc{ninco}}             & \multicolumn{2}{c}{\textsc{textures}}          & \multicolumn{2}{c}{\textsc{openimage\_o}}      & \multicolumn{2}{c}{\textsc{inaturalist}}       & \multicolumn{2}{c}{Mean}              \\ \cline{2-13} 
\multicolumn{1}{c}{}                                   & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ \\ \hline
MSP~\cite{hendrycks2016baseline}  & 96.90             & 57.16             & 94.72             & 57.16             & 77.13             & 79.76             & 76.21             & 83.05             & 64.53             & 87.90             & 81.90             & 73.01             \\
ODIN~\cite{liang2018enhancing}   & 91.60             & 52.63             & 82.56             & 76.55             & 74.07             & 81.60             & 72.83             & 85.64             & 70.75             & 86.73             & 78.36             & 76.63             \\
Mahalanobis~\cite{lee2018simple} & 95.60             & 45.16             & 97.60             & 39.16             & 93.60             & 72.16             & 93.60             & 73.16             & 91.60             & 75.16             & 94.40             & 60.96             \\
Energy~\cite{liu2020energy}      & 90.55             & 57.72             & 81.98             & 77.44             & \textbf{61.94}    & \textbf{86.55}    & \textbf{56.58}    & 87.46             & 54.35             & 89.82             & 69.08             & 79.80             \\
KNN~\cite{sun2022out}            & 86.90             & 57.94             & \textbf{76.24}    & \textbf{80.53}    & 63.52             & 84.67             & 56.92             & \textbf{87.52}             & 55.60             & 88.38             & 67.52             & \textbf{79.81}    \\
GEN~\cite{xixi2023GEN}           & 88.25             & 58.53             & 79.52             & 75.82             & 77.93             & 81.48             & 80.43             & 83.77    & 68.32             & 88.67             & 78.89             & 77.65             \\ 
\midrule
\textbf{PViT (Ours)}                                            &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   &                   \\
 
PCE + ResNet-18                                         & 89.73             & 57.22             & 82.23             & 73.69             & 66.60             & 82.65             & 57.45             & 82.05             & 52.35             & 85.64             & 69.67             & 76.25             \\

PCE + ViT                                              & \textbf{85.55}    & \textbf{62.63}    & 77.96             & 75.59             & 68.02             & 83.04             & 57.70             & 84.15             & \textbf{40.79}    & \textbf{90.55}    & \textbf{66.00}    & 79.19            
\\
\bottomrule
\end{tabular}



==> tab/imagenet_append.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{tabular}{lcccccccccccccccccc}
\toprule
\multicolumn{2}{l}{OOD Datasets} & \multicolumn{2}{c}{\textsc{inaturalist}} & \multicolumn{2}{c}{\textsc{sun}} & \multicolumn{2}{c}{\textsc{places}} & \multicolumn{2}{c}{\textsc{textures}} & \multicolumn{2}{c}{\textsc{ninco}} & \multicolumn{2}{c}{\textsc{openimage\_o}} & \multicolumn{2}{c}{\textsc{ssb-hard}} & \multicolumn{2}{c}{Mean} & ID \\ \cmidrule{3-18}
Methods & Model & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & ACC \\ \midrule
MSP & DeiT & 51.52 & 88.16 & 66.52 & 80.94 & 68.67 & 80.38 & 60.23 & 82.99 & 73.26 & 78.08 & 59.93 & 84.81 & 69.02 & 84.73 & 64.16 & 82.87 & 81.07 \\
MaxLogit & DeiT & 52.26 & 85.24 & 66.88 & 76.39 & 69.14 & 75.06 & 56.68 & 81.69 & 74.02 & 72.38 & 58.75 & 81.55 & 64.43 & 85.64 & 63.17 & 79.71 & 81.07 \\
Mahalanobis & DeiT & 21.28 & 95.59 & 61.55 & 85.12 & 61.48 & 83.92 & 53.94 & 87.35 & 58.74 & 85.98 & 44.03 & 91.73 & 70.85 & 76.58 & 53.12 & 86.61 & 81.07 \\
Energy & DeiT & 64.08 & 79.24 & 72.77 & 70.28 & 74.31 & 68.44 & 58.48 & 79.30 & 78.46 & 66.03 & 64.93 & 76.46 & 59.13 & 88.16 & 67.45 & 75.42 & 81.07 \\
SSD & DeiT & 25.58 & 94.21 & 65.75 & 81.04 & 66.58 & 79.90 & 53.35 & 85.28 & 61.93 & 82.89 & 48.23 & 90.14 & 66.57 & 80.58 & 55.43 & 84.86 & 81.07 \\
ViM & DeiT & 17.12 & 96.45 & 58.87 & 83.14 & 60.52 & 81.24 & 48.09 & 88.17 & 56.09 & 84.98 & 41.87 & 91.93 & 68.92 & 76.31 & 50.21 & 86.03 & 81.07 \\
KNN & DeiT & 71.35 & 85.55 & 79.51 & 79.48 & 78.61 & 78.27 & 68.58 & 82.76 & 78.94 & 76.73 & 66.11 & 85.86 & 59.56 & 90.23 & 71.81 & 82.70 & 81.07 \\
NNGuide & DeiT & 66.93 & 88.57 & 76.98 & 81.94 & 76.33 & 80.61 & 64.84 & 85.68 & 77.56 & 80.14 & 65.42 & 87.93 & 63.76 & 89.19 & 70.26 & 84.87 & 81.07 \\
\rowcolor[HTML]{EFEFEF} PViT + CE & DeiT & 2.26 & 99.39 & 30.98 & 93.38 & 40.35 & 90.99 & 32.96 & 92.05 & 41.63 & 90.74 & 16.59 & 96.58 & 58.32 & 84.49 & 31.87 & 92.52 & 81.33 \\
\rowcolor[HTML]{EFEFEF} PViT + KL & DeiT & 10.47 & 97.35 & 55.52 & 87.66 & 60.90 & 85.76 & 58.23 & 87.95 & 59.87 & 87.75 & 39.66 & 93.57 & 76.67 & 77.35 & 51.62 & 88.20 & 81.33 \\
\rowcolor[HTML]{EFEFEF} PViT + ED & DeiT & 3.27 & 99.08 & 30.85 & 93.00 & 38.24 & 91.28 & 33.30 & 90.63 & 38.23 & 90.93 & 18.78 & 95.81 & 56.78 & 84.72 & 31.35 & 92.21 & 81.33 \\\midrule
MSP & ViT-swag & 27.58 & 93.96 & 57.43 & 85.18 & 61.13 & 84.34 & 53.21 & 84.96 & 61.16 & 84.37 & 44.32 & 89.89 & 75.10 & 76.41 & 54.27 & 79.08 & 85.29 \\
MaxLogit & ViT-swag & 13.19 & 97.19 & 47.45 & 86.80 & 54.36 & 83.13 & 44.70 & 86.11 & 50.97 & 86.46 & 28.41 & 93.23 & 70.13 & 77.11 & 44.17 & 77.89 & 85.29 \\
Mahalanobis & ViT-swag & 4.94 & 98.85 & 58.77 & 88.15 & 65.62 & 85.45 & 43.49 & 90.30 & 41.54 & 91.17 & 23.87 & 95.92 & 68.17 & 76.97 & 43.77 & 79.25 & 85.29 \\
Energy & ViT-swag & 12.64 & 97.34 & 48.05 & 86.48 & 56.41 & 82.22 & 46.79 & 85.72 & 52.14 & 86.12 & 28.33 & 93.31 & 71.69 & 76.59 & 45.15 & 86.83 & 85.29 \\
SSD & ViT-swag & 11.19 & 97.50 & 84.91 & 70.87 & 88.23 & 65.10 & 69.38 & 79.81 & 67.00 & 78.96 & 45.01 & 88.62 & 89.96 & 59.10 & 65.10 & 70.91 & 85.29 \\
ViM & ViT-swag & 3.42 & 99.20 & 49.67 & 88.05 & 59.69 & 83.68 & 42.55 & 88.46 & 44.20 & 89.61 & 20.50 & 95.79 & 74.57 & 74.74 & 42.09 & 77.75 & 85.29 \\
KNN & ViT-swag & 29.46 & 94.07 & 72.15 & 83.88 & 74.17 & 81.47 & 51.21 & 87.17 & 68.80 & 82.50 & 45.25 & 91.49 & 86.43 & 66.51 & 61.07 & 77.27 & 85.29 \\
NNGuide & ViT-swag & 9.17 & 97.96 & 45.64 & 90.03 & 53.82 & 87.25 & 39.26 & 90.01 & 49.80 & 89.63 & 23.11 & 95.47 & 73.65 & 77.23 & 42.06 & 89.65 & 85.29 \\
\rowcolor[HTML]{EFEFEF} PViT + PCE & ViT-swag & 17.73 & 96.37 & 55.03 & 84.24 & 63.63 & 78.82 & 54.41 & 83.35 & 59.00 & 83.70 & 34.99 & 91.95 & 76.19 & 74.00 & 51.57 & 84.63 & 85.07 \\
\rowcolor[HTML]{EFEFEF} PViT + KL & ViT-swag & 44.15 & 94.11 & 66.00 & 86.22 & 70.09 & 83.98 & 60.99 & 87.29 & 65.02 & 86.26 & 49.70 & 92.23 & 75.92 & 77.99 & 61.70 & 86.87 & 85.07 \\
\rowcolor[HTML]{EFEFEF} PViT + ED & ViT-swag & 15.14 & 95.14 & 36.52 & 89.48 & 43.19 & 88.13 & 48.62 & 83.70 & 48.21 & 85.14 & 32.93 & 89.62 & 68.56 & 76.24 & 41.88 & 86.78 & 85.07 \\ \midrule
MSP & ResNet50 & 29.73 & 93.78 & 59.62 & 84.56 & 60.91 & 84.28 & 49.98 & 84.90 & 60.97 & 84.79 & 47.49 & 89.68 & 80.27 & 73.25 & 55.57 & 85.03 & 78.73 \\ 
MaxLogit & ResNet50 & 22.12 & 95.99 & 50.94 & 88.43 & 53.79 & 87.37 & 42.23 & 88.42 & 57.86 & 87.01 & 41.68 & 92.23 & 78.91 & 74.09 & 49.65 & 87.65 & 78.73 \\
Mahalanobis & ResNet50 & 34.97 & 94.79 & 64.98 & 86.55 & 70.30 & 83.92 & 15.02 & 95.52 & 63.75 & 87.13 & 37.51 & 93.89 & 85.41 & 71.71 & 53.13 & 87.64 & 78.73 \\
Energy & ResNet50 & 20.99 & 96.17 & 47.10 & 88.91 & 51.18 & 87.70 & 39.34 & 88.89 & 58.08 & 86.96 & 41.63 & 92.32 & 78.49 & 74.01 & 48.12 & 87.85 & 78.73 \\
SSD & ResNet50 & 33.68 & 94.64 & 56.00 & 88.34 & 65.09 & 84.51 & 11.79 & 96.54 & 69.00 & 83.63 & 37.93 & 93.29 & 88.30 & 66.49 & 51.68 & 86.78 & 78.73 \\
ViM & ResNet50 & 16.68 & 96.87 & 39.37 & 90.86 & 49.24 & 88.48 & 15.87 & 94.20 & 61.84 & 86.95 & 28.20 & 94.59 & 85.59 & 72.17 & 42.40 & 89.16 & 78.73 \\
KNN & ResNet50 & 37.60 & 93.87 & 54.53 & 86.98 & 63.32 & 83.54 & 17.43 & 94.13 & 69.45 & 82.02 & 40.75 & 92.46 & 90.07 & 61.65 & 53.31 & 84.95 & 78.73 \\
NNGuide & ResNet50 & 11.98 & 97.47 & 31.67 & 91.66 & 38.91 & 90.12 & 24.96 & 91.51 & 60.99 & 86.56 & 31.62 & 93.66 & 82.44 & 73.06 & 40.37 & 89.15 & 78.73 \\
\rowcolor[HTML]{EFEFEF} PViT + PCE & ResNet50 & 23.25 & 95.97 & 46.11 & 89.04 & 50.99 & 87.68 & 38.32 & 89.05 & 59.24 & 86.53 & 43.55 & 92.01 & 78.93 & 73.62 & 48.63 & 87.70 & 78.56 \\
\rowcolor[HTML]{EFEFEF} PViT + KL & ResNet50 & 37.11 & 94.12 & 69.32 & 84.66 & 71.61 & 83.74 & 45.50 & 87.27 & 64.09 & 85.90 & 51.72 & 91.03 & 81.12 & 73.06 & 60.07 & 85.68 & 78.56 \\
\rowcolor[HTML]{EFEFEF} PViT + ED & ResNet50 & 16.89 & 96.09 & 36.10 & 90.21 & 40.97 & 89.21 & 56.24 & 85.94 & 54.71 & 87.19 & 42.46 & 91.27 & 74.99 & 74.39 & 46.05 & 88.73 & 78.56 \\ \midrule
MSP & RegNet & 23.62 & 94.64 & 52.50 & 86.58 & 56.82 & 85.13 & 49.22 & 86.47 & 53.23 & 86.77 & 34.64 & 91.94 & 71.97 & 77.96 & 48.86 & 87.07 & 86.01 \\
MaxLogit & RegNet & 7.79 & 98.04 & 31.68 & 91.55 & 41.05 & 88.08 & 32.68 & 91.19 & 34.31 & 91.44 & 16.74 & 95.68 & 54.33 & 84.39 & 31.23 & 91.48 & 86.01 \\
Mahalanobis & RegNet & 2.22 & 99.36 & 49.33 & 89.85 & 61.86 & 85.77 & 27.91 & 93.90 & 38.23 & 92.06 & 19.51 & 96.48 & 71.89 & 77.71 & 38.71 & 90.73 & 86.01 \\
Energy & RegNet & 6.68 & 98.28 & 29.41 & 91.88 & 40.51 & 87.97 & 30.85 & 91.48 & 34.03 & 91.53 & 16.19 & 95.81 & 52.44 & 84.82 & 30.02 & 91.68 & 86.01 \\
SSD & RegNet & 5.11 & 98.82 & 60.35 & 85.88 & 70.88 & 80.27 & 38.14 & 92.58 & 54.30 & 86.31 & 28.77 & 93.54 & 83.70 & 69.72 & 48.75 & 86.73 & 86.01 \\
ViM & RegNet & 1.97 & 99.52 & 28.21 & 93.15 & 42.74 & 89.05 & 20.55 & 95.58 & 34.04 & 92.71 & 13.57 & 97.15 & 65.66 & 81.27 & 29.53 & 92.63 & 86.01 \\
KNN & RegNet & 4.32 & 98.76 & 46.15 & 88.45 & 56.30 & 85.15 & 28.33 & 91.93 & 56.99 & 85.57 & 21.30 & 95.51 & 86.19 & 67.01 & 42.80 & 87.48 & 86.01 \\
NNGuide & RegNet & 1.83 & 99.57 & 21.58 & 94.44 & 31.47 & 91.87 & 17.00 & 95.82 & 29.40 & 93.58 & 10.79 & 97.73 & 55.86 & 84.09 & 23.99 & 93.87 & 86.01 \\
\rowcolor[HTML]{EFEFEF} PViT + PCE & RegNet & 14.21 & 96.64 & 51.93 & 83.34 & 60.53 & 78.38 & 48.10 & 86.06 & 54.13 & 83.87 & 30.85 & 91.65 & 72.58 & 71.77 & 47.48 & 84.53 & 83.25 \\
\rowcolor[HTML]{EFEFEF} PViT + KL & RegNet & 23.71 & 94.96 & 69.04 & 82.56 & 69.99 & 81.10 & 61.68 & 86.14 & 61.04 & 86.12 & 38.60 & 92.00 & 81.28 & 73.54 & 57.91 & 85.20 & 83.25 \\
\rowcolor[HTML]{EFEFEF} PViT + ED & RegNet & 64.39 & 90.09 & 68.89 & 80.76 & 75.88 & 78.90 & 77.38 & 79.71 & 62.08 & 82.84 & 64.64 & 83.94 & 78.24 & 71.57 & 70.21 & 81.12 & 83.25 \\
\bottomrule
\end{tabular}


==> tab/imagenet_pvit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{tabular}{lccccccccccccccccc}
\hline
\multicolumn{1}{c}{}                                   & \multicolumn{2}{c}{\textsc{inaturalist}}                         & \multicolumn{2}{c}{\textsc{sun}}                                                       & \multicolumn{2}{c}{\textsc{places}}                                                    & \multicolumn{2}{c}{\textsc{textures}}                            & \multicolumn{2}{c}{\textsc{ninco}}                               & \multicolumn{2}{c}{\textsc{openimage\_o}}                        & \multicolumn{2}{c}{\textsc{SSB-hard}}                            & \multicolumn{2}{c}{Mean}                                                      &                           \\ \cline{2-17}
\multicolumn{1}{c}{\multirow{-2}{*}{Method}}           & \tiny FPR95$\downarrow$ & \tiny AUROC $\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \tiny FPR95$\downarrow$ & \tiny AUROC$\uparrow$ & \multirow{-2}{*}{ACC} \\ \hline
MSP~\cite{hendrycks2016baseline} & 52.21                                  & 88.05                                & 67.13                                  & 80.75                                & 68.99                                  & 80.17                                & 62.39                                  & 82.03                                & 61.10                                  & 84.37                                & 85.50                                  & 68.48                                & 74.04                                  & 77.98                                & 67.34                                  & 80.26                                & 81.07                     \\
MaxLogit~\cite{hendrycks2019scaling}  & 52.90                                  & 85.33                                & 67.57                                  & 76.36                                & 69.66                                  & 75.16                                & 58.79                                  & 80.76                                & 60.34                                  & 81.17                                & 86.23                                  & 64.18                                & 74.04                                  & 72.33                                & 67.08                                  & 76.47                                & 81.07                     \\
Mahalanobis~\cite{lee2018simple} & 21.40                                  & 95.55                                & 62.72                                  & 84.65                                & 63.08                                  & 83.73                                & 53.07                                  & 87.00                                & 43.62                                  & \textbf{91.66}                                & 76.52                                  & 70.48                                & 58.59                                  & \textbf{86.23}                                & 54.14                                  & 85.61                                & 81.07                     \\
Energy~\cite{liu2020energy}      & 62.68                                  & 79.98                                & 73.14                                  & 70.53                                & 74.55                                  & 68.81                                & 60.09                                  & 78.29                                & 65.66                                  & 76.45                                & 88.06                                  & 59.24                                & 78.85                                  & 65.76                                & 71.86                                  & 71.29                                & 81.07                     \\
SSD~\cite{sehwag2021ssd}              & 25.93                                  & 94.14                                & 68.80                                  & 80.31                                & 68.98                                  & 79.49                                & 50.32                                  & 85.20                                & 47.37                                  & 90.17                                & 80.19                                  & 66.61                                & 61.47                                  & 83.46                                & 57.58                                  & 82.77                                & 81.07                     \\
ViM~\cite{wang2022vim}                 & 18.67                                  & 96.20                                & 61.65                         & 82.44                                & 63.21                                  & 80.61                                & 45.43                                  & 88.10                                & 42.53                                  & 91.88                                & 76.66                                  & 68.88                                & 55.58                                  & 85.52                                & 51.96                         & 84.80                                & 81.07                     \\
KNN~\cite{sun2022out}            & 68.61                                  & 85.77                                & 80.21                                  & 79.21                                & 78.06                                  & 78.31                                & 67.66                                  & 82.31                                & 65.77                                  & 85.59                                & 89.65                                  & 59.09                                & 77.65                                  & 76.93                                & 75.37                                  & 78.17                                & 81.07                     \\
NNGuide~\cite{park2023nearest}   & 65.39                                  & 88.63                                & 78.40                                  & 81.60                                & 76.15                                  & 80.56                                & 64.41                                  & 85.02                                & 64.72                                  & 87.66                                & 88.92                                  & 63.27                                & 76.45                                  & 80.35                                & 73.49                                  & 81.01                                & 81.07                     \\
\rowcolor[HTML]{EFEFEF} 
PViT + PCE                                             & \textbf{2.25}                         & \textbf{99.39}                        & 30.99                                  & 93.38                                & 40.46                                  & 90.97                                & \textbf{32.94}                         & \textbf{92.08}                        & 41.51                                  & 90.77                                & 31.29                                  & 91.59                                & 58.27                                  & 84.53                                & 33.96                                  & 91.82                                & 80.82                     \\
\rowcolor[HTML]{EFEFEF} 
PViT + ED                                              & 2.72                                   & 99.15                                & \textbf{25.29}                         & \textbf{93.87}                        & \textbf{33.63}                         & \textbf{92.29}                        & 42.38                                  & 89.07                                & \textbf{37.38}                         & 90.24                        & \textbf{24.93}                         & \textbf{94.67}                        & \textbf{52.01}                         & 86.12                                & \textbf{31.19}                         & \textbf{92.20}                        & 80.82                     \\ \hline
MSP~\cite{hendrycks2016baseline} & 27.58                                  & 93.96                                & 57.43                                  & 85.18                                & 61.13                                  & 84.34                                & 53.21                                  & 84.96                                & 61.16                                  & 84.37                                & 44.32                                  & 89.89                                & 75.10                                  & 76.41                                & 54.27                                  & 79.08                                & 85.29                     \\
MaxLogit~\cite{hendrycks2019scaling}  & 13.19                                  & 97.19                                & 47.45                                  & 86.80                                & 54.36                                  & 83.13                                & 44.70                                  & 86.11                                & 50.97                                  & 86.46                                & 28.41                                  & 93.23                                & 70.13                                  & 77.11                                & 44.17                                  & 77.89                                & 85.29                     \\
Mahalanobis~\cite{lee2018simple} & 4.94                                   & 98.85                                & 58.77                                  & 88.15                                & 65.62                                  & 85.45                                & 43.49                                  & \textbf{90.30}                                & \textbf{41.54}                                  & \textbf{91.17}                                & 23.87                                  & \textbf{95.92}                                & \textbf{68.17}                                  & 76.97                                & 43.77                                  & 79.25                                & 85.29                     \\
Energy~\cite{liu2020energy}      & 12.64                                  & 97.34                                & 48.05                                  & 86.48                                & 56.41                                  & 82.22                                & 46.79                                  & 85.72                                & 52.14                                  & 86.12                                & 28.33                                  & 93.31                                & 71.69                                  & 76.59                                & 45.15                                  & 86.83                               & 85.29                     \\
SSD~\cite{sehwag2021ssd}              & 11.19                                  & 97.50                                & 84.91                                  & 70.87                                & 88.23                                  & 65.10                                & 69.38                                  & 79.81                                & 67.00                                  & 78.96                                & 45.01                                  & 88.62                                & 89.96                                  & 59.10                                & 65.10                                  & 70.91                                & 85.29                     \\
ViM~\cite{wang2022vim}                 & \textbf{3.42}                                   & \textbf{99.20}                       & 49.67                                  & 88.05                                & 59.69                                  & 83.68                                & 42.55                                  & 88.46                                & 44.20                                  & 89.61                                & \textbf{20.50}                                  & 95.79                                & 74.57                                  & 74.74                                & 42.09                                  & 77.75                                & 85.29                     \\
KNN~\cite{sun2022out}            & 29.46                                  & 94.07                                & 72.15                                  & 83.88                                & 74.17                                  & 81.47                                & 51.21                                  & 87.17                                & 68.80                                  & 82.50                                & 45.25                                  & 91.49                                & 86.43                                  & 66.51                                & 61.07                                  & 77.27                                & 85.29                     \\
NNGuide~\cite{park2023nearest}   & 9.17                                   & 97.96                                & 45.64                                  & \textbf{90.03}                               & 53.82                                  & 87.25                                & \textbf{39.26}                                  & 90.01                                & 49.80                                  & 89.63                                & 23.11                                  & 95.47                                & 73.65                                  & \textbf{77.23}                                & 42.06                                  & \textbf{89.65}                                & 85.29                     \\
\rowcolor[HTML]{EFEFEF} 
PViT + PCE                                             & 17.73                                  & 96.37                                & 55.03                                  & 84.24                                & 63.63                                  & 78.82                                & 54.41                                  & 83.35                                & 59.00                                  & 83.70                                & 34.99                                  & 91.95                                & 76.19                                  & 74.00                                & 51.57                                  & 84.63                                & 85.07                     \\
\rowcolor[HTML]{EFEFEF} 
PViT + ED                                              & 15.14                                  & 95.14                                & \textbf{36.52}                                  & 89.48                                & \textbf{43.19}                                  & \textbf{88.13}                                & 48.62                                  & 83.70                                & 48.21                                  & 85.14                                & 32.93                                  & 89.62                                & 68.56                                  & 76.24                                & \textbf{41.88}                                  & 86.78                                & 85.07                     \\ \cline{1-13}
\end{tabular}


==> tab/scale.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{ccccc}
\toprule
\multirow{2}{*} {Scale factor \( \alpha \)} & \multicolumn{2}{c}{\textsc{Texture}}           & \multicolumn{2}{c}{\textsc{SVHN}}              \\ \cmidrule{2-5} 
                              & {FPR95$\downarrow$} & {AUROC$\uparrow$} & {FPR95$\downarrow$} & {AUROC$\uparrow$} \\ \midrule
100                           & 0.84              & \textbf{99.55}             & 25.06             & 95.64             \\
10                            & 1.23              & 99.50             & \textbf{24.78}             & \textbf{95.96}             \\
5                             & \textbf{0.73}              & 99.22             & 24.83             & 95.33             \\
1                             & \textbf{0.73}              & 99.31             & 24.83             & 95.64             \\
0.1                           & 1.34              & 99.15             & 25.67             & 95.48             \\
0.01                          & 0.95              & 99.33             & 26.12             & 95.82            
\\
\bottomrule
\end{tabular}

